Learning Binary Decision Trees by Argmin Differentiation

We address the problem of learning binary decision trees that partition data for some downstream task. We propose to learn discrete parameters (i.e., for tree traversals and node pruning) and continuous parameters (i.e., for tree split functions and prediction functions) simultaneously using argmin differentiation. We do so by sparsely relaxing a mixed-integer program for the discrete parameters, to allow gradients to pass through the program to continuous parameters. We derive customized algorithms to efficiently compute the forward and backward passes. This means that our tree learning procedure can be used as an (implicit) layer in arbitrary deep networks, and can be optimized with arbitrary loss functions. We demonstrate that our approach produces binary trees that are competitive with existing single tree and ensemble approaches, in both supervised and unsupervised settings. Further, apart from greedy approaches (which do not have competitive accuracies), our method is faster to train than all other tree-learning baselines we compare with. The code for reproducing the results is available at https://github.com/vzantedeschi/LatentTrees.

==> Learning Latent Decision Trees/commands.tex <==
% TIKZ SETTINGS
\usetikzlibrary{cd,arrows,calc,shapes,positioning}
\tikzstyle{obs} = [circle,fill=white,draw=black,inner sep=1pt,minimum size=20pt,font=\fontsize{10}{10}\selectfont,node distance=1,thick]
\tikzstyle{latent} = [obs,dotted]
\tikzstyle{protected} = [obs,text=Orange,draw=Orange]
\tikzstyle{unfair} = [obs,text=BrickRed,draw=BrickRed]
\tikzstyle{target} = [obs,text=MidnightBlue,draw=MidnightBlue]
\tikzstyle{feature} = [obs,text=ForestGreen,draw=ForestGreen]

% Edge command from https://github.com/jluttine/tikz-bayesnet/blob/master/tikzlibrarybayesnet.code.tex
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1,thick] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% Header
\newcommand{\xhdr}[1]{\paragraph{#1.}}

\newcommand{\B}[1]{\mathbf{#1}}

% General math macros
\newcommand{\bR}{\ensuremath \mathbb{R}}
\newcommand{\bN}{\ensuremath \mathbb{N}}
\newcommand{\cG}{\ensuremath \mathcal{G}}
\newcommand{\cL}{\ensuremath \mathcal{L}}
\newcommand{\cF}{\ensuremath \mathcal{F}}
\newcommand{\cV}{\ensuremath \mathcal{V}}
\newcommand{\cE}{\ensuremath \mathcal{E}}
\newcommand{\cX}{\ensuremath \mathcal{X}}
\newcommand{\cY}{\ensuremath \mathcal{Y}}
\newcommand{\cZ}{\ensuremath \mathcal{Z}}
\newcommand{\cT}{\ensuremath \mathcal{T}}
\newcommand{\cN}{\ensuremath \mathcal{N}}
\newcommand{\cD}{\ensuremath \mathcal{D}}
\newcommand{\pa}{\ensuremath \mathrm{pa}}

\newcommand{\xb}{\ensuremath \B{x}}
\newcommand{\yb}{\ensuremath \B{y}}
\newcommand{\ab}{\ensuremath \B{a}}
\newcommand{\cb}{\ensuremath \B{c}}
\newcommand{\db}{\ensuremath \B{d}}
\newcommand{\zb}{\ensuremath \B{z}}
\newcommand{\qb}{\ensuremath \B{q}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\indep}{\perp\!\!\!\perp}
\DeclareMathOperator{\dep}{\not\! \perp\!\!\!\perp}
\newcommand{\usub}[2]{\underset{#1}{\underbrace{#2}}}
\newcommand{\given}{\,|\,}
\newcommand{\lhs}{\mathrm{LHS}}
\newcommand{\rhs}{\mathrm{RHS}}

\newcommand{\range}[2]{\{#1, \ldots, #2\}}
\newcommand{\paG}{\pa_{\cG}}
\newcommand\pfrac[2]{\frac{\partial #1}{\partial #2}}

% text surrounded by space
\newcommand{\qtxtq}[1]{\quad\text{#1}\quad}
\newcommand{\qqtxtqq}[1]{\qquad\text{#1}\qquad}

% Custom specifics
\DeclareMathOperator{\CFU}{\ensuremath \mathrm{CFU}}
\newcommand{\Yhat}{\ensuremath \hat{Y}}

% Comment commands
\newcommand{\nk}[1]{{\color{BrickRed}#1}}
\newcommand{\addref}{{\color{Orange}[ref]}}
\newcommand{\vlad}[1]{\textcolor{olive}{[VN:~#1]}}
\newcommand{\vale}[1]{\textcolor{green}{[VZ:~#1]}}
\newcommand{\matt}[1]{\textcolor{blue}{[MK:~#1]}}


% vlad's preferred look :)
\newcommand\hlf{\nicefrac{1}{2}}
\newcommand*{\eg}{\textit{e.g.}\@\xspace}
\newcommand*{\ie}{\textit{i.e.}\@\xspace}
\newcommand*{\wrt}{\textit{w.r.t.}\@\xspace}
\newcommand{\setto}{\stackrel{!}{=}}

% custom colors
%\definecolor{name}{HTML}{E0E0E0}
\definecolor{CRuby}{HTML}{D81159}
\definecolor{CMagenta}{HTML}{8F2D56}
\definecolor{CGreen}{HTML}{218380}
\definecolor{CYellow}{HTML}{FBB13C}
\definecolor{CBlue}{HTML}{73D2DE}


==> Learning Latent Decision Trees/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
%\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
%\let\ab\allowbreak


==> Learning Latent Decision Trees/sections/architecture.tex <==
\newsavebox{\miniz}
\savebox{\miniz}{
\begin{tikzpicture}[
  scale=1,
  every node/.style={inner sep=0pt, outer sep=0pt, draw,circle,minimum size=3pt},
  level 1/.style= {sibling distance=12pt},
  level 2/.style= {sibling distance=7pt},
  level distance=7pt
]
\node[fill=black] at (0, 0) {}
  child{node[fill=black!20] {}
    child{node[]{}}
    child{node[fill=black!20]{}}}
  child{node[fill=black!70] {}
    child{node[]{}}
    child{node[fill=black!70]{}}};
\end{tikzpicture}
}
%
\begin{tikzpicture}[scale=1]
\node at (1.4, 1.5) {(a)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$y$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{$\operatorname{Affine}([\xb;\zb])$} (y);
\end{tikzpicture}
%
\begin{tikzpicture}[scale=1]
\node at (1.4, 1.5) {(b)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$y$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{$\operatorname{MLP}([\xb;\zb])$} (y);
\end{tikzpicture}
%
\begin{tikzpicture}[scale=1]
\node at (1, 1.5) {(c)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2, 0) {$y$};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw[->] (z) -- node[above,font=\scriptsize] {$\operatorname{MLP}(\zb)$} (y);
\end{tikzpicture}




==> Learning Latent Decision Trees/sections/discussion.tex <==
% latent trees as efficient data structures
In this work we have presented a new optimization approach to learn trees for a variety of machine learning tasks. Our method works by sparsely relaxing a ILP for tree traversal and pruning, to enable simultaneous optimization of these parameters, alongside splitting parameters and downstream functions via argmin differentiation. Our approach nears or improves upon recent work in both supervised learning and hierarchical clustering. 
% future
We believe there are many exciting avenues for future work. One particularly interesting direction would be to unify recent advances in tight relaxations of nearest neighbor classifiers with this approach to learn efficient neighbor querying structures such as ball trees. Another idea is to adapt this method to learn instance-specific trees such as parse trees.


==> Learning Latent Decision Trees/sections/experiments.tex <==
In this section we showcase our method on both: (a) \emph{Classification/Regression} for tabular data, where tree-based models have been demonstrated to have superior performance over MLPs \citep{popov2019neural}; and (b) \emph{Hierarchical clustering} on unsupervised data. Our experiments demonstrate that our method leads to predictors that are competitive with state-of-the-art tree-based approaches, scaling better with the size of datasets and generalizing to many tasks.
% Given the derived exact solution for computing the path of each node through the
% tree $(\zb_i)$, our overall learning procedure learns the split function weights
% and the pruning parameters by backpropagation.
% As such, our tree induction can be integrated into deep neural networks for a
% variety of tasks and loss functions.
% In this section, we showcase this for two different tasks, namely supervised learning on tabular datasets and hierarchical clustering.
Further we visualize the trees learned by our method and how sparsity is easily adjusted by tuning the hyper-parameter $\lambda$.

\paragraph{Architecture details.}
We use a linear function or a multi-layer perceptron ($L$ fully-connected layers
with ELU activation~\citep{clevert2015fast} and dropout) for $f_\phi(\cdot)$ and
choose between linear or linear followed by ELU splitting functions $s_\theta(\cdot)$ (we limit
%these possibilities
the search for simplicity, there are no restrictions
%for these choices
except differentiability).

% These experiments are designed to show how our tree learning methodology can be flexibly adapted to different problem settings.

% can be adapted to distinctive problem settings,

% can be plugged into any model and even applied to raw inputs, yielding results comparable to state-of-the-art methods.


% TO ADD:
% We allow hyperparameter selection to decide on (a) $\lambda$; (b) the learning rate for solving eq.~\eqref{eq:obj}; (c) whether to use a linear function or a simple multi-layer perceptron for $f_\phi(\cdot)$; and (d) between linear or linear followed by an Elu activation \citep{clevert2015fast} splitting functions $s_\theta(\cdot)$ (we limit these possibilities for simplicity, there are no restrictions for these choices except differentiability).
%\begin{figure}[t!]
%\input{sections/architecture.tex}
%\caption{\label{fig:arch}Architecture \vlad{todo}.}
%\end{figure}
% Three settings /  model architectures:
% - [x; z] -> y (with skip connection) and linear predictor
% - [x; z] -> y (with skip connection) and MLP predictor
% - x -> z -> y (without skip connection) and MLP predictor


\subsection{Supervised Learning on Tabular Datasets}
\label{sec:tabular}
Our first set of experiments is on supervised learning with heterogeneous tabular datasets, where we consider both regression and binary classification tasks.
We minimize the Mean Square Error (MSE) on regression datasets and the Binary Cross-Entropy (BCE) on classification datasets.
% \paragraph{Baselines.}
We compare our results with tree-based architectures, which either train a single or an ensemble of decision trees.
Namely, we compare against the greedy CART algorithm  \citep{breiman1984classification} and two optimal decision tree learners:
OPTREE with local search~\citep[Optree-LS, ][]{dunn2018optimal} %, but upper bounding its tree depth.
and a state-of-the-art optimal tree method \citep[GOSDT, ][]{lin2020generalized}.
We also consider three baselines with probabilistic routing:
deep neural decision trees \citep[DNDT, ][]{yang2018deep},
% , which learns a decision tree with axis-aligned differentiable binning functions and soft routing;
deep neural decision forests~\citep{kontschieder2015deep} configured to jointly optimize the routing and the splits and to use an ensemble size of 1 (NDF-1), and adaptive neural networks~\citep[ANT, ][]{tanno2019adaptive}.
As for the ensemble baselines, we compare to NODE~\citep{popov2019neural}, the state-of-the-art method for training a forest of differentiable oblivious decision trees on tabular data, and to XGBoost~\citep{Chen:2016:XST:2939672.2939785}, a scalable tree boosting method.
% Similarly to our tree learning procedure, NODE's decision tree learning routine can be integrated in Deep Learning architectures and trained with back-propagation.
% As a downside, only oblivious trees can be trained and an ensemble of trees has to be built for good performance.
% \paragraph{Datasets.}
%
We carry out the experiments on the following datasets. %\citep{mldata}
%\begin{itemize}
%\item {\bf Year.} Regression task constructed from the Million Song Dataset
%\citep{msd,mldata}.
%\item {\bf Microsoft.}
%Regression approach to the MSLR-Web10k Query--URL relevance prediction for learning to rank \citep{mslr}.
%\item {\bf Yahoo.} Regression approach to the C14 learning-to-rank challenge. \vlad{check}
%\item {\bf Click.} Binary classification for link click prediction based on the KDD Cup 2012
%dataset, encoded and subsampled following \citet{popov2019neural}.
%\item {\bf Higgs.} Binary classification for predicting Higgs boson--producing
%events. \citep{higgs,mldata}
%\end{itemize}
\textbf{Regression:}
{\em Year} \citep{msd},
Temporal regression task constructed from the Million Song Dataset;
{\em Microsoft} \citep{mslr},
Regression approach to the MSLR-Web10k Query--URL relevance prediction for
learning to rank;
{\em Yahoo} \citep{chapelle2011yahoo}, Regression approach to the C14 learning-to-rank challenge.
\textbf{Binary classification:}
{\em Click}, Link click prediction based on the KDD Cup 2012
dataset, encoded and subsampled following \citet{popov2019neural};
{\em Higgs} \citep{higgs}, prediction of Higgs boson--producing
events.

\begin{table}[t!]
\caption{\label{tab:tabular-reg}%
Results on tabular regression datasets. We report average and standard deviations over $4$ runs of MSE and \textbf{bold} best results, and those within a standard deviation from it, for each family of algorithms (single tree or ensemble).
For the single tree methods we additionally report the average training times (s).}

\begin{center}
\scalebox{0.85}{
\begin{tabular}{clccc}
\hline
 &METHOD  & YEAR & MICROSOFT & YAHOO \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Single}}}
& CART & $96.0 \pm 0.4$ & $0.599 \pm 1\text{e-}3$ & $0.678 \pm 17\text{e-}3$\\
& ANT   & $\bm{77.8 \pm 0.6}$ & $\bm{0.572 \pm 2\text{e-}3}$ & $\bm{0.589 \pm 2\text{e-}3}$\\
& Ours    &$\bm{77.9\pm0.4}$ & $\bm{0.573\pm2\text{e-}3}$ & $\bm{0.591 \pm 1\text{e-}3}$  \\\hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
& NODE     &$\bm{76.2 \pm 0.1}$ & $0.557 \pm 1\text{e-}3$ & $0.569\pm1\text{e-}3$ \\
& XGBoost  &$78.5 \pm 0.1$ & $\bm{0.554 \pm 1\text{e-}3}$ & $\bm{0.542\pm1\text{e-}3}$\\\hline\hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Time}}}
& CART & $23$s & $20$s & $26$s \\
& ANT & $4674$s & $1457$s & $4155$s \\
& ours & $1354$s & $1117$s & $825$s \\ \hline
\end{tabular}}
\end{center}
% \vspace{-2ex}
\end{table}

For all tasks, we follow the preprocessing and task setup from
\citep{popov2019neural}.
%the preprocessed datasets are available at \vlad{TODO}.
All datasets come with training/test splits.
We make use of 20\% of the training set as validation set for selecting the best model over training and for tuning the hyperparameters.
We tune the hyperparameters for all methods.
% but for Optree, as its long training time makes hyper-parameter tuning unfeasible.
and optimize eq.~\eqref{eq:obj} and all neural network methods (DNDT, NDF, ANT and NODE) using the Quasi-Hyperbolic Adam~\citep{ma2018quasi} stochastic gradient descent method.
% , with default parameters and learning rate of $0.001$ and batch size equal to $512$.
Further details are provided in the supplementary.
Tables~\ref{tab:tabular-reg} and~\ref{tab:tabular-cls} report the obtained results on the regression and classification datasets respectively.\footnote{GOSDT/DNDT/Optree-LS/NDF are for classification only.}
Unsurprisingly, ensemble methods outperfom single-tree ones on all datasets, although at the cost of being harder to visualize/interpret.
Our method has the advantage of (a) generalizing to any task; (b) outperforming or matching all single-tree methods; (c) approaching the performance of ensemble-based methods; (d) scaling well with the size of datasets.
These experiments show that our model is also significantly faster to train, compared to its differentiable tree counterparts NDF-1 and ANT, while matching or beating the performance of these baselines, and it generally provides the best trade-off between time complexity and accuracy over all datasets (visualizations of this trade-off are reported in the supplementary material).
Further results on smaller datasets are available in the supplementary material to provide a comparison with optimal tree baselines.
%Among single-tree methods, ours has the advantage of generalizing to any task and having the best trade-off between prediction accuracy and training time (see Figures~\ref{fig:time-click} and~\ref{fig:time-higgs}).

\begin{table}
\caption{\label{tab:tabular-cls}%
Results on tabular classification datasets. We report average and standard deviations over $4$ runs of error rate. Best result for each family of algorithms (single tree or ensemble) are in \textbf{bold}.  Experiments are run on a machine with 16 CPUs and 64GB of RAM, with a training time limit of $3$ days. We denote methods that exceed this memory and training time as OOM and OOT, respectively.
For the single tree methods we additionally report the average training times (s) when available.}

\begin{center}
\scalebox{0.9}{
\begin{tabular}{clcc}
\hline
 &METHOD  & CLICK & HIGGS \\ \hline
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Single Tree}}}
& GOSDT   & OOM & OOM \\
& OPTREE-LS  & OOT & OOT\\
& DNDT    & $0.4866 \pm 1\text{e-}2$ & OOM\\
& NDF-1   & $0.3344 \pm 5\text{e-}4$ & $0.2644 \pm 8\text{e-}4$\\
& CART & $0.3426 \pm 11\text{e-}3$ & $0.3430\pm 8\text{e-}3$\\
& ANT     & $0.4035 \pm 0.1150$ & $0.2430 \pm 6\text{e-}3$\\
& Ours    & $\bm{0.3340 \pm 3\text{e-}4}$ & $\bm{0.2201\pm3\text{e-}4}$ \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
& NODE     & $\bm{0.3312 \pm 2\text{e-}3}$ & $\bm{0.210\pm5\text{e-}4}$ \\
& XGBoost  & $\bm{0.3310 \pm 2\text{e-}3}$ & $0.2334 \pm 1\text{e-}3$\\\hline\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Time}}}
& DNDT & $681$s & -\\
& NDF-1 & $3768$s & $43593$s \\
& CART & $3$s & $113$s\\
& ANT & $75600$s & $62335$s\\
& ours & $524$s & $18642$s \\ \hline
\end{tabular}}
\end{center}

\end{table}

\begin{figure*}

    \centering
    \includegraphics[width=\textwidth]{figures/pruning/pruned_all.pdf}
    \caption{\label{fig:pruning}%
{\em Glass} tree routing distribution, in rounded percent of dataset, for $\lambda$ left-to-right in $\{1, 10, 100\}$.
The larger $\lambda$, the more nodes are pruned.
We report dendrogram purity (DP) and represent the nodes by the percentage of
points traversing them (normalized at each depth level) and with a color
intensity depending on their $\ab_t$ (the darker the higher $\ab_t$). The empty nodes are labeled by a dash $-$ and the inactive nodes ($a_t \!=\! 0$) have been removed.
% \vspace{-1ex}
}
\end{figure*}

\subsection{Self-Supervised Hierarchical Clustering}\label{sec:clust}

\begin{table}
    \caption{\label{tab:clust}%
Results for hierarchical clustering. We report average and standard deviations of {\em dendrogram purity} over four runs.} %Best results are in bold.}
%        \vspace{1ex}
    \begin{center}\small
        \begin{tabular}{lcc}\hline
        METHOD  & GLASS & COVTYPE \\
        \hline
        Ours         & $0.468\pm0.028$ & $\mathbf{0.459\pm0.008}$ \\
        gHHC             &$0.463\pm0.002$ & $0.444\pm0.005$ \\
        HKMeans             &$\mathbf{0.508\pm0.008}$ & $0.440\pm0.001$ \\
        BIRCH             &$0.429\pm0.013$ & $0.440\pm0.002$ \\\hline
        \end{tabular}
    \end{center}
\end{table}

To show the versatility of our method, we carry out a second set of experiments on hierarchical clustering tasks. Inspired by the recent success of self-supervised learning approaches \citep{lan2019albert,he2020momentum}, we learn a tree for hierarchical clustering in a self-supervised way. Specifically, we regress a subset of input features from the remaining features, minimizing the MSE. This allows us to use eq.~\eqref{eq:obj} to learn a hierarchy (tree).
%This time, our method is trained in a self-supervised way, by regressing two of the available input features and minimizing the Mean Squared Error.
%Even though no supervision on the class labels is provided at training, we expect the constructed tree to group points of the same class in order to have good performance on the downstream task.
%\vlad{is there some paper we can cite for this way of doing self supervision?}
To evaluate the quality of the learned trees, we compute their dendrogram purity \citep[DP;][]{monath2019gradient}.
DP measures the ability of the learned tree to separate points from different classes, and corresponds to the expected purity of the least common ancestors of points of the same class.
%This score, however, does not account for the existing hierarchy between classes.
% For image data, we follow SimCLR's framework
% \citep{chen2020simple},
% with the LT block as encoder and a MLP as projection head,
% NT-Xent \citep{sohn,wu2018unsupervised,oord2018representation} as contrastive loss;
% \vlad{what specifically is spatial data? just ALOI? digits too?}
% \vale{just ALOI now, because the transformations proposed in SimCLR don't seem to work on DIGITS. for DIGITS, I am now regressing half of the image.}

We experiment on the following datasets: {\em Glass} \citep{mldata}:
glass identification for forensics, and {\em Covtype}
\citep{blackard1999comparative,mldata}: cartographic variables for forest cover
type identification.
%\begin{itemize}
%\item {\bf Glass.} Glass identification dataset for forensics \citep{mldata}.
%\item {\bf Covtype.} Cartographic variables for forest cover type prediction.
%\citep{blackard1999comparative,mldata}.
% \item {\bf ALOI.} Amsterdam Library of Object Images
% \citep{geusebroek2005amsterdam}.
% \item {\bf Digits.} NIST handwritten digit images
% \citep{alpaydin1998cascading,mldata}
%\end{itemize}
For {\em Glass}, we regress features `Refractive Index' and `Sodium,' and for
{\em Covtype} the horizontal and vertical `Distance To Hydrology.'
We split the datasets into training/validation/test sets, with sizes 60\%/20\%/20\%. Here we only consider linear $f_\phi$.
%For this set of experiments, the number of fully connected layers of the MLP predictor is set to $0$, resulting in a linear predictor.
As before, we optimize Problem~\ref{eq:obj} using the Quasi-Hyperbolic Adam
algorithm and tune the hyper-parameters using the validation reconstruction error.

As baselines, we consider:
BIRCH~\citep{zhang1997birch} and Hierarchical KMeans (HKMeans), the standard methods for performing clustering on large datasets; and the recently proposed gradient-based Hyperbolic Hierarchical Clustering \citep[gHHC, ][]{monath2019gradient} designed to construct  trees in hyperbolic space.
Table~\ref{tab:clust} reports the dendrogram purity scores for all methods. Our method yields results comparable to all baselines, even though not specifically tailored to hierarchical clustering.
%Even if our method is not specifically designed for hierarchical clustering problems, it achieves performance comparable or better than baselines.

% We further analyze the trees learned on {\em Glass} dataset with the proposed self-supervised procedure.
\paragraph{Tree Pruning}
The hyper-parameter $\lambda$ in Problem~\ref{eq:qp_prune} controls how aggressively the tree is pruned, hence the amount of tree splits that are actually used to make decisions.
This is a fundamental feature of our framework as it allows to smoothly trim the portions of the tree that are not necessary for the downstream task, resulting in lower computing and memory demands at inference. % as the tree representation, and the model in general, can be compressed.
In Figure~\ref{fig:pruning}, we study the effects of pruning on the tree learned on {\em Glass} with a depth fixed to $D \!=\! 4$.
We report how inputs are distributed over the learned tree for different values of $\lambda$.
We notice that increasing $\lambda$ effectively prune nodes and entire portions of the tree, without significantly impact performance (as measured by dendrogram purity).
% We notice that the number of empty nodes, \ie, nodes that are not traversed by any data point, increases together with $\lambda$ up to a certain value in order not to significantly deteriorate results (as measured by dendrogram purity).
%Moreover, even without the regularization term ($\lambda=0$), our method removes nodes that have few points assigned to them. % adding the pruning regularization effectively removes those nodes that have few assigned points when $\lambda=0$.

To look into the evolution of pruning during training, we further plot the \% of active (unpruned) nodes within a training epoch in Figure~\ref{fig:epoch-an}.
We observe that (a) it appears possible to increase and decrease this fraction through training (b) the fraction seems to stabilize in the range $45\%$-$55\%$ after a few epochs.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/GLASS-reg=10.pdf}
    \caption{Percentage of active nodes during training as a function of the number of epochs on {\em Glass}, $D \!=\! 6, \lambda\!=\!10$.}
    \label{fig:epoch-an}
\end{figure}

\paragraph{Class Routing}
To gain insights on the latent structure learned by our method, we study how points are routed through the tree, depending on their class.
The {\em Glass} dataset is particularly interesting to analyze as its classes come with an intrinsic hierarchy, \eg, with superclasses \textit{Window} and \textit{NonWindow}.
%Still, we expect points from the same class or super class to traverse the tree in a similar way.
Figure~\ref{fig:class-routing} reports the class routes for four classes.
As the trees are constructed without supervision, we do not expect the structure to exactly reflect the class partition and hierarchy. Still, we observe that points from the same class or super-class traverse the tree in a similar way.
Indeed, trees for class \textit{Build}~\ref{fig:build}
and class \textit{Vehicle}~\ref{fig:vehicle} that both belong to the \textit{Window} super-class, share similar paths, unlike the classes Containers~\ref{fig:cont}
and Headlamps~\ref{fig:head}.

\begin{figure}[t!]
    \centering
    \subfigure[Window-Float-Build]{\label{fig:build}\includegraphics[width=0.24\textwidth]{figures/glass/class0.pdf}}\hfill
    \subfigure[Window-Float-Vehicle]{\label{fig:vehicle}\includegraphics[width=0.24\textwidth]{figures/glass/class2.pdf}}\hfill
    \subfigure[NonW-Containers]{\label{fig:cont}\includegraphics[width=0.24\textwidth]{figures/glass/class4.pdf}}\hfill
    \subfigure[NonW-Headlamps]{\label{fig:head}\includegraphics[width=0.24\textwidth]{figures/glass/class6.pdf}}
    % \includegraphics[width=\textwidth]{figures/glass/hier_clustering.pdf}
    \caption{\label{fig:class-routing}%
Class routing distributions on {\em Glass}, with distributions normalized over each depth level. Trees were trained with optimal hyper-parameters (depth $D\!=\!5$), but we plot nodes up to $D\!=\!3$ for visualization ease. Empty nodes are labeled by a dash $-$.
    }
\end{figure}



% tabular datasets
% hierarchical clustering
%   - linear splits
%   - contrastive learning images


==> Learning Latent Decision Trees/sections/experiments_arxiv.tex <==
\begin{wrapfigure}[10]{R}{.3\textwidth}
\input{sections/fig_intro.tex}
\caption{\label{fig:arch}Model overview.}

\end{wrapfigure}
In this section we showcase our method on both: (a) \emph{Classification/Regression} for tabular data, where tree-based models have been demonstrated to have superior performance over MLPs \citep{popov2019neural}; and (b) \emph{Hierarchical clustering} on unsupervised data. Our experiments demonstrate that our method leads to predictors that are competitive with state-of-the-art tree-based approaches. 
% Given the derived exact solution for computing the path of each node through the
% tree $(\zb_i)$, our overall learning procedure learns the split function weights
% and the pruning parameters by backpropagation.
% As such, our tree induction can be integrated into deep neural networks for a
% variety of tasks and loss functions.
% In this section, we showcase this for two different tasks, namely supervised learning on tabular datasets and hierarchical clustering.
Further we visualize the trees learned by our method, and how sparsity is easily adjusted by tuning the regularization parameter $\lambda$. 

\paragraph{Architecture details.} 
We use a linear function or a multi-layer perceptron ($L$ fully-connected layers with Elu activation~\citep{clevert2015fast} and dropout) for $f_\phi(\cdot)$ and choose between linear or linear followed by Elu splitting functions $s_\theta(\cdot)$ (we limit 
%these possibilities 
the search for simplicity, there are no restrictions 
%for these choices 
except differentiability).

% These experiments are designed to show how our tree learning methodology can be flexibly adapted to different problem settings. 

% can be adapted to distinctive problem settings, 

% can be plugged into any model and even applied to raw inputs, yielding results comparable to state-of-the-art methods.


% TO ADD:
% We allow hyperparameter selection to decide on (a) $\lambda$; (b) the learning rate for solving eq.~\eqref{eq:obj}; (c) whether to use a linear function or a simple multi-layer perceptron for $f_\phi(\cdot)$; and (d) between linear or linear followed by an Elu activation \citep{clevert2015fast} splitting functions $s_\theta(\cdot)$ (we limit these possibilities for simplicity, there are no restrictions for these choices except differentiability).
%\begin{figure}[t!]
%\input{sections/architecture.tex}
%\caption{\label{fig:arch}Architecture \vlad{todo}.}
%\end{figure}
% Three settings /  model architectures:
% - [x; z] -> y (with skip connection) and linear predictor
% - [x; z] -> y (with skip connection) and MLP predictor
% - x -> z -> y (without skip connection) and MLP predictor


\subsection{Supervised Learning on Tabular Datasets}
Our first set of experiments is on supervised learning with heterogeneous tabular datasets, where we consider both regression and binary classification tasks.
We minimize the Mean Squared Error (MSE) on regression datasets and the Binary Cross-Entropy (BCE) on classification datasets.
% \paragraph{Baselines.}
We compare our results with tree-based architectures, which either train a single or an ensemble of decision trees.
Namely, we compare to the greedy classification and regression trees (CART)~\citep{breiman1984classification} and to the optimal decision tree learner~\citep[OPTREE;][]{bertsimas2017optimal}. %, but upper bounding its tree depth.
We also consider two baselines with probabilistic routing:
deep neural decision trees \citep[DNDT;][]{yang2018deep}
% , which learns a decision tree with axis-aligned differentiable binning functions and soft routing;
and deep neural decision forests~\citep{kontschieder2015deep} configured to use an ensemble size of 1 (NDF-1).
As for the ensemble baselines, we compare to NODE~\citep{popov2019neural}, the state-of-the-art method for training a forest of differentiable oblivious decision trees on tabular data, and to XGBoost~\citep{Chen:2016:XST:2939672.2939785}, a scalable tree boosting method.
% Similarly to our tree learning procedure, NODE's decision tree learning routine can be integrated in Deep Learning architectures and trained with back-propagation.
% As a downside, only oblivious trees can be trained and an ensemble of trees has to be built for good performance.
% \paragraph{Datasets.}
%
We carry out the experiments on the following datasets: \citep{mldata}
%\begin{itemize}
%\item {\bf Year.} Regression task constructed from the Million Song Dataset
%\citep{msd,mldata}.
%\item {\bf Microsoft.}
%Regression approach to the MSLR-Web10k Query--URL relevance prediction for learning to rank \citep{mslr}.
%\item {\bf Yahoo.} Regression approach to the C14 learning-to-rank challenge. \vlad{check}
%\item {\bf Click.} Binary classification for link click prediction based on the KDD Cup 2012
%dataset, encoded and subsampled following \citet{popov2019neural}.
%\item {\bf Higgs.} Binary classification for predicting Higgs boson--producing
%events. \citep{higgs,mldata}
%\end{itemize}
\textbf{Regression.}
{\em Year} \citep{msd}:
Temporal regression task constructed from the Million Song Dataset;
{\em Microsoft} \citep{mslr}:
Regression approach to the MSLR-Web10k Query--URL relevance prediction for
learning to rank;
{\em Yahoo} \citep{chapelle2011yahoo}: Regression approach to the C14 learning-to-rank challenge.
\textbf{Binary classification.}
{\em Click}: Link click prediction based on the KDD Cup 2012
dataset, encoded and subsampled following \citet{popov2019neural};
{\em Higgs} \citep{higgs}: prediction of Higgs boson--producing
events.

For all tasks, we follow the preprocessing and task setup from
\citep{popov2019neural}.
%the preprocessed datasets are available at \vlad{TODO}.
All datasets come with training/test splits.
We make use of 20\% of the training set as validation set for selecting the best model over the epochs and for tuning the hyperparameters.
We tune the hyperparameters for all methods but for OPTREE, as its long training time makes hyper-parameter tuning unfeasible. Details are provided in the supplementary.
Finally, we optimize eq.~\eqref{eq:obj} and all neural network methods (DNDT, NDF, and NODE) using the Quasi-Hyperbolic Adam~\citep{ma2018quasi} stochastic gradient descent method, with default parameters and batch size equal to $512$.
Table~\ref{tab:tabular} reports the obtained results.\footnote{DNDT, OPTREE and NDF handle only classification tasks.} 
Unsurprisingly, ensemble methods outperfom single-tree ones on all datasets, although at the cost of being harder to visualize/interpret. 
Our method has the advantage of (a) generalizing to any task; (b) outperforming or coming in second for all single-tree methods; (c) approaching the performance of ensemble-based methods.
%Among single-tree methods, ours has the advantage of generalizing to any task and having the best trade-off between prediction accuracy and training time (see Figures~\ref{fig:time-click} and~\ref{fig:time-higgs}).

% \begin{table}
% 	\begin{minipage}{0.7\linewidth}
% 		\label{tab:clust}
%         \caption{Results for hierarchical clustering. We report average and standard deviations of Dendrogram Purity over $4$ runs. Best results and all within a standard deviation from it are in bold.
%         % \vlad{make sure to explain what bold means}
%         }
%         \vspace{1ex}
%         \begin{center}
%             % \begin{tabular}{lcc}
%             % {\bf METHOD}  &{\bf GLASS} &{\bf COVTYPE} \\
%             % \hline \\
%             % Ours         & $\mathbf{0.494\pm0.025}$ & $\mathbf{0.467\pm0.006}$ \\
%             % gHHC             &$0.463\pm0.002$ & $0.444\pm0.005$ \\
%             % HKMeans             &$\mathbf{0.508\pm0.008}$ & $0.440\pm0.001$ \\
%             % BIRCH             &$0.429\pm0.013$ & $0.440\pm0.002$ \\
%             % \end{tabular}
%             \begin{tabular}{clccc}
%  & method  &{\bf YEAR} &{\bf MICROSOFT} &{\bf YAHOO} \\
%  \hline \\
% \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Single Tree}}}
% & CART & $97.40 \pm 0.37$ & $0.6914 \pm 3\text{e-}3$ & $0.6190 \pm 3\text{e-}3$ \\
% & DNDT    & - & - & - & $0.4866 \pm 1\text{e-}2$ & OOM\\
% & OPTREE  & - & - & - & $0.4100 \pm 4\text{e-}2$ & OOT\\
% & NDF-1   & - & - & - & $\bm{0.3344 \pm 5\text{e-}4}$ & $\bm{0.2644 \pm 8\text{e-}4}$\\
% & Ours    &$\bm{77.52\pm0.50}$ & $\bm{0.5772\pm12\text{e-}4}$ & $\bm{0.5937 \pm 6\text{e-}4}$ & $0.3383 \pm 15\text{e-}4$ & $0.2995\pm16\text{e-}4$\\
% \hline \\
% \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
% & NODE     &$\bm{76.21 \pm 0.12}$ & $0.5570 \pm 2\text{e-}4$ & $0.5692\pm2\text{e-}4$ & $\bm{0.3312 \pm 2\text{e-}3}$ & $\bm{0.2101\pm5\text{e-}4}$ \\
% & XGBoost  &$78.53 \pm 0.09$ & $\bm{0.5544 \pm 1\text{e-}4}$ & $\bm{0.5420\pm4\text{e-}4}$ & $\bm{0.3310 \pm 2\text{e-}3}$ & $0.2328 \pm 3\text{e-}4$\\
% \end{tabular}
%         \end{center}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.3\linewidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{figures/pruning/all-reg.pdf}
%         \vspace{-3ex}
%         \captionof{figure}{Number of empty nodes (EN) as a function of $\lambda$.}
%         \label{fig:lambda}
% 	\end{minipage}
% \end{table}

\begin{table}[t]
\caption{Results on tabular datasets. We report average and standard deviations over $4$ runs of MSE for regression datasets: {\em Year}, {\em Microsoft} and {\em Yahoo}, and error rate for classification datasets: {\em Click} and {\em Higgs}. Best result, and those within a standard deviation from it, for each family of algorithms (single tree or ensemble) are in \textbf{bold}. Dashes `-' indicate that the method cannot be run (i.e., a method is designed only for classification). Experiments are run on a machine with 16 CPUs and 63GB of RAM, with a training time limit of $3$ days. We denote methods that exceed this memory and training time as OOM and OOT, respectively.}
\label{tab:tabular}
\begin{center}
\begin{tabular}{clccccc}
 &{\bf METHOD}  &{\bf YEAR} &{\bf MICROSOFT} &{\bf YAHOO} &{\bf CLICK} &{\bf HIGGS}\\
 \hline \\
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Single Tree}}}
& CART & $97.40 \pm 0.37$ & $0.6914 \pm 3\text{e-}3$ & $0.6190 \pm 3\text{e-}3$ & $0.3780 \pm 6\text{e-}3$ & $0.3220 \pm 1\text{e-}3$\\
& DNDT    & - & - & - & $0.4866 \pm 1\text{e-}2$ & OOM\\
& OPTREE  & - & - & - & $0.4100 \pm 4\text{e-}2$ & OOT\\
& NDF-1   & - & - & - & $\bm{0.3344 \pm 5\text{e-}4}$ & $\bm{0.2644 \pm 8\text{e-}4}$\\
& Ours    &$\bm{77.52\pm0.50}$ & $\bm{0.5772\pm12\text{e-}4}$ & $\bm{0.5937 \pm 6\text{e-}4}$ & $0.3383 \pm 15\text{e-}4$ & $0.2995\pm16\text{e-}4$\\
\hline \\
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
& NODE     &$\bm{76.21 \pm 0.12}$ & $0.5570 \pm 2\text{e-}4$ & $0.5692\pm2\text{e-}4$ & $\bm{0.3312 \pm 2\text{e-}3}$ & $\bm{0.2101\pm5\text{e-}4}$ \\
& XGBoost  &$78.53 \pm 0.09$ & $\bm{0.5544 \pm 1\text{e-}4}$ & $\bm{0.5420\pm4\text{e-}4}$ & $\bm{0.3310 \pm 2\text{e-}3}$ & $0.2328 \pm 3\text{e-}4$\\
\end{tabular}
\end{center}
\end{table}

\subsection{Self-Supervised Hierarchical Clustering}\label{sec:clust}
To show the versatility of our method, we carry out a second set of experiments on hierarchical clustering tasks. Inspired by the recent success of self-supervised learning approaches \citep{lan2019albert,he2020momentum}, we learn a tree for hierarchical clustering in a self-supervised way. Specifically, we regress a subset of input features from the remaining features, minimizing the MSE. This allows us to use eq.~\eqref{eq:obj} to learn a hierarchy (tree). 
%This time, our method is trained in a self-supervised way, by regressing two of the available input features and minimizing the Mean Squared Error.
%Even though no supervision on the class labels is provided at training, we expect the constructed tree to group points of the same class in order to have good performance on the downstream task.
%\vlad{is there some paper we can cite for this way of doing self supervision?}
To evaluate the quality of the learned trees, we compute its dendrogram purity \citep[DP;][]{monath2019gradient}.
DP measures the ability of the learned tree to separate points from different classes, and corresponds to the expected purity of the least common ancestors of points of the same class.
%This score, however, does not account for the existing hierarchy between classes.
% For image data, we follow SimCLR's framework
% \citep{chen2020simple},
% with the LT block as encoder and a MLP as projection head,
% NT-Xent \citep{sohn,wu2018unsupervised,oord2018representation} as contrastive loss;
% \vlad{what specifically is spatial data? just ALOI? digits too?}
% \vale{just ALOI now, because the transformations proposed in SimCLR don't seem to work on DIGITS. for DIGITS, I am now regressing half of the image.}

We experiment on the following datasets: {\em Glass} \citep{mldata}:
glass identification for forensics, and {\em Covtype}
\citep{blackard1999comparative,mldata}: cartographic variables for forest cover
type identification.
%\begin{itemize}
%\item {\bf Glass.} Glass identification dataset for forensics \citep{mldata}.
%\item {\bf Covtype.} Cartographic variables for forest cover type prediction.
%\citep{blackard1999comparative,mldata}.
% \item {\bf ALOI.} Amsterdam Library of Object Images
% \citep{geusebroek2005amsterdam}.
% \item {\bf Digits.} NIST handwritten digit images
% \citep{alpaydin1998cascading,mldata}
%\end{itemize}
For {\em Glass}, we regress features `Refractive Index' and `Sodium,' and for
{\em Covtype} the horizontal and vertical `Distance To Hydrology.'
We split the datasets into training/validation/test sets, with sizes 60\%/20\%/20\%. Here we only consider linear $f_\phi$. 
%For this set of experiments, the number of fully connected layers of the MLP predictor is set to $0$, resulting in a linear predictor.
As before, we optimize Problem~\ref{eq:obj} using the Quasi-Hyperbolic Adam
algorithm, with batch size equal to $512$ for {\em Covtype} and $8$ for {\em Glass}, and tune the hyper-parameters using the validation set.

As baselines, we consider:
BIRCH~\citep{zhang1996birch} and Hierarchical KMeans (HKMeans), the standard methods for performing clustering on large datasets; and the recently proposed gradient-based Hyperbolic Hierarchical Clustering (gHHC)~\citep{monath2019gradient} designed to construct  trees in hyperbolic space.
Table~\ref{tab:clust} reports the dendrogram purity scores for all methods. Our method matches or outperforms all methods, even though not specifically tailored to hierarchical clustering.
%Even if our method is not specifically designed for hierarchical clustering problems, it achieves performance comparable or better than baselines.
\begin{table}
\caption{Results for hierarchical clustering. We report average and standard deviations of {\em dendrogram purity} over four runs. Best results and all within a standard deviation from it are in bold.}
%        \vspace{1ex}
\begin{center}
    \begin{tabular}{lcc}
    {\bf METHOD}  &{\bf GLASS} &{\bf COVTYPE} \\
    \hline \\
    Ours         & $\mathbf{0.494\pm0.025}$ & $\mathbf{0.467\pm0.006}$ \\
    gHHC             &$0.463\pm0.002$ & $0.444\pm0.005$ \\
    HKMeans             &$\mathbf{0.508\pm0.008}$ & $0.440\pm0.001$ \\
    BIRCH             &$0.429\pm0.013$ & $0.440\pm0.002$ \\
    \end{tabular}
\end{center}
\label{tab:clust}
\end{table}

% We further analyze the trees learned on {\em Glass} dataset with the proposed self-supervised procedure.
\paragraph{Tree Pruning}
The hyper-parameter $\lambda$ in eq.~\ref{eq:obj} controls how aggressively the tree is pruned, hence the amount of tree splits that are actually used to make decisions.
This is a fundamental feature of our framework as it allows to smoothly trim the portions of the tree that are not necessary for the downstream task, resulting in lower computing and memory demands at inference. % as the tree representation, and the model in general, can be compressed.
In Figure~\ref{fig:pruning}, we study the effects of pruning on the tree learned on {\em Glass} with a depth fixed to $D \!=\! 3$.
We report how inputs are distributed over the learned tree for different values of $\lambda$.
We notice that the number of empty nodes, \ie, nodes that are not traversed by any data point, increases together with $\lambda$ up to a certain value in order not to significantly deteriorate results (as measured by dendrogram purity).
%Moreover, even without the regularization term ($\lambda=0$), our method removes nodes that have few points assigned to them. % adding the pruning regularization effectively removes those nodes that have few assigned points when $\lambda=0$.

\begin{figure}
    \centering
    \includegraphics[width=.9\textwidth]{figures/pruning/pruned_all.pdf}
    \caption{{\em Glass} tree routing distribution, in rounded percent of dataset,
for $\lambda$ left-to-right in $\{0, 0.001, 0.1\}$.
The larger $\lambda$, the more nodes are pruned.
We report dendrogram purity (DP) and total empty nodes (EN).
\label{fig:pruning}}
\end{figure}

\paragraph{Class Routing}
In order to gain insights on the latent structure learned by our method, we study how points are routed through the tree, depending on their class.
The {\em Glass} dataset is particularly interesting to analyze as its classes come with an intrinsic hierarchy, \eg, with superclasses \textit{Window} and \textit{NonWindow}.
%Still, we expect points from the same class or super class to traverse the tree in a similar way.
Figure~\ref{fig:class-routing} reports the class routes for four classes.
As the trees are constructed without supervision, we do not expect the structure to exactly reflect the class partition and hierarchy. Still, we observe that points from the same class or super-class to traverse the tree in a similar way.
Indeed, trees for class \textit{Build}~\ref{fig:build} 
and class \textit{Vehicle}~\ref{fig:vehicle}, which both belong to \textit{Window} super-class, share similar paths, unlike the classes Containers~\ref{fig:cont} 
and Headlamps~\ref{fig:head}.

\begin{figure}
    \centering
    \subfigure[Window-Float-Build]{\label{fig:build}\includegraphics[width=0.4\textwidth]{figures/glass/class0.pdf}}\hfill
    \subfigure[Window-Float-Vehicle]{\label{fig:vehicle}\includegraphics[width=0.4\textwidth]{figures/glass/class2.pdf}}\hfill
    \subfigure[NonW-Containers]{\label{fig:cont}\includegraphics[width=0.4\textwidth]{figures/glass/class4.pdf}}\hfill
    \subfigure[NonW-Headlamps]{\label{fig:head}\includegraphics[width=0.4\textwidth]{figures/glass/class6.pdf}}
    % \includegraphics[width=\textwidth]{figures/glass/hier_clustering.pdf}
    \caption{Class routing distributions on {\em Glass}, with distributions normalized over each depth level. The decision tree was trained with optimal hyper-parameters, (depth $D\!=\!6$), but we plot nodes up to level $D\!=\!4$ for visualization ease.
    }
    \label{fig:class-routing}
\end{figure}



% tabular datasets
% hierarchical clustering
%   - linear splits
%   - contrastive learning images


==> Learning Latent Decision Trees/sections/fig_intro.tex <==
\newsavebox{\miniz}
\savebox{\miniz}{
\begin{tikzpicture}[
  scale=1,
  every node/.style={inner sep=0pt, outer sep=0pt, draw,circle,minimum size=3pt},
  level 1/.style= {sibling distance=12pt},
  level 2/.style= {sibling distance=7pt},
  level distance=7pt
]
\node[fill=black] at (0, 0) {}
  child{node[fill=black!20] {}
    child{node[]{}}
    child{node[fill=black!20]{}}}
  child{node[fill=black!70] {}
    child{node[]{}}
    child{node[fill=black!70]{}}};
\end{tikzpicture}
}
%
\begin{tikzpicture}[scale=.86]
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$\ell$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1.2, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathrm{T}_{\lambda}\big(q_{\bm{\theta}}(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw[dashed] (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{${f}_{\bm{\phi}}(\xb,\zb)$} (y);
\end{tikzpicture}


==> Learning Latent Decision Trees/sections/fig_z.tex <==
\tikzstyle{zir} = [CGreen, ultra thick]
\tikzstyle{zil} = [CMagenta, ultra thick, dashed]
\begin{tikzpicture}[scale = 0.75]
  \draw[->] (-2, 0) -- (2.6, 0) node[below] {\small $s_{\theta_t}(x_i)$};
  \draw[->] (0, -0.2) -- (0, 1.7);
  \foreach \x in {-1.5,-1,...,1.5}
 	\draw (\x,1pt) -- (\x,-1pt)
	node[anchor=north] {\scriptsize \x};
  \foreach \y in {0.5,1}
 	\draw (1pt,\y) -- (-1pt,\y) 
 		node[anchor=east] {\scriptsize \y}; 
 \draw[domain=-2:0, variable=\x,zir] plot ({\x}, {0});
  \draw[domain=0:2, variable=\x,zir] plot ({\x}, {1}) node[above] {$z_{ir}$};
  \draw[domain=-2:0, variable=\x,zil] plot ({\x}, {1});
  \draw[domain=0:2, variable=\x, zil] plot ({\x}, {0}) node[above] {$z_{il}$};
%   \draw[domain=-2:3, variable=\x, red, ultra thick] plot ({\x}, {left(\x)}) node[above] {$z_{il}$};
\end{tikzpicture}
\hfill
\begin{tikzpicture}[scale = 0.75]
  \draw[->] (-2, 0) -- (2.6, 0) node[below] {\small $s_{\theta_t}(x_i)$};
  \draw[->] (0, -0.2) -- (0, 1.7);
  \foreach \x in {-1.5,-1,...,1.5}
 	\draw (\x,1pt) -- (\x,-1pt)
	node[anchor=north] {\scriptsize \x};
  \foreach \y in {0.5,1}
 	\draw (1pt,\y) -- (-1pt,\y) 
 		node[anchor=east] {\scriptsize \y}; 
 \draw[domain=-2:-0.5, variable=\x, zir] plot ({\x}, {0});
 \draw[domain=-0.5:0.5, variable=\x, zir] plot ({\x}, {\x + 0.5});
  \draw[domain=0.5:2, variable=\x, zir] plot ({\x}, {1}) node[above] {$z_{ir}$};
  \draw[domain=-2:-0.5, variable=\x, zil] plot ({\x}, {1});
 \draw[domain=-0.5:0.5, variable=\x, zil] plot ({\x}, {-\x + 0.5});
  \draw[domain=0.5:2, variable=\x, zil] plot ({\x}, {0}) node[above] {$z_{il}$};
%   \draw[domain=-2:3, variable=\x, red, ultra thick] plot ({\x}, {left(\x)}) node[above] {$z_{il}$};
\end{tikzpicture}

==> Learning Latent Decision Trees/sections/introduction.tex <==
% latent structure is important for many problems
Learning discrete structures from unstructured data is extremely useful for a wide variety of real-world problems \citep{gilmer2017neural,kool2018attention,yang2018deep}.
% one of the most flexible representations is via trees
One of the most computationally-efficient, easily-visualizable discrete structures that are able to represent complex functions are \emph{binary trees}. For this reason, there has been a massive research effort on how to learn such binary trees since the early days of machine learning \citep{payne1977algorithm,breiman1984classification,bennett1992decision,bennett1996optimal}.
% optimization has gone three directions:
%   1. greedy optimization;
%   2. relax hard decisions of tree, optimize with gradient-based techniques;
%   3. used mixed-integer programming to find an optimal tree
Learning binary trees has historically been done in one of three ways.
The first is via \emph{greedy optimization}, which includes popular decision-tree methods such as classification and regression trees
\citep[CART, ][]{breiman1984classification} and ID3 trees \citep{quinlan1986induction}, among many others. These methods optimize a splitting criterion for each tree node, based on the data routed to it.
The second set of approaches are based on \emph{probabilistic
relaxations}~\citep{irsoy2012soft,yang2018deep,DBLP:conf/icml/0001PMTM20},
optimizing all splitting parameters at once via gradient-based methods, by relaxing hard branching decisions into branching probabilities.
The third approach optimizes trees using \emph{mixed-integer programming} \citep[MIP, ][]{bennett1992decision,bennett1996optimal}. This jointly optimizes all continuous and discrete parameters to find globally-optimal trees.\footnote{Here we focus on learning single trees instead of tree ensembles; our work easily extends to ensembles.}


% they each have their own downside:
%   1. very suboptimal: tree splits often don't optimize the same loss that we want the full tree to minimize
%   2. we lose nice properties such as:
%       - interpretability
%       - computational speed
%       if we try to gain them back we need to approximate which could harm optimality
%   3. no generalization guarantees, we forgoe the guarantees of convexity or stochastic optimization; also specific to quadratic/convex losses

\begin{figure}[t!]
    \centering
    {\includegraphics[width=\columnwidth]{figures/overall.pdf}
    }
    \caption{A schematic of the approach.}
    \label{fig:overall}
    %$n$ takes values in a range that covers common choices of batch size. Time and $n$ axis are represented in logarithmic scale.}
    %\label{fig:alg-time}
%         \includegraphics[width=0.99\textwidth]{figures/pruning/all-reg.pdf}
% %        \vspace{-3ex}
%         \captionof{figure}{Empty nodes (EN) as we vary $\lambda$.}
        %\label{fig:lambda}
\end{figure}

Each of these approaches has their shortcomings. First, greedy optimization is
generally suboptimal: tree splitting criteria are even intentionally crafted to be different than the global tree loss, as the global loss may not encourage tree growth \citep{breiman1984classification}. Second, probabilistic relaxations: (a) are rarely sparse, so inputs contribute to all branches even if they are projected to hard splits after training; (b) they do not have principled ways to prune trees, as the distribution over pruned trees is often intractable. Third, MIP approaches, while optimal, are only computationally tractable on training datasets with thousands of inputs \citep{bertsimas2017optimal}, and do not have well-understood out-of-sample generalization guarantees.

% our approach
% - sparse relaxation + argmin diff
% - insight:
%   - set up an MIP to learn input traversal + pruning
%   - tightly relax using quadratic regularization
%   - this results in an optimization problem that is continuous and differentiable almost everywhere
%   - learn continuous parameters through this

In this paper we present an approach to binary tree learning based on sparse relaxation and argmin differentiation (as depicted in Figure~\ref{fig:overall}).
Our main insight is that by quadratically relaxing an MIP that learns the discrete parameters of the tree (input traversal and node pruning), we can differentiate through it to simultaneously learn the continuous parameters of splitting decisions. This allows us to leverage the superior generalization capabilities of stochastic gradient optimization to learn decision splits, and gives a principled approach to learning tree pruning.
Further, we derive customized algorithms to compute the forward and backward passes through this program that are much more efficient than generic approaches \citep{optnet,cvxpylayers2019}.
The resulting learning method %generalizes to a variety of tasks
% (here we study its performance on supervised classification/regression and on self-supervised hierarchical clustering),
can learn trees with any differentiable splitting functions to minimize any differentiable loss, both tailored to the data at hand. %(e.g. convolutional for processing images).
% We demonstrate that (a) in classification/regression our method,
% which learns a single tree and a classifier on top of it, is competitive with greedy, probabilistic, MIP-based tree methods, and even powerful ensemble methods;
% (b) in hierarchical clustering we match or improve upon the state-of-the-art.

\paragraph{Notation.} We denote scalars, vectors, and sets, as $x$, $\xb$,
and $\mathcal{X}$, respectively.
A binary tree is a set $\mathcal{T}$ containing nodes $t \in \mathcal{T}$
with the additional structure that each node has at most one left child and at
most one right child, and each node except the unique root has exactly one
parent.
We denote the $l_2$ norm of a vector by $\|\xb\| \coloneqq\left(\sum_i
x_i^2\right)^{\frac{1}{2}}$. The unique projection of point $\xb \in \mathbb{R}^d$ onto a convex set $C \subset
\mathbb{R}^d$ is $\operatorname{Proj}_{C}(\xb) \coloneqq \argmin_{\yb \in C} \|\yb - \xb\|$.
In particular, projection onto an interval is given by
$\operatorname{Proj}_{[a, b]}(x) = \max(a, \min(b, x))$.
%and
%equiped with a parent-child relationship denoted as $p(t) = s$ if $s$ is the
%parent of node $t$. (Each non-root node has exactly one parent, and each node
%is a parent of at most two nodes.)


==> Learning Latent Decision Trees/sections/methods.tex <==
Given inputs $\{\xb_i \in \mathcal{X} \}_{i=1}^n$,  %where each $\xb \in [0,1]^p$.
our goal is to learn a latent binary decision tree $\cT$ with maximum depth $D$. This tree sends each input $\xb$ through branching nodes to a specific leaf node  in the tree. Specifically, all branching nodes $\cT_B \subset \cT$ split an input $\xb$ by forcing it to go to its left child if
$s_\theta(\xb) < 0$,
and right otherwise. There are three key parts of the tree that need to be
identified: 1. The \emph{continuous} parameters $\theta_t \in \mathbb{R}^d$ that
describe how $s_{\theta_t}(.)$ splits inputs at every node $t$; 2. The
\emph{discrete} paths $\zb$ made by each input $\xb$ through the tree; 3. The
\emph{discrete} choice $a_t$ of whether a node $t$ should be active or pruned,
i.e. inputs should reach/traverse it or not. We next describe how to represent each of these.
% Our strategy will be to first fix splitting parameters $\theta_t$ for all $t$. Then to introduce a mixed-integer program (MIP) for learning paths $\zb$ and pruning $d_t$. %We then modify this to a mixed-integer program (MIP) that solves both 2 and 3.
% Finally we sparsely relax the MIP to allow for argmin differentiation to simultaneously solve for $\theta_t$.

% Our goal is to learn $\cT$ that is good for some downstream task. To do so,
% %by learning a scoring vector $\{ \boldsymbol{\eta} \}_{i=1}^n$ where $\boldsymbol{\eta} \in \mathbb{R}^T$ that describes the benefit of sending $\xb_i$ along a particular route in the tree.
% we will learn the splitting parameters of the tree $\{ \theta_t,\}_{t \in \cT_B}$.
% % For these parameters we impose the following constrain
% % \begin{align}
% %     \sum_{j=1}^d a_{jt} = 1, \;\;\; 0 \leq \ab_t, b_t \leq 1,
% %     \;\;\; \forall t \in \cT_B. \nonumber
% % \end{align}
% Specifically, let $\cT$ have maximum depth $D$. %This tree has at most $T \!=\! 2^{(D+1)} \!-\! 1$.
%nodes that are one of two types: (a) \emph{branching nodes}: $\cT_B$; and (b) \emph{leaf nodes}: $\cT_L$. Branching nodes split an  %$\ab^\top \xb < b$

\setlength{\textfloatsep}{8pt}
\begin{figure}
    \centering
    {\includegraphics[width=\columnwidth]{figures/eq_1_fig2_v2.pdf}
    }
    \caption{A depiction of equation~\eqref{eq:lp_no_prune} for optimizing tree traversals given the tree parameters $\bm{\theta}$.}
    \label{fig:eq_1}
    %$n$ takes values in a range that covers common choices of batch size. Time and $n$ axis are represented in logarithmic scale.}
    %\label{fig:alg-time}
%         \includegraphics[width=0.99\textwidth]{figures/pruning/all-reg.pdf}
% %        \vspace{-3ex}
%         \captionof{figure}{Empty nodes (EN) as we vary $\lambda$.}
        %\label{fig:lambda}
\end{figure}
\subsection{Tree Traversal \& Pruning Programs}
Let the splitting functions of a complete tree $\{s_{\theta_t}: \mathcal{X} \to \mathbb{R}\}_{t=1}^{|\cT_B|}$ be fixed. The path through which a point $\xb$ traverses the tree can be encoded in
a vector $\zb \in \{0,1\}^{|\cT|}$, where each component $z_t$ indicates whether $\xb$ reaches node $t \in \cT$.
The following integer linear program (ILP) is maximized by a vector $\zb$ that describes \emph{tree traversal}:
%not clear what "vectorized indicator for x" means
%the vectorized indicator for $\xb$
\begin{align}
    % \max_{\zb_1, \ldots, \zb_n} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
    % \mbox{s.t. } \forall i \in [n],\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    % & r_{it} = \min \{ s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_R(t), \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    % & l_{it} = \min \{ -s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\top \xb
    % & z_{it} \in \{0, 1\}. \nonumber
    \max_{\zb} \;\;& \zb^\top \qb \label{eq:lp_no_prune} \\
    \mbox{s.t. } \forall t \in \cT \setminus \{ \text{root} \},\;\;& q_{t} = \min \{ R_{t} \cup L_{t} \} \nonumber \\
    & R_{t} = \{ s_{\theta_{t'}}(\xb) \;\;\;\!\mid \;\; \forall t' \in A_R(t)\} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    & L_{t} = \{ -s_{\theta_{t'}}(\xb) \mid \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\top \xb
    & z_{t} \in \{0, 1\}, \nonumber
\end{align}
where we fix $q_1\!=\!z_1\!=\!1$ (i.e., the root). Here $A_L(t)$ is the set of ancestors of node $t$ whose left child must be followed to get to $t$, and similarly for $A_R(t)$. % In the edge case where $A_L(t) = \varnothing$ define $l_t = \infty$ (and similarly for $A_R(t)$ and $r_t$).}
The quantities $q_{t}$ (where $\qb \!\in\! \mathbb{R}^{|\cT|}$ is the tree-vectorized version of $q_{t}$) describe the `reward' of sending $\xb$ to node $t$. This is based on how well the splitting functions leading to $t$ are satisfied ($q_{t}$ is positive if all splitting functions are satisfied and negative otherwise). This is visualized in Figure~\ref{fig:eq_1} and formalized below.
% however we allow for the full range of possible thresholds in order to relax to a continuous problem

\begin{lemma}\label{lemma:tree}
For an input $\xb$ and binary tree $\cT$ with splits $\{s_{\theta_{t}}, \forall t \in \cT_B\}$, the ILP in eq.~\eqref{eq:lp_no_prune} describes a valid tree traversal $\zb$ for $\xb$ (i.e., $z_t=1$ for any $t \in \cT$ if $\xb$ reaches $t$).
\end{lemma}

\begin{proof}
Assume without loss of generality that $s_{\theta_{t}}(\xb) \neq 0$ for all $t \in \cT$ (if this does not hold for some node $\tilde{t}$ simply add a small constant $\epsilon$ to $s_{\theta_{\tilde{t}}}(\xb)$). Recall that for any non-leaf node $t'$ in the fixed binary tree $\cT$, a point $\xb$ is sent to the left child if $s_{\theta_{t'}}(\xb) < 0$ and to the right child otherwise. Following these splits from the root, every point $\xb$ reaches a unique leaf node $f_{\xb} \in \cF$, where $\cF$ is the set of all leaf nodes.
Notice first that both $\min L_{f_{\xb}} > 0$ and $ \min R_{f_{\xb}} > 0$.\footnote{We use the convention that $\min \varnothing = \infty$ (i.e., for paths that go down the rightmost or leftmost parts of the tree).}
This is because $\forall t' \in A_L(f_{\xb})$ it is the case that $s_{\theta_{t'}}(\xb) < 0$, and  $\forall t' \in A_R(f_{\xb})$ we have that $s_{\theta_{t'}}(\xb) > 0$.
This is due to the definition of $f_{\xb}$ as the leaf node that $\xb$ reaches (i.e., it traverses to $f_{\xb}$ by following the aforementioned splitting rules).
Further, for any other leaf $f \in \cF \setminus \{f_{\xb}\}$ we have that either $\min L_{f} < 0$ or $\min R_{f} < 0$. This is because there exists a node $t'$ on the path to $f$ (and so $t'$ is either in $A_L(f)$ or $A_R(f)$) that does not agree with the splitting rules. For this node it is either the case that (i) $s_{\theta_{t'}}(\xb) > 0$ and $t' \in A_L(f)$, or that (ii) $s_{\theta_{t'}}(\xb) < 0$ and $t' \in A_R(f)$. In the first case $\min L_f < 0$, in the second $\min R_f < 0$. Therefore we have that $q_f < 0$ for all $f \in \cF \setminus \{f_{\xb}\}$, and $q_{f_{\xb}} > 0$. In order to maximize the objective $\zb^\top \qb$ we will have that $z_{f_{\xb}} = 1$ and $z_f = 0$. Finally, let $\mathcal{N}_{f_{\xb}}$ be the set of non-leaf nodes visited by $\xb$ on its path to $f_{\xb}$. Now notice that the above argument applied to leaf nodes can be applied to nodes at any level of the tree: $q_t > 0$ for $ t \in \mathcal{N}_{f_{\xb}}$ while $q_{t'} < 0$ for $t' \in \cT \setminus \mathcal{N}_{f_{\xb}} \cup f_{\xb}$. Therefore $\zb_{\mathcal{N}_{f_{\xb}} \cup f_{\xb}} = 1$ and $\zb_{\cT \setminus \mathcal{N}_{f_{\xb}} \cup f_{\xb}} = 0$, completing the proof.
\end{proof}

This solution is unique so long as $s_{\theta_{t}}(\xb_i)
\!\neq\! 0$ for all $t \in \cT, i \in \{1, \ldots, n\}$ (\ie, $s_{\theta_{t}}(\xb_i) \!=\! 0$ means equal preference to split $\xb_i$ left or right). Further the integer constraint on $z_{it}$ can be relaxed to an interval constraint $z_{it} \in [0, 1]$ w.l.o.g. This is because if $s_{\theta_{t}}(\xb_i)
\neq 0$ then $z_t=0$ if and only if $q_t < 0$ and $z_t=1$ when $q_t > 0$ (and $q_t \neq 0$).


% To do so, we will first introduce an inner optimization problem: a linear program (LP) that describes how a set of inputs $\{\xb_i\}_{i=1}^b$ traverses through the tree given fixed splitting parameters $\{ \theta_t\}_{t \in \cT_B}$. Specifically let $z_{it} \in [0,1]$ indicate if $\xb_i$ reaches node $t \in \cT$ (let $\zb_i \in [0,1]^T$ be the vector indicator every tree node for $\xb_i$)
% \begin{align}
%     \max_{\zb_1, \ldots, \zb_b} \;\;& \sum_{i=1}^b \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
%     \mbox{s.t.}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
%     & l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\toeq.p \xb
%     & z_{it} \in [0, 1] \nonumber
% \end{align}

While the above program works for any fixed tree, we would like to be able to also learn the structure of the tree itself.
% Let $\eta_t \in \bR$ be our preference for pruning/keeping node $t$ (larger $\eta_t$ indicates node $t$ should be kept).
% To encourage this pruning preference while ensuring connectivity,
We do so by learning a pruning optimization variable $a_t \in \{0,1\}$, indicating if node $t \in \cT$ is active (if $1$) or pruned (if $0$). %This can be used to prune whole portions of the tree, as all nodes with pruned parents are pruned.
We adapt eq.~\eqref{eq:lp_no_prune} into the following pruning-aware mixed integer program (MIP) considering all inputs $\{\xb_i\}_{i=1}^n$:
%to learn a valid pruning that obeys $\eta_t$:
%(where $\bm{\eta} \in [0,1]^{|\mathcal{T}|}$ is $\eta_t$ vectorized for all $t$):
\begin{align}
    \max_{\zb_1, \ldots, \zb_n, \ab} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i - \frac{\lambda}{2} \|\ab\|^2 \label{eq:ourilp} \\ %\label{eq:ilp_prune} \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} \}\nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in \{0,1\} \nonumber
    %q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    %& r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    %& l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ %
    %& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} %\}\nonumber \\
    %& z_{it} \leq a_t \nonumber \\
    %& z_{it} \in [0, 1], a_t \in \{0,1\}. \nonumber
\end{align}
with $\|\cdot\|$ denoting the $l_2$ norm.
We remove the first three constraints in eq.~\eqref{eq:lp_no_prune} as they are a deterministic computation independent of $\zb_1,\ldots,\zb_n,\ab$. We denote by $p(t)$ the parent of node $t$. The new constraints $a_t \leq a_{p(t)}$ ensure that child nodes $t$ are pruned if the parent node $p(t)$ is pruned, hence enforcing the tree hierarchy, while the other new constraint $z_{it} \leq a_t$ ensures that no point $\xb_i$ can reach node $t$ if node $t$ is pruned, resulting in losing the associated reward $q_{it}$. %In the above we have assumed fixed tree parameters $\theta_t$.
% \vlad{the 0-1 relaxation of z is no longer exact once we add pruning; the sentence in bold in the last paragraph might give the wrong impression}
Overall, the problem consists in a trade-off, controlled by hyper-parameter $\lambda \in \mathbb{R}$, between minimizing the number of active nodes through the pruning regularization term (since $a_t \in \{0,1\}, \|\ab\|^2 = \sum_t a_t^2 = \sum_t \mathbb{I}(a_t = 1)$) while maximizing the reward from points traversing the nodes.
%Notice that other norms, e.g. $\|\|_1$, could be considered on $\ab$ for controlling the pruning.
%%%%%%%%%%%%%%%%%%%
% OLD STUFF BELOW %
%%%%%%%%%%%%%%%%%%%

% We design a differentiable linear program (LP) that sparsely approximates an integer linear program (ILP) that is inspired by the mixed-integer program (MIP) of \citet{bertsimas2017optimal}.

% We introduce the following variables for our ILP:
% \begin{itemize}
%     % \item $\ab_t \in \mathbb{R}^d$: the splitting parameter for node $t \in \cT_B$
%     % \item $b_t \in \mathbb{R}$: the splitting threshold for node $t \in \cT_B$
%     \item $d_t \in \{0,1\}$: is node $t \in \cT$ active or not (i.e., 0 if it has it been pruned)
%     %if node $t \in \cT_B$ splits or not (if not we force all points to a leaf node)
%     \item $z_{it} \in \{0,1\}$: if $\xb_i$ reaches node $t \in \cT$
%     %\item $l_t \in \{0,1\}$: if node contains any points $t \in \cT_L$
%     %\item $c_{kt} \in \{0,1\}$: if node $t \in \cT_L$ predicts class $k$ (let $\cb_t$ be the $k$-dimensional indicator vector)
%     %\item $q_{ik} \in \{0,1\}$: if $\xb_i$ is predicted class $k$
% \end{itemize}

% % HERERERE:
% % We first observe that the following ILP produces
% % \begin{align}

% % \end{align}

% Given these variables we propose the following ILP:
% \begin{align}
%     \max \;\;& \frac{1}{nT} \sum_{i=1}^n \sum_{t \in \cT} \Bigg( \sum_{m \in A_R(t)} (\ab_m^\top \xb_i - b_m) z_{it} + \sum_{m' \in A_L(t)} ( b_{m'} - \ab_{m'}^\top \xb_i) z_{it} \Bigg) + \frac{\alpha}{T} \sum_{t \in \cT} \eta_t d_t \label{eq:ilp} \\% \in   \sum  (y_i - \langle \boldsymbol{\eta}^\top, \zb_i \rangle )^2   %+ \alpha \sum_{t \in \cT_B} d_t     % \Big( \sum_{j \in \cT_L} z_{it} \cb_{t} \Big) \label{eq:ilp} \\\
%     %\mbox{s.t.}\;\;& \sum_{k=1}^K c_{kt} = l_t, \;\;\; \forall t \in \cT_L \\
%     \mbox{s.t.}\;\;& \ab_m^\top \xb_i \geq b_m - (1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_R(t), \\
%     & \ab_m^\top (\xb_i + \mu)  \leq b_m + (1 + \mu)(1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_L(t), \\
%     %&\sum_{t \in \cT} z_{it} = d_t, \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq l_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq d_t, \forall t \in \cT, \\
%     %&l_{t} \leq d_t, \forall t \in \cT, \\
%     %&\sum_{i=1}^n z_{it} \geq N_{\mbox{min}} l_t, \;\;\; \forall t \in \cT, \;\;\;  i = 1, \ldots, n, \\
%     &z_{it} \leq d_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     & d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \\
%     & z_{ti} \leq z_{p(t)i}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{ti} + z_{s(t)i} \leq 1, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{\textrm{root}i} = 1, \;\;\; \forall i = 1, \ldots, n, \\
%     & d_{\textrm{root}} = 1, \\
% % & \sum_{t \in \cT_L} z_{it} = 1, \;\;\; \forall i = 1, \ldots, n, \\
% % %    & \sum_{k=1}^K c_{kt} = 1, \;\;\; \forall t \in \cT_L, \\
% % 0-c
% % 1-c
% % 1-1
% % 0-1
% % 0-0
% % 1-0
% %     \sum_{t \in \cT_L} z_{it} + c_{tk} \leq p_{ik}, \;\;\; \forall t \in \cT_L, \\
% %     \sum_{t \in \cT_L} \sum_{k=1}^K  k z_{it} c_{tk}
% %     \sum_{t \in \cT_L} z_{it}
% %     \sum_{k=1}^K k c_{tk} = p_{t}
% %     z_{it}
%     & z_{it} \in \{0, 1\}, \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \\
%     & d_t \in \{0, 1\} \;\;\; \forall t \in \cT.
% \end{align}
% where $p(t)$ is the parent node of node $t$ , $s(t)$ is the sibling node of node $t$, $\mu$ is a small constant (e.g., $5 \times 10^{-3})$, and $\boldsymbol{\eta}, \ab, b, \xb, y$ are all inputs. %Thus, the multiplication between $\cb_t$ and $z_{it}$ is the only quadratic term, all constraints are linear.

% We explain each line now:
% \begin{itemize}
%     \item (1): This line encourages z to represent the tree by zeroing out the term it is multiplied with, if that term is negative, and vice-versa.
%     % \item (1): This line takes the representation $\zb_i \in \{0, 1\}^T$ that describes the path that $\xb_i$ traverses through the tree and scores it by $\boldsymbol{\eta}$.
%     \item (2)/(3): These enforce points to follow the rules of the tree, see equations (9)-(14) in \citet{bertsimas2017optimal}.
%     \item (4): This ensures that a point does not go to a node if it has been pruned, i.e., $d_t = 0$.
%     \item (5): This ensures that a child node is pruned if its parent is pruned.
%     \item (6): Prevents a point $\xb$ from going to a child node if it does not go to a parent node.
%     \item (7): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (8)/(9): The root cannot be pruned and every point should go through it.
%     % \item
%     % %a child node from branching if a parent node doesn't branch (i.e., $d_{p(t)} = 0$).
%     % \item (4): This ensures that no points $\xb$ go to node $t$ if $l_t$ decides so. Or equivalently makes $l_t=1$ if points go to node $t$.
%     % \item (5): This makes sure that $l_t=0$ (i.e., no points go to node $t$) if that node has been pruned (i.e., $d_t=0$).
%     % \item (6): This enforces a minimum number of points $N_{\mbox{min}}$ at each leaf node.
%     % \item (7)/(8): (optional) As we assume inputs $\xb$ are bounded in $[0,1]^d$ we restrict our splitting parameters to fall in the same range $[0,1]$.
%     % %\item (8)/(9): This prunes the full tree. Specifically, this ensures that we send points left at branch node $t$ if $d_t=0$ (i.e., if we do not split at node $t$). It does so by ensuring that $\ab_t=0$ and $b_t=0$ if $d_t=0$.
%     % \item (10):
%     % \item (11): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (10)/(11): Ensures variables are binary.
% \end{itemize}

% Relaxing $z_{it} \in [0,1]$ allows points to partially reach multiple nodes. We can think of this as each point as having some probability of going down multiple paths. %Relaxing $l_t \in [0,1]$ allows leaf nodes $t$ to partially contain points. As above this can be thought of as nodes containing points with some probability.
% Relaxing $d_t \in [0,1]$ allows nodes $t$ to be partially active. This can be thought of as a distribution over trees.

\input{sections/new_problem}
% \subsection{Learning Tree Parameters}

% A natural approach to learn splitting parameters $\theta_t$ would be to do so in the MIP itself, as in the optimal tree literature. However, this would severely restrict allowed splitting functions as even linear splitting functions can only practically run on at most thousands of training inputs \citep{bertsimas2017optimal}. Instead, we propose to learn $s_{\theta_{t}}$ via gradient descent.
% % as function more complicated than linear/quadratic
% % most high-performance MIP solvers (Gurobi, GLPK, SCIP) allow only linear/quadratic constraints
% % In a twist from the optimal tree learning literature, instead of learning splitting parameters $\theta_t$ within the MIP
% % we regard
% % the split weights $\theta_t$ as neural network parameters and not
% % variables in the nested optimization problem; we thus learn their value using gradient descent.
% % To do so, first note that the first three constraints in eq.~\eqref{eq:ilp_prune} are a
% % deterministic computation of the values of $\qb$. Thus we can remove these as constraints, leaving the simpler problem
% % \begin{equation}\label{eq:ourilp}
% % \begin{aligned}
% %     \max_{\zb_1, \ldots, \zb_n, \db} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i + \bm{\eta}^\top \db\\
% %     \mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \setminus \{\text{root}\} \\
% %     & z_{it} \leq d_t \\
% %     & z_{it} \in [0, 1], d_t \in \{0,1\}.
% % \end{aligned}
% % \end{equation}
% To do so, we must be able to compute
% %To embed decision tree induction as a differentiable hidden layer in a
% %neural network, we require access to
% the gradients
% $\pfrac{\zb}{\bm{\eta}}$ and $\pfrac{\zb}{\qb}$. However, the solutions of  eq.~\ref{eq:ourilp} are discontinuous and piecewise-constant.

% To solve this, we relax the integer constraint on $\ab$ to the interval $[0,1]$ and add quadratic regularization $-\nicefrac{1}{2}\sum_i \| \zb_i \|_2^2 -\nicefrac{1}{2} \| \ab \|_2^2$.
% Rearranging and negating the objective yields
% %\begin{equation}
% \begin{align}
%   \mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \argmin_{\zb_1, \ldots, \zb_n, \ab} \;\;& \hlf\sum_{i=1}^n \| \zb_i - \qb_i \|^2 + \hlf \| \bm{\eta} - \ab \|^2 \label{eq:qp_prune}
%  \\
%     \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT
% \setminus \{\text{root}\}  \nonumber \\
%     & z_{it} \leq a_t \nonumber \\
%     & z_{it} \in [0, 1], a_t \in [0,1]. \nonumber
% \end{align}
% The regularization makes the objective strongly convex, so from convex duality
% it follows that $\mathrm{T}_{\bm{\eta}}$ is Lipschitz continuous
% \citep[Corollary 3.5.11]{zalinescu}.
% By Rademacher's theorem \citep[Theorem 9.1.2]{borweinlewis}, $\mathrm{T}_{\bm{\eta}}$ is thus differentiable almost everywhere.
% Generic methods such as OptNet~\citep{optnet} could be used to compute the
% solution and the gradients. However,
% by using the tree structure of the constraints, we next derive an efficient specialized algorithm.
% %We then show how this view
% %gives a direct, efficient computation of the backward pass.
% The main insight, shown below, reframes pruned binary tree learning
% as isotonic optimization.
% \begin{proposition}\label{prop:iso}
% Let $\mathcal{C}= \big\{ \ab \in \mathbb{R}^{|\mathcal{T}|} :
% a_t \leq a_{p(t)} ~~\text{for all}~~ t \in \mathcal{T} \setminus \{ \text{root}
% \} \big\}.$
% Consider
% \begin{equation}\label{eq:nested_qp_prune}
% \ab^\star = \argmin_{\ab\in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\;
% \sum_{t \in \mathcal{T}} \Big( \hlf {(a_t - \eta_t)}^2
% + \sum_{i: a_t \leq q_{it}} \hlf {(a_t - q_{it})}^2 \Big)\,.
% \end{equation}
% Define%
% \footnote{Here $\operatorname{Proj}_{\mathcal{S}}(x)$ is the projection of $x$ onto set $\mathcal{S}$. If $\mathcal{S}$ are box constraints, projection amounts to clipping.}
% $[z^\star]_{it} = \operatorname{Proj}_{[0, a_t^\star]}(q_{it})$.
% Then, $\mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \zb^\star_1, \ldots, \zb^\star_n, \ab^\star$.
% \end{proposition}
% \begin{proof}
% The constraints and objective function of eq.~\ref{eq:qp_prune} are separable,
% so we may push the minimization \wrt $\zb$ inside the objective, resulting in:
% \begin{equation}
% \argmin_{\ab \in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\; \hlf \| \bm{\eta} - \ab \|^2
% + \sum_{t \in \mathcal{T}} \sum_{i=1}^n
% \min_{0 \leq z_{it} \leq a_t} \hlf{({z}_{it} - {q}_{it})}^2\,.
% \end{equation}
% Each of the inner nested minimizations,
% $\min_{0 \leq z_{it} \leq a_t} \hlf (z_{it} - q_{it})^2$
% is a one-dimensional projection onto box constraints, with solution
% $z^\star_{it} = \operatorname{Proj}_{[0, a_t]}(q_{it})$.
% %\begin{equation}\label{eq:z_from_d} z_{it} = {[q_{it}]}_{[0, d_t]}.\end{equation}
% We may use this result to eliminate $\zb$ from the objective,
% noting that
% \begin{equation}
% \hlf(z^\star_{it} - q_{it})^2 =
% \begin{cases}
% \hlf~q_{it}^2, & q_{it} < 0\\
% 0, & 0 \leq q_{it} < a_t\\
% \hlf(a_t - q_{it})^2, & q_{it} \geq a_t\\
% \end{cases}
% \end{equation}

% the first two conditions are constants \wrt $a_t$
% %As a function of $a_t$, the first two conditions are constants.
% Thus, the objective functions eq.~(\ref{eq:qp_prune}) and eq.~(\ref{eq:nested_qp_prune})
% differ by a constant. As their constraints are also the same, they have equivalent minimizers $\ab^\star$.
% %This leaves us with the equivalent problem in $\db$,
% %\begin{equation}\label{eq:nested_qp_prune}
% %\begin{aligned}
%     %\min_{\bm{d}} \;\;&
% %\sum_t \Big( \hlf {(d_t - \eta_t)}^2
% %+ \sum_{i: d_t \leq q_{it}} \hlf {(d_t - q_{it})}^2 \Big) \\
% %\mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \\
% %& d_t \in [0,1].
% %\end{aligned}
% %\end{equation}
% %After solving this problem, we may use \Eqref{eq:z_from_d} to get
% %the optimal $\zb$ (and likewise for gradients, using the chain rule.)
% \end{proof}
% \begin{algorithm}[t]\small
% \caption{Latent decision tree induction via isotonic optimization.\label{alg}}
% \begin{algorithmic}[1]
% %\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
% %\State \textbf{Initialize:}
% \State initial partition
% $\mathcal{G} \leftarrow \big\{ \{1\}, \{2\}, \cdots \}
% \subset 2^\mathcal{T}$
% \ForAll {$G \in \mathcal{G}$}
% \State $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
% \Comment{Proposition~\ref{prop:scalar_subproblem}}
% \EndFor
% \While {exists $t$ such that $a_t > a_{p(t)}$}
% \State $t_\text{max} \leftarrow \argmax_t \{a_t: a_t > a_{p(t)}\}$
% \State merge $G \leftarrow G \cup G'$ where $t \in G$ and $p(t) \in G'$.
% \State update  $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
% \Comment{Proposition~\ref{prop:scalar_subproblem} again}
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% \paragraph{Efficiently inducing trees as isotonic optimization.}
% From Proposition~\ref{prop:iso},
% notice that eq.~\ref{eq:nested_qp_prune} is an instance of tree-structured isotonic
% optimization:
% the objective decomposes over \emph{nodes}, and the inequality constraints
% correspond to edges in a rooted tree:
% \begin{equation}\label{eq:nested_qp_prune_isotonic}
% \argmin_{\ab \in \mathcal{C}} \sum_{t \in \mathcal{T}} g_t(a_t)\,,
% % \qquad \text{subject to}\qquad d_t \leq d_{p(t)}~\text{for all }t
% %\in \cT \setminus \{ \text{root}\},
% ~~~~\text{where}~~~~ g_t(a_t) =
% \hlf {(a_t - \eta_t)}^2
% +\!\sum_{i: a_t \leq q_{it}}\!\!\hlf {(a_t - q_{it})}^2  + \iota_{[0,1]}(a_t).
% \end{equation}
% where $\iota_{[0,1]}(a_t)\!=\!\infty$ if $a_t \notin [0,1]$ and $0$ otherwise.
% This problem can be solved by a generalized \emph{pool adjacent violators} (PAV)
% algorithm: Obtain a tentative solution by ignoring the constraints, then
% iteratively remove violating edges $a_t > a_{p(t)}$ by \emph{pooling together}
% the nodes at the end points. At the optimum, the nodes are organized into a
% partition $\mathcal{G} \subset 2^\mathcal{T}$, such that if two nodes $t, t'$
% are in the same group $G \in \mathcal{G}$, then $a_t = a_t' \coloneqq a_G$.

% When the inequality constraints are the edges of a rooted tree, as is the case
% here, the PAV algorithm finds the optimal solution in at most $|\mathcal{T}|$ steps,
% where each involves updating the $a_G$ value for a newly-pooled group by solving
% a one-dimensional subproblem of the form \citep{yu2016exact}\footnote{Compared to \citet{yu2016exact}, our tree inequalities are in the opposite
% direction.  This is equivalent to a sign flip of parameter $\ab$, \ie,
% to selecting the \emph{maximum} violator rather than the minimum one at each
% iteration.}
% \begin{equation}\label{eq:scalar_subproblem}
% a_G = \argmin_{a \in \bR} \sum_{t \in G} g_t(a)\,,
% \end{equation}
% resulting in Algorithm~\ref{alg}.
% It remains to show how to solve eq.~\ref{eq:scalar_subproblem}. The next
% result, proved in Appendix~\ref{supp:scalar_subproblem}, gives an exact and efficient solution,
% with an algorithm that requires finding the nodes with highest
% $q_{it}$ (\ie, the nodes where $\xb_i$ is most highly encouraged to traverse).

% \begin{proposition}\label{prop:scalar_subproblem}%
% The solution to the one-dimensional problem in
% eq.~(\ref{eq:scalar_subproblem}) for any $G$ is given by
% \begin{equation}\argmin_{a \in \bR} \sum_{t \in G} g_t(a) =
% \operatorname{Proj}_{[0,1]}\big(a(k^\star)\big) \quad \text{where}\quad a(k^\star) \coloneqq
% \frac{\sum_{t \in G} \eta_t + \sum_{(i,t) \in S(k^\star)} q_{it}}{|G|+k^\star},
% \end{equation}
% $S(k) = \{j^{(1)}, \ldots, j^{(k)}\}$ is the set of indices $j=(i,t) \in
% \{1, \ldots, n\} \times G$ into
% the $k$ highest values of $\qb$, \ie,
% $q_{j^{(1)}} \geq
% q_{j^{(2)}} \geq \ldots \geq
% %q_{j^{(k)}} \geq \ldots \geq
% q_{j^{(m)}}$,
% and $k^\star$ is the smallest $k$ satisfying
% $a(k) > q_{j^{(k+1)}}$.
% \end{proposition}

% Figure~\ref{fig:time} shows the speed of our specialized algorithm compared to a leading generic optimizer (details in Appendix~\ref{app:time}).

% \paragraph{Backward pass and efficient implementation details.}
% Algorithm~\ref{alg} is a sequence of differentiable operations that can be
% implemented \emph{as is} in automatic differentiation frameworks. However,
% because of the prominent loops and indexing operations, we opt for a low-level
% implementation as a \texttt{C++} extension.
% Since the $\qb$ values are constant \wrt $\ab$, we only need to sort them
% once as preprocessing. % in \vlad{TODO but should be sth like $\mathcal{O}(d(n \log n))$}.
% For the backward pass, rather than relying on automatic
% differentiation, we make two remarks about the form of $\ab$.
% Firstly, its elements are organized in groups, \ie, $a_t = a_t' = a_G$ for $\{t,
% t'\} \subset G$. Secondly, the value $a_G$ inside each group
% depends only on  the optimal support set $S^\star_G \coloneqq S(k^\star)$ as
% defined for each subproblem  by Proposition~\ref{prop:scalar_subproblem}.
% Therefore, in the forward pass, we must store only the node-to-group mappings
% and the sets $S^\star_G$. Then, if $G$ is the group of node $t$,
% \begin{equation*}
% \pfrac{a^\star_t}{\eta_{t'}} = \begin{cases}
% \frac{1}{|G| + k^\star},
% & 0 < a^\star_t < 1 ~\text{and}~
% t' \in G,\\
% 0,&\text{otherwise.}
% \end{cases}
% ~~
% \pfrac{a^\star_t}{q_{it'}} = \begin{cases}
% \frac{1}{|G| + k^\star},
% & 0 < a^\star_t < 1,
% ~\text{and}~
% (i,t') \in S^\star_G,\\
% 0,&\text{otherwise.}
% \end{cases}.
% \end{equation*}
% As $\mathrm{T}_{\bm{\eta}}$ is differentiable almost everywhere, these
% expressions yield the unique Jacobian at all but a measure-zero set of
% points, where they yield one of the Clarke generalized Jacobians
% \citep{clarke_book}.
% We then rely on automatic differentiation to propagate gradients from $\qb$ to
% the split parameters $\theta$; since $\qb$ is defined elementwise via $\min$
% functions, the gradient propagates through the minimizing path,
% by Danskin's theorem \citep[Proposition B.25,][]{bertsekas-nonlin,danskin_theorem}.

% \subsection{The Overall Objective}
% % skip connection = concatenation of input and tree path
% % MLP = [Linear, Elu, Dropout] * num layers + Linear

% \begin{algorithm}[t]\small
% \caption{\label{alg:learn}Learning with latent decision tree representations.}
% \begin{algorithmic}[1]
% %\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
% %\State \textbf{Initialize:}
% \State initialize neural network parameters $\bm{\phi},\bm{\theta}$
% %(architecture-specific)
% \State initialize pruning scores $\bm{\eta} \sim \mathcal{U}(-1, 1)$
% \Repeat
% \State sample batch $\{\xb_i\}_{i \in B}$
% \State induce traversals $\{\zb_i\}_{i \in B}, \ab =
% \mathrm{T}_{\bm{\eta}}\big(\{q_{\bm{\theta}}(\xb_i)\}\big)$
% \Comment{algorithm~\ref{alg}; differentiable}
% \State update parameters using
% $\nabla_{\{\bm{\theta},\bm{\eta},\bm{\phi}\}}
% \ell(f_{\bm{\phi}} (\xb_i, \zb_i)) + \lambda \|\bm{\eta}\|_\Omega$
% \Comment{autograd}
% %\Until{convergence}
% \end{algorithmic}
% \end{algorithm}

% We are now able to describe the overall optimization procedure that simultaneously learns tree parameters: (a) input traversals $\zb_1, \ldots, \zb_n$; (b) tree pruning $\ab$; and (c) split parameters $\theta_t$. Given this tree, we will additionally learn a function $f_\phi(\zb, \xb)$ to minimize an arbitrary loss $\ell(\cdot)$ as follows,
% \begin{equation}
% \begin{aligned}
%     \min_{\bm{\theta},\bm{\eta},\bm{\phi}}\;\;& \sum_{i=1}^n \ell\big(f_\phi(\xb_i, \zb_i)\big) + \lambda \| \bm{\eta} \|_{\Omega} \label{eq:obj} \\
%     \mbox{where}\;\;& \zb_1, \ldots, \zb_n, \ab := \mathrm{T}_{\bm{\eta}}\big(q_{\bm{\theta}}(\xb_1), \ldots, q_{\bm{\theta}}(\xb_n)\big)\,.
% \end{aligned}
% \end{equation}
% In practice, we perform mini-batch updates for efficient training;
% the procedure is sketched in Algorithm~\ref{alg:learn}.
% Recall $\mathrm{T}_{\bm{\eta}}(\cdot)$ is the solution to the tree program (eq.~\ref{eq:qp_prune}), so we may update the parameters $\bm{\eta}$ and $\bm{\theta}$ by back-propagation. Here we define $q_{\theta}(\xb_i) := \qb_i$ to make explicit the dependence of $\qb_i$ on $\theta$. The regularization $\| \cdot \|_{\Omega}$ can be any norm (in practice we find $\Omega=\infty$ to perform the best.)
% The overall model is represented in Figure~\ref{fig:arch}.
% %Specifically, $\qb_i$ is given by a  deterministic function $q_{\theta}(\xb_i)$.

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}


% Given a loss function $\ell$
% Given this, we can write the overall objective
% \matt{Working on this}


% In the following, we train via end-to-end back-propagation a Deep Neural Network built as a composition of a Latent Tree (LT) layer followed by a MultiLayer Perceptron (MLP) predictor.
% We also design an optional skip connection between the input $\xb$ and the predictor to circumvent the LT layer, as illustrated in Figure~\ref{fig:arch}.
% The skip connection is particularly useful for regression tasks or when the predictor is a single linear layer, as in these scenarios relying only on the coarse tree representation may hinder results.
% We construct the MLP predictor as a sequence of fully connected layers, with Elu activation~\citep{clevert2015fast} and dropout~\citep{srivastava2014dropout}, followed by a final fully connected layer.
% We refer to the set of predictor's parameters as $\phi$.
% Given a fixed tree depth, the LT layer's training parameters consist of pruning parameter $\bm{\eta}$ and splitting parameters $\theta = \{ \bm{\theta}_t\}_{t \in \cT_B}$.

% Our optimization procedure consists in alternating between solving Problem~\ref{eq:qp_prune}, i.e. computing the tree routing $\bm{z}$, and optimizing the model parameters by gradient descent:

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}

% where $\ell(.)$ is the loss function of choice, depending on the downstream task at hand, measuring the goodness of the predictor's output w.r.t. the target $y$;
% $\lambda$ is the hyper-parameter controlling the trade-off between pruning strength and performance.

% As mentioned before, our formulation allows for integrating any type of split function.
% Depending on the task and on the type of inputs, one could train decision hyper-planes or even more complex functions, such as Convolutional Neural Networks.
% In the following, we make use of decision hyper-planes, and tune whether to apply an Elu activation to their output.
% \vlad{elu is monotonic so I would expect it not to
% change the decision boundary, right? or am I missing something}
% \vale{I'd say that the splits are the same, but the leaf values used as representation are different.}


==> Learning Latent Decision Trees/sections/methods_arxiv.tex <==
Given inputs $\{\xb_i\}_{i=1}^n$,  %where each $\xb \in [0,1]^p$.
our goal is to learn a latent binary decision tree $\cT$ with maximum depth $D$. This tree sends each input $\xb$ through branching nodes to a specific leaf node  in the tree. Specifically, all branching nodes $\cT_B \subset \cT$ split an input $\xb$ by forcing it to go to its left child if
$s_\theta(\xb) < 0$,
and right otherwise. There are three key parts of the tree that need to be identified: 1. The \emph{continuous} parameters $\theta_t \in \mathbb{R}^d$ that describe how $s_{\theta_t}$ splits inputs at every node $t$; 2. The \emph{discrete} paths $\zb$ made by each input $\xb$ through the tree; 3. The \emph{discrete} choice $a_t$ of whether a node $t$ should be active or pruned. We describe how to learn each of these below.
% Our strategy will be to first fix splitting parameters $\theta_t$ for all $t$. Then to introduce a mixed-integer program (MIP) for learning paths $\zb$ and pruning $d_t$. %We then modify this to a mixed-integer program (MIP) that solves both 2 and 3.
% Finally we sparsely relax the MIP to allow for argmin differentiation to simultaneously solve for $\theta_t$.

% Our goal is to learn $\cT$ that is good for some downstream task. To do so,
% %by learning a scoring vector $\{ \boldsymbol{\eta} \}_{i=1}^n$ where $\boldsymbol{\eta} \in \mathbb{R}^T$ that describes the benefit of sending $\xb_i$ along a particular route in the tree.
% we will learn the splitting parameters of the tree $\{ \theta_t,\}_{t \in \cT_B}$.
% % For these parameters we impose the following constrain
% % \begin{align}
% %     \sum_{j=1}^d a_{jt} = 1, \;\;\; 0 \leq \ab_t, b_t \leq 1,
% %     \;\;\; \forall t \in \cT_B. \nonumber
% % \end{align}
% Specifically, let $\cT$ have maximum depth $D$. %This tree has at most $T \!=\! 2^{(D+1)} \!-\! 1$.
%nodes that are one of two types: (a) \emph{branching nodes}: $\cT_B$; and (b) \emph{leaf nodes}: $\cT_L$. Branching nodes split an  %$\ab^\top \xb < b$

\subsection{Tree-Traversal \& Pruning Programs}

Imagine the splitting functions of the tree $s_{\theta_t}$ are fixed. Given this, the following integer linear program (ILP) describes how inputs $\xb$ traverse the tree. The solution $z_{it} \in \{0,1\}$ indicates if $\xb_i$ reaches node $t \in \cT$ (for notational simplicity let $\zb_i \in \{0,1\}^{|\cT|}$ be the vectorized indicator for $\xb_i$),
\begin{align}
    \max_{\zb_1, \ldots, \zb_n} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
    \mbox{s.t. } \forall i \in [n],\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    & r_{it} = \min \{ s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_R(t), \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    & l_{it} = \min \{ -s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\top \xb
    & z_{it} \in \{0, 1\}. \nonumber
\end{align}
Here $A_L(t)$ is the set of ancestors of node $t$ whose left child must be followed to get to $t$, and similarly for $A_R(t)$. The quantities $q_{it}$ (where $\qb_i \in \mathbb{R}^{|\cT|}$ is the tree-vectorized version of $q_{it}$) describe the `reward' of sending $\xb_i$ to node $t$. This is based on how well the splitting functions leading to $t$ are satisfied ($q_{it}$ is positive if all splitting functions are satisfied and negative otherwise).

Notice that the solution is unique so long as $s_{\theta_{t}}(\xb_i)
\!\neq\! 0$ for all $t \in \cT, i \in \{1, \ldots, n\}$ (\ie, $s_{\theta_{t}}(\xb_i) \!=\! 0$ means there is no preference to split $\xb_i$ left or right). Further note that \textbf{the integer constraint on $z_{it}$ can be relaxed to an interval constraint $z_{it} \in [0, 1]$ without loss of generality}. This is because if $s_{\theta_{t}}(\xb_i)
\neq 0$ then $z_t=0$ if and only if $q_t < 0$ and $z_t=1$ when $q_t > 0$ (and $q_t \neq 0$).


% To do so, we will first introduce an inner optimization problem: a linear program (LP) that describes how a set of inputs $\{\xb_i\}_{i=1}^b$ traverses through the tree given fixed splitting parameters $\{ \theta_t\}_{t \in \cT_B}$. Specifically let $z_{it} \in [0,1]$ indicate if $\xb_i$ reaches node $t \in \cT$ (let $\zb_i \in [0,1]^T$ be the vector indicator every tree node for $\xb_i$)
% \begin{align}
%     \max_{\zb_1, \ldots, \zb_b} \;\;& \sum_{i=1}^b \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
%     \mbox{s.t.}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
%     & l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\toeq.p \xb
%     & z_{it} \in [0, 1] \nonumber
% \end{align}

While the above program works for any fixed tree, we would like to be able to also learn the structure of the tree itself. Let $\eta_t \in \bR$ be our preference for pruning/keeping node $t$ (larger $\eta_t$ indicates node $t$ should be kept). 
To encourage this pruning preference while ensuring connectivity,
we introduce an additional optimization variable $a_t \in \{0,1\}$, indicating if node $t \in \cT$ is active (if $1$) or pruned (if $0$).
We may now adapt eq.~\ref{eq:lp_no_prune} into the following pruning-aware mixed integer program (MIP):
%to learn a valid pruning that obeys $\eta_t$:
%(where $\bm{\eta} \in [0,1]^{|\mathcal{T}|}$ is $\eta_t$ vectorized for all $t$):
\begin{align}
    \max_{\zb_1, \ldots, \zb_n, \ab} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i + \boldsymbol{\eta}^\top \ab \label{eq:ourilp} \\ %\label{eq:ilp_prune} \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} \}\nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in \{0,1\}. \nonumber
    %q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    %& r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    %& l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ %
    %& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} %\}\nonumber \\
    %& z_{it} \leq a_t \nonumber \\
    %& z_{it} \in [0, 1], a_t \in \{0,1\}. \nonumber
\end{align}
Here we have removed the first three constraints in eq.~\ref{eq:lp_no_prune} as they are a deterministic computation independent of $\zb_1,\ldots,\zb_n,\ab$. Further $p(t)$ indicates the parent of node $t$. The added constraint $a_t \leq a_{p(t)}$ ensures that child nodes $t$ are pruned if parent nodes $p(t)$ are pruned. While the new constraint $z_{it} \leq a_t$ ensures that no point $\xb_i$ can reach node $t$ if node $t$ is pruned. %In the above we have assumed fixed tree parameters $\theta_t$.



%%%%%%%%%%%%%%%%%%%
% OLD STUFF BELOW %
%%%%%%%%%%%%%%%%%%%

% We design a differentiable linear program (LP) that sparsely approximates an integer linear program (ILP) that is inspired by the mixed-integer program (MIP) of \citet{bertsimas2017optimal}.

% We introduce the following variables for our ILP:
% \begin{itemize}
%     % \item $\ab_t \in \mathbb{R}^d$: the splitting parameter for node $t \in \cT_B$
%     % \item $b_t \in \mathbb{R}$: the splitting threshold for node $t \in \cT_B$
%     \item $d_t \in \{0,1\}$: is node $t \in \cT$ active or not (i.e., 0 if it has it been pruned)
%     %if node $t \in \cT_B$ splits or not (if not we force all points to a leaf node)
%     \item $z_{it} \in \{0,1\}$: if $\xb_i$ reaches node $t \in \cT$
%     %\item $l_t \in \{0,1\}$: if node contains any points $t \in \cT_L$
%     %\item $c_{kt} \in \{0,1\}$: if node $t \in \cT_L$ predicts class $k$ (let $\cb_t$ be the $k$-dimensional indicator vector)
%     %\item $q_{ik} \in \{0,1\}$: if $\xb_i$ is predicted class $k$
% \end{itemize}

% % HERERERE:
% % We first observe that the following ILP produces
% % \begin{align}

% % \end{align}

% Given these variables we propose the following ILP:
% \begin{align}
%     \max \;\;& \frac{1}{nT} \sum_{i=1}^n \sum_{t \in \cT} \Bigg( \sum_{m \in A_R(t)} (\ab_m^\top \xb_i - b_m) z_{it} + \sum_{m' \in A_L(t)} ( b_{m'} - \ab_{m'}^\top \xb_i) z_{it} \Bigg) + \frac{\alpha}{T} \sum_{t \in \cT} \eta_t d_t \label{eq:ilp} \\% \in   \sum  (y_i - \langle \boldsymbol{\eta}^\top, \zb_i \rangle )^2   %+ \alpha \sum_{t \in \cT_B} d_t     % \Big( \sum_{j \in \cT_L} z_{it} \cb_{t} \Big) \label{eq:ilp} \\\
%     %\mbox{s.t.}\;\;& \sum_{k=1}^K c_{kt} = l_t, \;\;\; \forall t \in \cT_L \\
%     \mbox{s.t.}\;\;& \ab_m^\top \xb_i \geq b_m - (1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_R(t), \\
%     & \ab_m^\top (\xb_i + \mu)  \leq b_m + (1 + \mu)(1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_L(t), \\
%     %&\sum_{t \in \cT} z_{it} = d_t, \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq l_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq d_t, \forall t \in \cT, \\
%     %&l_{t} \leq d_t, \forall t \in \cT, \\
%     %&\sum_{i=1}^n z_{it} \geq N_{\mbox{min}} l_t, \;\;\; \forall t \in \cT, \;\;\;  i = 1, \ldots, n, \\
%     &z_{it} \leq d_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     & d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \\
%     & z_{ti} \leq z_{p(t)i}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{ti} + z_{s(t)i} \leq 1, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{\textrm{root}i} = 1, \;\;\; \forall i = 1, \ldots, n, \\
%     & d_{\textrm{root}} = 1, \\
% % & \sum_{t \in \cT_L} z_{it} = 1, \;\;\; \forall i = 1, \ldots, n, \\
% % %    & \sum_{k=1}^K c_{kt} = 1, \;\;\; \forall t \in \cT_L, \\
% % 0-c
% % 1-c
% % 1-1
% % 0-1
% % 0-0
% % 1-0
% %     \sum_{t \in \cT_L} z_{it} + c_{tk} \leq p_{ik}, \;\;\; \forall t \in \cT_L, \\
% %     \sum_{t \in \cT_L} \sum_{k=1}^K  k z_{it} c_{tk}
% %     \sum_{t \in \cT_L} z_{it}
% %     \sum_{k=1}^K k c_{tk} = p_{t}
% %     z_{it}
%     & z_{it} \in \{0, 1\}, \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \\
%     & d_t \in \{0, 1\} \;\;\; \forall t \in \cT.
% \end{align}
% where $p(t)$ is the parent node of node $t$ , $s(t)$ is the sibling node of node $t$, $\mu$ is a small constant (e.g., $5 \times 10^{-3})$, and $\boldsymbol{\eta}, \ab, b, \xb, y$ are all inputs. %Thus, the multiplication between $\cb_t$ and $z_{it}$ is the only quadratic term, all constraints are linear.

% We explain each line now:
% \begin{itemize}
%     \item (1): This line encourages z to represent the tree by zeroing out the term it is multiplied with, if that term is negative, and vice-versa.
%     % \item (1): This line takes the representation $\zb_i \in \{0, 1\}^T$ that describes the path that $\xb_i$ traverses through the tree and scores it by $\boldsymbol{\eta}$.
%     \item (2)/(3): These enforce points to follow the rules of the tree, see equations (9)-(14) in \citet{bertsimas2017optimal}.
%     \item (4): This ensures that a point does not go to a node if it has been pruned, i.e., $d_t = 0$.
%     \item (5): This ensures that a child node is pruned if its parent is pruned.
%     \item (6): Prevents a point $\xb$ from going to a child node if it does not go to a parent node.
%     \item (7): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (8)/(9): The root cannot be pruned and every point should go through it.
%     % \item
%     % %a child node from branching if a parent node doesn't branch (i.e., $d_{p(t)} = 0$).
%     % \item (4): This ensures that no points $\xb$ go to node $t$ if $l_t$ decides so. Or equivalently makes $l_t=1$ if points go to node $t$.
%     % \item (5): This makes sure that $l_t=0$ (i.e., no points go to node $t$) if that node has been pruned (i.e., $d_t=0$).
%     % \item (6): This enforces a minimum number of points $N_{\mbox{min}}$ at each leaf node.
%     % \item (7)/(8): (optional) As we assume inputs $\xb$ are bounded in $[0,1]^d$ we restrict our splitting parameters to fall in the same range $[0,1]$.
%     % %\item (8)/(9): This prunes the full tree. Specifically, this ensures that we send points left at branch node $t$ if $d_t=0$ (i.e., if we do not split at node $t$). It does so by ensuring that $\ab_t=0$ and $b_t=0$ if $d_t=0$.
%     % \item (10):
%     % \item (11): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (10)/(11): Ensures variables are binary.
% \end{itemize}

% Relaxing $z_{it} \in [0,1]$ allows points to partially reach multiple nodes. We can think of this as each point as having some probability of going down multiple paths. %Relaxing $l_t \in [0,1]$ allows leaf nodes $t$ to partially contain points. As above this can be thought of as nodes containing points with some probability.
% Relaxing $d_t \in [0,1]$ allows nodes $t$ to be partially active. This can be thought of as a distribution over trees.

\subsection{Learning Tree Parameters}

A natural approach to learn splitting parameters $\theta_t$ would be to do so in the MIP itself, as in the optimal tree literature. However, this would severely restrict allowed splitting functions as even linear splitting functions can only practically run on at most thousands of training inputs \citep{bertsimas2017optimal}. Instead, we propose to learn $s_{\theta_{t}}$ via gradient descent.
% as function more complicated than linear/quadratic
% most high-performance MIP solvers (Gurobi, GLPK, SCIP) allow only linear/quadratic constraints
% In a twist from the optimal tree learning literature, instead of learning splitting parameters $\theta_t$ within the MIP
% we regard
% the split weights $\theta_t$ as neural network parameters and not
% variables in the nested optimization problem; we thus learn their value using gradient descent.
% To do so, first note that the first three constraints in eq.~\eqref{eq:ilp_prune} are a
% deterministic computation of the values of $\qb$. Thus we can remove these as constraints, leaving the simpler problem
% \begin{equation}\label{eq:ourilp}
% \begin{aligned}
%     \max_{\zb_1, \ldots, \zb_n, \db} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i + \bm{\eta}^\top \db\\
%     \mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \setminus \{\text{root}\} \\
%     & z_{it} \leq d_t \\
%     & z_{it} \in [0, 1], d_t \in \{0,1\}.
% \end{aligned}
% \end{equation}
To do so, we must be able to compute
%To embed decision tree induction as a differentiable hidden layer in a
%neural network, we require access to
the gradients
$\pfrac{\zb}{\bm{\eta}}$ and $\pfrac{\zb}{\qb}$. However, the solutions of  eq.~\ref{eq:ourilp} are discontinuous and piecewise-constant.

To solve this, we relax the integer constraint on $\ab$ to the interval $[0,1]$ and add quadratic regularization $\nicefrac{1}{2}\sum_i \| \zb_i \|_2^2 + \nicefrac{1}{2} \| \ab \|_2^2$.
Rearranging and negating the objective yields 
%\begin{equation}
\begin{align}
   \mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \argmin_{\zb_1, \ldots, \zb_n, \ab} \;\;& \hlf\sum_{i=1}^n \| \zb_i - \qb_i \|^2 + \hlf \| \bm{\eta} - \ab \|^2 \label{eq:qp_prune}
 \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT
\setminus \{\text{root}\}  \nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in [0,1]. \nonumber
\end{align}
The regularization makes the objective strongly convex, so
$\mathrm{T}_{\bm{\eta}}$ is continuous and almost everywhere differentiable~\citep{optnet}. 
Rather than relying on generic solvers,
by using the tree structure of the constraints, we derive an efficient specialized algorithm.
%We then show how this view
%gives a direct, efficient computation of the backward pass.
The main insight, shown below, reframes pruned binary tree learning
as isotonic optimization.
\begin{proposition}\label{prop:iso}
Let $\mathcal{C}= \big\{ \ab \in \mathbb{R}^{|\mathcal{T}|} :
a_t \leq a_{p(t)} ~~\text{for all}~~ t \in \mathcal{T} \setminus \{ \text{root}
\} \big\}.$
Consider
\begin{equation}\label{eq:nested_qp_prune}
\ab^\star = \argmin_{\ab\in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\;
\sum_{t \in \mathcal{T}} \Big( \hlf {(a_t - \eta_t)}^2
+ \sum_{i: a_t \leq q_{it}} \hlf {(a_t - q_{it})}^2 \Big)\,.
\end{equation}
Define%
\footnote{Here $\operatorname{Proj}_{\mathcal{S}}(x)$ is the projection of $x$ onto set $\mathcal{S}$. If $\mathcal{S}$ are box constraints, projection amounts to clipping.}
$[z^\star]_{it} = \operatorname{Proj}_{[0, a_t^\star]}(q_{it})$.
Then, $\mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \zb^\star_1, \ldots, \zb^\star_n, \ab^\star$.
\end{proposition}
\begin{proof}
The constraints and objective function of eq.~\ref{eq:qp_prune} are separable,
so we may push the minimization \wrt $\zb$ inside the objective, resulting in:
\begin{equation}
\argmin_{\ab \in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\; \hlf \| \bm{\eta} - \ab \|^2
+ \sum_{t \in \mathcal{T}} \sum_{i=1}^n
\min_{0 \leq z_{it} \leq a_t} \hlf{({z}_{it} - {q}_{it})}^2\,.
\end{equation}
Each of the inner nested minimizations,
$\min_{0 \leq z_{it} \leq a_t} \hlf (z_{it} - q_{it})^2$
is a one-dimensional projection onto box constraints, with solution
$z^\star_{it} = \operatorname{Proj}_{[0, a_t]}(q_{it})$.
%\begin{equation}\label{eq:z_from_d} z_{it} = {[q_{it}]}_{[0, d_t]}.\end{equation}
We may use this result to eliminate $\zb$ from the objective,
noting that
\begin{equation}
\hlf(z^\star_{it} - q_{it})^2 =
\begin{cases}
\hlf~q_{it}^2, & q_{it} < 0\\
0, & 0 \leq q_{it} < a_t\\
\hlf(a_t - q_{it})^2, & q_{it} \geq a_t\\
\end{cases}
\end{equation}

the first two conditions are constants \wrt $a_t$
%As a function of $a_t$, the first two conditions are constants.
Thus, the objective functions eq.~(\ref{eq:qp_prune}) and eq.~(\ref{eq:nested_qp_prune})
differ by a constant. As their constraints are also the same, they have equivalent minimizers $\ab^\star$.
%This leaves us with the equivalent problem in $\db$,
%\begin{equation}\label{eq:nested_qp_prune}
%\begin{aligned}
    %\min_{\bm{d}} \;\;&
%\sum_t \Big( \hlf {(d_t - \eta_t)}^2
%+ \sum_{i: d_t \leq q_{it}} \hlf {(d_t - q_{it})}^2 \Big) \\
%\mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \\
%& d_t \in [0,1].
%\end{aligned}
%\end{equation}
%After solving this problem, we may use \Eqref{eq:z_from_d} to get
%the optimal $\zb$ (and likewise for gradients, using the chain rule.)
\end{proof}
\begin{algorithm}[t]\small
\caption{Latent decision tree induction via isotonic optimization.\label{alg}}
\begin{algorithmic}[1]
%\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
%\State \textbf{Initialize:}
\State initial partition
$\mathcal{G} \leftarrow \big\{ \{1\}, \{2\}, \cdots \}
\subset 2^\mathcal{T}$
\ForAll {$G \in \mathcal{G}$}
\State $d_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\Comment{Proposition~\ref{prop:scalar_subproblem}}
\EndFor
\While {exists $t$ such that $a_t > a_{p(t)}$}
\State $t_\text{max} \leftarrow \argmax_t \{a_t: a_t > a_{p(t)}\}$
\State merge $G \leftarrow G \cup G'$ where $t \in G$ and $p(t) \in G'$.
\State update  $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\Comment{Proposition~\ref{prop:scalar_subproblem} again}
\EndWhile
\end{algorithmic}
\end{algorithm}
\paragraph{Efficiently inducing trees as isotonic optimization.}
From Proposition~\ref{prop:iso},
notice that eq.~\ref{eq:nested_qp_prune} is an instance of tree-structured isotonic
optimization:
the objective decomposes over \emph{nodes}, and the inequality constraints
correspond to edges in a rooted tree:
\begin{equation}\label{eq:nested_qp_prune_isotonic}
\argmin_{\ab \in \mathcal{C}} \sum_{t \in \mathcal{T}} g_t(a_t)\,,
% \qquad \text{subject to}\qquad d_t \leq d_{p(t)}~\text{for all }t
%\in \cT \setminus \{ \text{root}\},
~~~~\text{where}~~~~ g_t(a_t) =
\hlf {(a_t - \eta_t)}^2
+\!\sum_{i: a_t \leq q_{it}}\!\!\hlf {(a_t - q_{it})}^2  + \iota_{[0,1]}(a_t).
\end{equation}
where $\iota_{[0,1]}(a_t)\!=\!\infty$ if $a_t \notin [0,1]$ and $0$ otherwise.
This problem can be solved by a generalized \emph{pool adjacent violators} (PAV)
algorithm: Obtain a tentative solution by ignoring the constraints, then
iteratively remove violating edges $a_t > a_{p(t)}$ by \emph{pooling together}
the nodes at the end points. At the optimum, the nodes are organized into a
partition $\mathcal{G} \subset 2^\mathcal{T}$, such that if two nodes $t, t'$
are in the same group $G \in \mathcal{G}$, then $a_t = a_t' \coloneqq a_G$.

When the inequality constraints are the edges of a rooted tree, as is the case
here, the PAV algorithm finds the optimal solution in at most $|\mathcal{T}|$ steps,
where each involves updating the $a_G$ value for a newly-pooled group by solving
a one-dimensional subproblem of the form \citep{yu2016exact}\footnote{Compared to \citet{yu2016exact}, our tree inequalities are in the opposite
direction.  This is equivalent to a sign flip of parameter $\ab$, \ie,
to selecting the \emph{maximum} violator rather than the minimum one at each
iteration.}
\begin{equation}\label{eq:scalar_subproblem}
a_G = \argmin_{a \in \bR} \sum_{t \in G} g_t(a)\,,
\end{equation}
resulting in Algorithm~\ref{alg}.
It remains to show how to solve eq.~\ref{eq:scalar_subproblem}. The next
result gives an exact and efficient solution,
with an algorithm that requires finding the nodes with highest
$q_{it}$ (\ie, the nodes where $\xb_i$ is most highly encouraged to traverse).

\begin{proposition}\label{prop:scalar_subproblem}%
The solution to the one-dimensional problem in
eq.~(\ref{eq:scalar_subproblem}) for any $G$ is given by
\begin{equation}\argmin_{a \in \bR} \sum_{t \in G} g_t(a) =
\operatorname{Proj}_{[0,1]}\big(a(k^\star)\big) \quad \text{where}\quad a(k) \coloneqq
\frac{\sum_{t \in G} \eta_t + \sum_{(i,t) \in S(k^\star)} q_{it}}{|G|+k^\star},
\end{equation}
$S(k) = \{j^{(1)}, \ldots, j^{(k)}\}$ is the set of indices $j=(i,t) \in
\{1, \ldots, n\} \times G$ into
the $k$ highest values of $\qb$, \ie,
$q_{j^{(1)}} \geq
q_{j^{(2)}} \geq \ldots \geq
%q_{j^{(k)}} \geq \ldots \geq
q_{j^{(m)}}$,
and $k^\star$ is the smallest $k$ satisfying
$a(k) > q_{j^{(k+1)}}$.
\end{proposition}

\begin{proof}
Let $G \subset \mathcal{T}$ be a subset of (pooled) node indices.
We seek to solve
\begin{equation}\label{eq:subproblem-explicit}
\argmin_{a \in \bR} \sum_{t \in G} g_t(a)
~:=~
\argmin_{a \in [0, 1]} \sum_{t \in G}
\hlf {(a - \eta_t)}^2
+ \sum_{i: a \leq q_{it}} \hlf {(a - q_{it})}^2
\end{equation}
Note that the final summation implicitly depends on the unknown $a$.
But, regardless of the
value of $a$, if $q_{it} \leq q_{i't'}$ and $q_{it}$ is included in the sum, then $q_{i't'}$ must also be included by transitivity.
We may therefore characterize the solution $a^\star$ via the number
of active inequality constraints
$k^\star = \big| \{(i, t) : a^\star \leq q_{i,t} \}\big|$.
We do not know $a^\star$, but it is trivial to find by testing all possible values of $k$. For each $k$, we may find the set $S(k)$ defined in the proposition. For a given $k$, the candidate objective is
\begin{equation}
J_k(a) = \sum_{t \in G} \hlf(a - \eta_t)^2 + \sum_{(i,t) \in S(k)} \hlf(a - q_{it})^2
\end{equation}
and the corresponding $a(k)$ minimizing it can be found by setting the gradient
to zero:
\begin{equation}
J'_k(a)
= \sum_{t \in G} (a - \eta_t)
+ \sum_{(i,t) \in S(k)} (a - q_{i,t})
:= 0
\quad
\iff
\quad
a(k) = \frac{\sum_{t \in G} \eta_t + \sum_{(i,t) \in S(k)} q_{it}}{|G|+k}.
\end{equation}
Since $|S(k)|=k$ and each increase in $k$ adds a non-zero term to the
objective, we must have $J_1\big(a(1)\big) \leq J_1\big(a(2)\big) \leq
J_2\big(a(2)\big) \leq \ldots$,
so we must take $k$ to be as small as possible,
while also ensuring the condition $|\{(i,t) : a(k) \leq q_{it}\}| = k$,
or, equivalently, that $a(k) > q_{j^{([k+1])}}$.
The box constraints may be integrated
at this point via clipping, yielding $a^\star =
\operatorname{Proj}_{[0,1]} \big(a(k^\star)\big)$.
\end{proof}

\paragraph{Benchmarking solver times}
We study the running time of Algorithm~\ref{alg} depending on the number of data points $n$ and the chosen tree depth $D$.
We compare its solving time with the time needed by the popular convex optimization framework {\bf Cvxpy}~\citep{diamond2016cvxpy, agrawal2018rewriting} to solve Problem~\ref{eq:qp_prune} with OSQP solver~\citep{osqp}\footnote{We ran experiments with the commercial solver GUROBI~\citep{gurobi} but didn't find significant differences with using OSQP.}.
We report the solving times in Figure~\ref{fig:alg-time}, where we vary one parameter $n$ or $D$ at a time and fix the other.
The algorithm that we specifically designed to solve Problem~\eqref{eq:qp_prune} is several magnitude faster than the considered generic solver.

\begin{figure}
    \centering
    \subfigure[Fixed number of points $n = 100$]{\includegraphics[width=0.45\textwidth]{figures/time-depth.pdf}
    }\hfill
    \subfigure[Fixed tree depth $D = 3$]{\includegraphics[width=0.45\textwidth]{figures/time-points.pdf}
    }
    \caption{Comparison of Algorithm~\ref{alg}'s running time (ours) with the running time of {\bf Cvxpy} with OSQP solver. $n$ takes values in a range that covers common choices of batch size. Time and $n$ axis are represented in logarithmic scale.
    }
    \label{fig:alg-time}
\end{figure}

\paragraph{Backward pass and efficient implementation details.}
Algorithm~\ref{alg} is a sequence of differentiable operations that can be
implemented \emph{as is} in automatic differentiation frameworks. However,
because of the prominent loops and indexing operations, we opt for a low-level
implementation as a \texttt{C++} extension.
Since the $\qb$ values are constant \wrt $\ab$, we only need to sort them
once as preprocessing. % in \vlad{TODO but should be sth like $\mathcal{O}(d(n \log n))$}.
For the backward pass, rather than relying on automatic
differentiation, we make two remarks about the form of $\ab$.
Firstly, its elements are organized in groups, \ie, $a_t = a_t' = a_G$ for $\{t,
t'\} \subset G$. Secondly, the value $a_G$ inside each group
depends only on  the optimal support set $S^\star_G \coloneqq S(k^\star)$ as
defined for each subproblem  by Proposition~\ref{prop:scalar_subproblem}.
Therefore, in the forward pass, we must store only the node-to-group mappings
and the sets $S^\star_G$. Then, if $G$ is the group of node $t$,
\begin{equation*}
\pfrac{a^\star_t}{\eta_{t'}} = \begin{cases}
\frac{1}{|G| + k^\star},
& 0 < a^\star_t < 1 ~\text{and}~
t' \in G,\\
0,&\text{otherwise.}
\end{cases}
~~
\pfrac{a^\star_t}{q_{it'}} = \begin{cases}
\frac{1}{|G| + k^\star},
& 0 < a^\star_t < 1,
~\text{and}~
(i,t') \in S^\star_G,\\
0,&\text{otherwise.}
\end{cases}.
\end{equation*}


\subsection{The Overall Objective}
% skip connection = concatenation of input and tree path
% MLP = [Linear, Elu, Dropout] * num layers + Linear
We are now able to describe the overall optimization procedure that simultaneously learns tree parameters (a) input traversals $\zb_1, \ldots, \zb_n$; (b) tree pruning $\ab$; and (c) split parameters $\theta_t$. Given this tree, we will additionally learn a function $f_\phi(\zb, \xb)$ to minimize an arbitrary loss $\ell(\cdot)$ as follows,
\begin{equation}
\begin{aligned}
    \min_{\bm{\theta},\bm{\eta},\bm{\phi}}\;\;& \sum_{i=1}^n \ell\big(f_\phi(\xb_i, \zb_i)\big) + \lambda \| \bm{\eta} \|_{\Omega} \label{eq:obj} \\
    \mbox{where}\;\;& \zb_1, \ldots, \zb_n, \ab := \mathrm{T}_{\bm{\eta}}\big(q_{\bm{\theta}}(\xb_1), \ldots, q_{\bm{\theta}}(\xb_n)\big)\,.
\end{aligned}
\end{equation}
Recall $\mathrm{T}_{\bm{\eta}}(\cdot)$ is the solution to the tree program (eq.~\ref{eq:qp_prune}), so we may update the parameters $\bm{\eta}$ and $\bm{\theta}$ by back-propagation. Here we define $q_{\theta}(\xb_i) := \qb_i$ to make explicit the dependence of $\qb_i$ on $\theta$. The regularization $\| \cdot \|_{\Omega}$ can be any norm (in practice we find $\Omega=\infty$ to perform the best.)

%Specifically, $\qb_i$ is given by a  deterministic function $q_{\theta}(\xb_i)$.

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}


% Given a loss function $\ell$
% Given this, we can write the overall objective
% \matt{Working on this}


% In the following, we train via end-to-end back-propagation a Deep Neural Network built as a composition of a Latent Tree (LT) layer followed by a MultiLayer Perceptron (MLP) predictor.
% We also design an optional skip connection between the input $\xb$ and the predictor to circumvent the LT layer, as illustrated in Figure~\ref{fig:arch}.
% The skip connection is particularly useful for regression tasks or when the predictor is a single linear layer, as in these scenarios relying only on the coarse tree representation may hinder results.
% We construct the MLP predictor as a sequence of fully connected layers, with Elu activation~\citep{clevert2015fast} and dropout~\citep{srivastava2014dropout}, followed by a final fully connected layer.
% We refer to the set of predictor's parameters as $\phi$.
% Given a fixed tree depth, the LT layer's training parameters consist of pruning parameter $\bm{\eta}$ and splitting parameters $\theta = \{ \bm{\theta}_t\}_{t \in \cT_B}$.

% Our optimization procedure consists in alternating between solving Problem~\ref{eq:qp_prune}, i.e. computing the tree routing $\bm{z}$, and optimizing the model parameters by gradient descent:

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}

% where $\ell(.)$ is the loss function of choice, depending on the downstream task at hand, measuring the goodness of the predictor's output w.r.t. the target $y$;
% $\lambda$ is the hyper-parameter controlling the trade-off between pruning strength and performance.

% As mentioned before, our formulation allows for integrating any type of split function.
% Depending on the task and on the type of inputs, one could train decision hyper-planes or even more complex functions, such as Convolutional Neural Networks.
% In the following, we make use of decision hyper-planes, and tune whether to apply an Elu activation to their output.
% \vlad{elu is monotonic so I would expect it not to
% change the decision boundary, right? or am I missing something}
% \vale{I'd say that the splits are the same, but the leaf values used as representation are different.}


==> Learning Latent Decision Trees/sections/new_problem.tex <==
\subsection{Learning Tree Parameters}

We now consider the problem of learning the splitting parameters $\theta_t$.
A natural approach would be to do so in the MIP itself, as in the optimal tree literature. However, this would severely restrict allowed splitting functions as even linear splitting functions can only practically run on at most thousands of training inputs \citep{bertsimas2017optimal}. Instead, we propose to learn $s_{\theta_{t}}$ via gradient descent.

To do so, we must be able to compute the partial derivatives
$\partial\ab/\partial\qb$ and $\partial\zb/\partial\qb$. However, the solutions of eq.~\eqref{eq:ourilp} are piecewise-constant, leading to null gradients.
To avoid this, we relax the integer constraint on $\ab$ to the interval $[0,1]$ and add quadratic regularization $-\nicefrac{1}{4}\sum_i (\| \zb_i \|^2 +\| 1 - \zb_i \|^2)$.
The regularization term for $\zb$ is symmetric so that it shrinks solutions toward even left-right splits
(see Figure~\ref{fig:split-z} for a visualization, and the supplementary for a more detailed justification with an empirical evaluation of the approximation gap). Rearranging and negating the objective yields
\begin{figure}%[width=.5\textwidth]
\centering
\input{sections/fig_z.tex}
\caption{\label{fig:split-z}Routing of point $\xb_i$ at node $t$, without pruning, without (left) or with (right) quadratic relaxation. Depending on the decision split $s_{\theta_t}(\cdot)$, $\xb_i$ reaches node $t$'s left child $l$ (right child $r$ respectively) if $z_{il} > 0$ ($z_{ir} > 0$).
The relaxation makes $\zb_i$ continuous and encourages points to have a margin ($| s_{\theta_t}| > 0.5$).}
\end{figure}


\begin{align}
   \mathrm{T}_{\lambda}(\qb_1, \ldots, \qb_n) =  \label{eq:qp_prune} \\ \argmin_{\zb_1, \ldots, \zb_n, \ab} \;\;& \nicefrac{\lambda}{2} \| \ab \|^2 + \hlf\sum_{i=1}^n \| \zb_i - \qb_i -\nicefrac{1}{2} \|^2 \nonumber
 \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT
\setminus \{\text{root}\}  \nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in [0,1]. \nonumber
\end{align}

The regularization makes the objective strongly convex. It follows from convex duality that $\mathrm{T}_{\lambda}$ is Lipschitz continuous
\citep[Corollary 3.5.11]{zalinescu}.
By Rademacher's theorem \citep[Theorem 9.1.2]{borweinlewis}, $\mathrm{T}_{\lambda}$ is thus differentiable almost everywhere.
Generic methods such as OptNet~\citep{optnet} could be used to compute the
solution and gradients. However,
by using the tree structure of the constraints, we next derive an efficient specialized algorithm.
%We then show how this view
%gives a direct, efficient computation of the backward pass.
The main insight, shown below, reframes pruned binary tree learning
as isotonic optimization.

\begin{proposition}\label{prop:iso}
Let $\mathcal{C}= \big\{ \ab \in \mathbb{R}^{|\mathcal{T}|} :
a_t \leq a_{p(t)} ~~\text{for all}~~ t \in \mathcal{T} \setminus \{ \text{root}
\} \big\}.$
Consider $\ab^\star$ the optimal value of
\begin{equation}\label{eq:nested_qp_prune}
\argmin_{\ab\in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}}
\sum_{t \in \mathcal{T}} \Big( \frac{\lambda}{2} a_t^2
+\!\!\sum_{i: a_t < q_{it} + \hlf}\!\!{(a_t - q_{it} - \hlf)}^2 \Big)\,.
\end{equation}
Define%
\footnote{Here $\operatorname{Proj}_{\mathcal{S}}(x)$ is the projection of $x$ onto set $\mathcal{S}$. If $\mathcal{S}$ are box constraints, projection amounts to clipping.}
$\zb_i^\star$ such that $z^\star_{it} = \operatorname{Proj}_{[0, a_t^\star]}(q_{it} + \hlf)$.
Then, $\mathrm{T}_{\lambda}(\qb_1, \ldots, \qb_n) = \zb^\star_1, \ldots, \zb^\star_n, \ab^\star$.
\end{proposition}
\begin{proof}
The constraints and objective of eq.~\eqref{eq:qp_prune} are separable,
so we may push the minimization \wrt $\zb$ inside the objective:
\begin{equation}
\argmin_{\ab \in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \! \frac{\lambda}{2} \| \ab \|^2
\!\!+\!\!\sum_{t \in \mathcal{T}}\!\sum_{i=1}^n
\min_{0 \leq z_{it} \leq a_t} \hlf{({z}_{it} - {q}_{it} - \hlf)}^2\,.
\end{equation}
Each inner minimization
$\min_{0 \leq z_{it} \leq a_t} \hlf (z_{it} - q_{it} - \hlf)^2$
is a one-dimensional projection onto box constraints, with solution
$z^\star_{it} = \operatorname{Proj}_{[0, a_t]}(q_{it} + \hlf)$.
%\begin{equation}\label{eq:z_from_d} z_{it} = {[q_{it}]}_{[0, d_t]}.\end{equation}
We use this to eliminate $\zb$,
noting that each term $\hlf(z^\star_{it} - q_{it} - \hlf)^2$ yields
\begin{equation}
\begin{cases}
\hlf (q_{it} + \hlf)^2, & q_{it} < - \hlf\\
0, & - \hlf \leq q_{it} < a_t - \hlf \\
\hlf(a_t - q_{it} - \hlf)^2, & q_{it} \geq a_t - \hlf.\\
\end{cases}
\end{equation}
The first two branches are constants \wrt $a_t$
The problems in eq.~\eqref{eq:qp_prune} and eq.~\eqref{eq:nested_qp_prune}
differ by a constant and have the same constraints,
therefore they have the same solutions.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=.42\textwidth]{figures/coloring.pdf}
    \caption{One step in the tree isotonic optimization process from Algorithm~\ref{alg}.
    Shaded tubes depict the partition groups $\mathcal{G}$, and the emphasized
arc is the largest among the violated inequalities. The group of $t_{\max}$
    merges with the group of its parent,
    and the new value for the new, larger group $a_G$ is computed.}
    \label{fig:coloring}
\end{figure}

\begin{algorithm}[t]\small
\caption{Pruning via isotonic optimization\label{alg}}
\begin{algorithmic}
%\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
%\State \textbf{Initialize:}
\STATE initial partition
$\mathcal{G} \leftarrow \big\{ \{1\}, \{2\}, \cdots \}
\subset 2^\mathcal{T}$
\FOR {$G \in \mathcal{G}$}
\STATE $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\hfill\COMMENT{Eq.~\eqref{eq:nested_qp_prune_isotonic}, Prop.~\ref{prop:scalar_subproblem}}
\ENDFOR
\REPEAT
\STATE $t_\text{max} \leftarrow \argmax_t \{a_t: a_t > a_{p(t)}\}$
\STATE merge $G \leftarrow G \cup G'$ where $G' \ni t_{\max}$ and $G \ni p(t_{\max})$.
\STATE update  $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\hfill\COMMENT{Eq.~\eqref{eq:nested_qp_prune_isotonic}, Prop.~\ref{prop:scalar_subproblem}}
\UNTIL{ no more violations $a_t > a_{p(t)}$ exist}
\end{algorithmic}
\end{algorithm}

\paragraph{Efficiently inducing trees as isotonic optimization.}

From Proposition~\ref{prop:iso},
notice that eq.~\eqref{eq:nested_qp_prune} is an instance of tree-structured isotonic
optimization:
the objective decomposes over \emph{nodes}, and the inequality constraints
correspond to edges in a rooted tree:
\begin{align}\label{eq:nested_qp_prune_isotonic}
&\argmin_{\ab \in \mathcal{C}} \sum_{t \in \mathcal{T}} g_t(a_t)\,, ~~~~\text{where} \\
% \qquad \text{subject to}\qquad d_t \leq d_{p(t)}~\text{for all }t
%\in \cT \setminus \{ \text{root}\},
 g_t(a_t) =&
\frac{\lambda}{2} a_t^2
+\!\sum_{i: a_t \leq q_{it} + \hlf}\!\!\hlf {(a_t - q_{it} - \hlf)}^2  + \iota_{[0,1]}(a_t). \nonumber
\end{align}
where $\iota_{[0,1]}(a_t)\!=\!\infty$ if $a_t \notin [0,1]$ and $0$ otherwise.
This problem can be solved by a generalized \emph{pool adjacent violators} (PAV)
algorithm: Obtain a tentative solution by ignoring the constraints, then
iteratively remove violating edges $a_t > a_{p(t)}$ by \emph{pooling together}
the nodes at the end points.
Figure~\ref{fig:coloring} provides an illustrative example of the procedure.
At the optimum, the nodes are organized into a
partition $\mathcal{G} \subset 2^\mathcal{T}$, such that if two nodes $t, t'$
are in the same group $G \in \mathcal{G}$, then $a_t = a_{t'} \coloneqq a_G$.

When the inequality constraints are the edges of a rooted tree, as is the case
here, the PAV algorithm finds the optimal solution in at most $|\mathcal{T}|$ steps,
where each involves updating the $a_G$ value for a newly-pooled group by solving
a one-dimensional subproblem of the form \citep{yu2016exact}\footnote{Compared to \citet{yu2016exact}, our tree inequalities are in the opposite
direction.  This is equivalent to a sign flip of parameter $\ab$, \ie,
to selecting the \emph{maximum} violator rather than the minimum one at each
iteration.}
\begin{equation}\label{eq:scalar_subproblem}
a_G = \argmin_{a \in \bR} \sum_{t \in G} g_t(a)\,,
\end{equation}
resulting in Algorithm~\ref{alg}.
It remains to show how to solve eq.~\eqref{eq:scalar_subproblem}. The next
result, proved in the supplementary, gives an exact and efficient solution,
with an algorithm that requires finding the nodes with highest
$q_{it}$ (\ie, the nodes which $\xb_i$ is most highly encouraged to traverse).

\begin{figure}
    \centering
    {\includegraphics[width=0.4\textwidth]{figures/time-D3.pdf}
    }
    \caption{Comparison of Algorithm~\ref{alg}'s running time (ours) with the running time of cvxpylayers~\citep{cvxpylayers2019} for tree depth $D \!=\! 3$, varying $n$.}
    \label{fig:time}
    %$n$ takes values in a range that covers common choices of batch size. Time and $n$ axis are represented in logarithmic scale.}
    %\label{fig:alg-time}
%         \includegraphics[width=0.99\textwidth]{figures/pruning/all-reg.pdf}
% %        \vspace{-3ex}
%         \captionof{figure}{Empty nodes (EN) as we vary $\lambda$.}
        \label{fig:lambda}
\end{figure}

\pagebreak
\begin{proposition}\label{prop:scalar_subproblem}%
The solution to the one-dimensional problem in
eq.~\eqref{eq:scalar_subproblem} for any $G$ is given by
\begin{align}\argmin_{a \in \bR} \sum_{t \in G} g_t(a) =
\operatorname{Proj}_{[0,1]}\big(a(k^\star)\big) \\ \text{where}\quad a(k^\star) \coloneqq
\frac{\sum_{(i,t) \in S(k^\star)} (q_{it} + \hlf)}{\lambda|G|+k^\star}, \nonumber
\end{align}
$S(k) = \{j^{(1)}, \ldots, j^{(k)}\}$ is the set of indices $j=(i,t) \in
\{1, \ldots, n\} \times G$ into
the $k$ highest values of $\qb$, \ie,
$q_{j^{(1)}} \geq
q_{j^{(2)}} \geq \ldots \geq
%q_{j^{(k)}} \geq \ldots \geq
q_{j^{(m)}}$,
and $k^\star$ is the smallest $k$ satisfying
$a(k) > q_{j^{(k+1)}} + \hlf$.
\end{proposition}

Figure~\ref{fig:time} compares our algorithm to a generic differentiable solver (details and additional comparisons in supplementary material).

\paragraph{Backward pass and efficient implementation details.}
Algorithm~\ref{alg} is a sequence of differentiable operations that can be
implemented \emph{as is} in automatic differentiation frameworks. However, because of the prominent loops and indexing operations, we opt for a low-level implementation as a \texttt{C++} extension.
Since the $\qb$ values are constant \wrt $\ab$, we only need to sort them
once as preprocessing, resulting in a overall time complexity of $\mathcal{O}(n |\cT| \log (n |\cT|))$ and space complexity of $\mathcal{O}(n |\cT|)$.
For the backward pass, rather than relying on automatic
differentiation, we make two remarks about the form of $\ab$.
Firstly, its elements are organized in groups, \ie, $a_t = a_t' = a_G$ for $\{t,
t'\} \subset G$. Secondly, the value $a_G$ inside each group
depends only on  the optimal support set $S^\star_G \coloneqq S(k^\star)$ as
defined for each subproblem  by Proposition~\ref{prop:scalar_subproblem}.
Therefore, in the forward pass, we must store only the node-to-group mappings
and the sets $S^\star_G$. Then, if $G$ contains $t$,
\begin{equation*}
\pfrac{a^\star_t}{q_{it'}} = \begin{cases}
\frac{1}{\lambda |G| + k^\star},
& 0 < a^\star_t < 1,
~\text{and}~
(i,t') \in S^\star_G,\\
0,&\text{otherwise.}
\end{cases}
\end{equation*}
As $\mathrm{T}_{\lambda}$ is differentiable almost everywhere, these
expressions yield the unique Jacobian at all but a measure-zero set of
points, where they yield one of the Clarke generalized Jacobians
\citep{clarke_book}.
We then rely on automatic differentiation to propagate gradients from $\zb$ to $\qb$, and from $\qb$ to
the split parameters $\bm{\theta}$: since $\qb$ is defined elementwise via $\min$
functions, the gradient propagates through the minimizing path,
by Danskin's theorem \citep[Proposition B.25,][]{bertsekas-nonlin,danskin_theorem}.
 \subsection{The Overall Objective}
% skip connection = concatenation of input and tree path
% MLP = [Linear, Elu, Dropout] * num layers + Linear

\begin{algorithm}[t]\small
\caption{\label{alg:learn}Learning with decision tree representations.}
\begin{algorithmic}
%\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
%\State \textbf{Initialize:}
\STATE initialize neural network parameters $\bm{\phi},\bm{\theta}$
%(architecture-specific)
\REPEAT
\STATE sample batch $\{\xb_i\}_{i \in B}$
\STATE induce traversals:
\STATE $\{\zb_i\}_{i \in B}, \ab =
\mathrm{T}_\lambda\big(\{q_{\bm{\theta}}(\xb_i)\}\big)$
\hfill\COMMENT{Algorithm~\ref{alg}; differentiable}
\STATE update parameters using
$\nabla_{\{\bm{\theta},\bm{\phi}\}}
\ell(f_{\bm{\phi}} (\xb_i, \zb_i))$
\hfill\COMMENT{autograd}
\UNTIL{convergence or stopping criterion is met}
\end{algorithmic}
\end{algorithm}

% \begin{wrapfigure}[10]{R}{.3\textwidth}
% \input{sections/fig_intro.tex}
% \caption{\label{fig:arch}Model overview.}
% \vspace{-10ex}
% \end{wrapfigure}

We are now able to describe the overall optimization procedure that simultaneously learns tree parameters: (a) input traversals $\zb_1, \ldots, \zb_n$; (b) tree pruning $\ab$; and (c) split parameters $\bm{\theta}$.
Instead of making predictions using heuristic scores over the training points assigned to a leaf (e.g., majority class), we learn a prediction function $f_\phi(\zb, \xb)$ that minimizes an arbitrary loss $\ell(\cdot)$ as follows:
\begin{equation}
\begin{aligned}
    \min_{\bm{\theta},\bm{\phi}}\;\;& \sum_{i=1}^n \ell\big(f_\phi(\xb_i, \zb_i)\big) \label{eq:obj} \\
    \mbox{where}\;\;& \zb_1, \ldots, \zb_n, \ab := \mathrm{T}_{\lambda}\big(q_{\bm{\theta}}(\xb_1), \ldots, q_{\bm{\theta}}(\xb_n)\big)\,.
\end{aligned}
\end{equation}
This corresponds to embedding a decision tree as a layer of a deep neural network (using $\zb$ as intermediate representation) and optimizing the parameters $\bm{\theta}$ and $\bm{\phi}$ of the whole model by back-propagation.
In practice, we perform mini-batch updates for efficient training;
the procedure is sketched in Algorithm~\ref{alg:learn}.
% Recall $\mathrm{T}_{\lambda}(\cdot)$ is the solution to the tree program (eq.~\ref{eq:qp_prune}), so we may update the parameters $\bm{\theta}$ by back-propagation.
Here we define $q_{\theta}(\xb_i) := \qb_i$ to make explicit the dependence of $\qb_i$ on $\bm{\theta}$.
% The regularization $\| \cdot \|_{\Omega}$ can be any norm (in practice we find $\Omega=\infty$ to perform the best.)
% The overall model is .


==> Learning Latent Decision Trees/sections/related.tex <==
The paradigm of \emph{binary tree learning} has the goal of finding a tree that iteratively splits data into meaningful, informative subgroups, guided by some criterion.
%, without any existing trees to guide the learning process.
Binary tree learning appears in a wide variety of problem settings across machine learning. We briefly review work in two learning settings where latent tree learning plays a key role: 1. \emph{Classification/Regression}; and 2. \emph{Hierarchical clustering}. %We also contrast our approach with the field of \emph{latent parse trees} which learn per-instance trees.
Due to the generality of our setup (tree learning with arbitrary split functions, pruning, and downstream objective), our approach can be used to learn trees in any of these settings. Finally, we detail how parts of our algorithm are inspired by recent work in isotonic regression.

\paragraph{Classification/Regression.}
% greedy
Decision trees for classification and regression have a storied history, with early popular methods that include classification and regression trees
\citep[CART, ][]{breiman1984classification}, ID3 \citep{quinlan1986induction}, and C4.5 \citep{quinlan1993c4}. While powerful, these methods are greedy: they sequentially identify `best' splits as those which optimize a split-specific score (often different from the global objective). As such, learned trees are likely sub-optimal for the classification/regression task at hand.
%Furthermore, this score is often different from the overall classification/regression objective, as using this objective as a split score tends to produce poor splits as the tree depth grows \citep{breiman1984classification}.
% probabilistic
To address this, \citet{carreira2018alternating} proposes an alternating algorithm for refining the structure and decisions of a tree so that it is smaller and with reduced error, however still sub-optimal.
Another approach is to probabilistically relax the discrete splitting decisions of the tree \citep{irsoy2012soft,yang2018deep,tanno2019adaptive}. This allows the (relaxed) tree to be optimized \wrt the overall objective using gradient-based techniques, with known generalization
benefits \citep{hardt2016train,hoffer2017train}. Variations on this approach aim at learning tree ensembles termed `decision forests' \citep{kontschieder2015deep,lay2018random,popov2019neural,DBLP:conf/icml/0001PMTM20}. The downside of the probabilistic relaxation approach is that there is no principled way to prune these trees  as inputs pass through all nodes of the tree with some probability.
% MIP
A recent line of work has explored mixed-integer program (MIP) formulations for learning decision trees.
Motivated by the billion factor speed-up in MIP in the last 25 years,
\citet{rudin2018learning} proposed a mathematical programming approach for learning provably optimal decision lists~\citep[one-sided decision trees;][]{letham2015interpretable}.
This resulted in a line of recent follow-up works extending the problem to binary decision trees~\citep{hu2019optimal,lin2020generalized} by adapting the efficient discrete optimization algorithm \citep[CORELS, ][]{angelino2017learning}.
%solving related problems and/or improving the MIP
Related to this line of research, \citet{bertsimas2017optimal} and its follow-up works~\citep{gunluk2018optimal,aghaei2019learning,verwer2019learning,aghaei2020learning} phrased the objective of CART as an MIP that could be solved exactly.
Even given this consistent speed-up all these methods are only practical on datasets with at most thousands of inputs \citep{bertsimas2017optimal} and with non-continuous features.
Recently, \citet{DBLP:conf/nips/ZhuMPNK20} addressed these tractability concerns principally with a data selection mechanism that preserves information.
Still, the out-of-sample generalizability of MIP approaches is not well-studied, unlike stochastic gradient descent learning.

\paragraph{Hierarchical clustering.}
Compared to standard flat clustering, hierarchical clustering provides a structured organization of unlabeled data in the form of a tree. To learn such a clustering the vast majority of methods are greedy and work in one of two ways: 1. \emph{Agglomerative}: a `bottom-up' approach that starts each input in its own cluster and iteratively merges clusters; and 2. \emph{Divisive}: a `top-down' approach that starts with one cluster and recusively splits clusters  \citep{zhang1997birch,widyantoro2002incremental,krishnamurthy2012efficient,dasgupta2016cost,kobren2017hierarchical,moseley2017approximation}. These methods suffer from similar issues as greedy approaches for classification/regression do: they may be sub-optimal for optimizing the overall tree. Further they are often computationally-expensive due to their sequential nature. Inspired by approaches for classification/regression, recent work has designed probabilistic relaxations for learning hierarchical clusterings via gradient-based methods \citep{monath2019gradient}.

Our work takes inspiration from both the MIP-based and gradient-based
approaches. Specifically, we frame learning the discrete tree parameters as an MIP, which we sparsely relax to allow continuous parameters to be optimized by argmin differentiation methods.

\paragraph{Argmin differentiation.}
Solving an optimization problem as a differentiable module within a parent problem tackled with gradient-based optimization methods is known as argmin differentiation, an instance of bi-level optimization \citep{colson2007overview,gould}. This situation arises in as diverse scenarios as hyperparameter optimization
\citep{pedregosa2016hyperparameter}, meta-learning \citep{metalearning}, or structured prediction \citep{ves,domke,sparsemap}.
General algorithms for quadratic \cite{optnet} and disciplined convex
programming \citep[Section 7,][]{amos2019differentiable,cvxpylayers2019,diffcone} have
been given, as well as expressions for more specific cases like isotonic
regression \citep{djolonga}. Here, by taking advantage of the structure of the decision tree induction problem, we obtain a direct, efficient algorithm.

\paragraph{Latent parse trees.} Our work resembles but should not be confused with the latent
parse tree literature in natural language processing
\citep{yogatama2017learning,lapata,choi2018learning,williams2018latent,sparsemapcg,caio-iclr,caio-acl,maillard2019jointly,kimcompound,kimrnng}.
% These works learn unsupervised constituency or
% dependency parsers that induce a syntactic representation of for each training
% or test sentence, in order to help with some downstream task (\eg, sentiment
% classification). In contrast, for a dataset, our work induces a single
% \emph{decision tree}, which each sample traverses stochastically but sparsely, yielding an encoding based on the path taken.
% %
% While the goals and models are quite different, the underlying toolkit of
% differentiable optimization appears in some of these works, and it is possible
% that further connections will emerge in the future.  %\vlad{I commented most of
% %what was here, since it seems distracting as this task is really quite
% %substantially different.}
%The goal of these works are to learn novel parse trees to improve performance on downstream tasks such as sentiment analysis \citep{socher2013recursive} and textual entailment \citep{bowman2016fast}.
%grew out of the success of tree-structured recursive neural networks (TreeRNNs) \citep{socher2011semi}. TreeRNNs produce structured representations by leveraging sentence parse trees, which have have been shown to be useful for sentiment analysis \citep{socher2013recursive} and textual entailment \citep{bowman2016fast}. Instead, of using existing parse trees, latent parse tree methods learn these trees without supervision to produce improved representations for downstream tasks.
%
%Note that these works differ from other popular works on parse tree learning and program induction, which learn models given data on `correct' trees \citep{vinyals2015grammar,dyer2016recurrent,aharoni2017towards,kusner2017grammar,yin2017syntactic,alvarez2017tree,chen2018towards,chen2018tree,shiv2019novel}.
This line of work has a different goal than ours: to induce a tree for each
individual data point (e.g., sentence). In contrast, our work aims to learn a
single tree, for all instances to pass through.

\paragraph{Isotonic regression.} Also called monotonic regression, isotonic regression \citep{barlowstatistical} constrains the regression function to be non-decreasing/non-increasing. This is useful if one has prior knowledge of such monotonicity (\eg, the mean temperature of the climate is non-decreasing). A classic algorithm is pooling-adjacent-violators (PAV),
which optimizes the pooling of adjacent points that violate the monotonicity constraint
\citep{barlowstatistical}. This initial algorithm has been generalized and incorporated into convex programming frameworks (see \citet{mair2009isotone} for an excellent summary of the history of isotonic regression and its extensions). Our work builds off of the generalized PAV (GPAV) algorithm of \citet{yu2016exact}.


==> sections/architecture.tex <==
\newsavebox{\miniz}
\savebox{\miniz}{
\begin{tikzpicture}[
  scale=1,
  every node/.style={inner sep=0pt, outer sep=0pt, draw,circle,minimum size=3pt},
  level 1/.style= {sibling distance=12pt},
  level 2/.style= {sibling distance=7pt},
  level distance=7pt
]
\node[fill=black] at (0, 0) {}
  child{node[fill=black!20] {}
    child{node[]{}}
    child{node[fill=black!20]{}}}
  child{node[fill=black!70] {}
    child{node[]{}}
    child{node[fill=black!70]{}}};
\end{tikzpicture}
}
%
\begin{tikzpicture}[scale=1]
\node at (1.4, 1.5) {(a)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$y$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{$\operatorname{Affine}([\xb;\zb])$} (y);
\end{tikzpicture}
%
\begin{tikzpicture}[scale=1]
\node at (1.4, 1.5) {(b)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$y$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{$\operatorname{MLP}([\xb;\zb])$} (y);
\end{tikzpicture}
%
\begin{tikzpicture}[scale=1]
\node at (1, 1.5) {(c)};
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2, 0) {$y$};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathcal{LT}_\eta\big(\qb(\xb)\big)$} (z);
\draw[->] (z) -- node[above,font=\scriptsize] {$\operatorname{MLP}(\zb)$} (y);
\end{tikzpicture}




==> sections/experiments_arxiv.tex <==
\begin{wrapfigure}[10]{R}{.3\textwidth}
\input{sections/fig_intro.tex}
\caption{\label{fig:arch}Model overview.}

\end{wrapfigure}
In this section we showcase our method on both: (a) \emph{Classification/Regression} for tabular data, where tree-based models have been demonstrated to have superior performance over MLPs \citep{popov2019neural}; and (b) \emph{Hierarchical clustering} on unsupervised data. Our experiments demonstrate that our method leads to predictors that are competitive with state-of-the-art tree-based approaches. 
% Given the derived exact solution for computing the path of each node through the
% tree $(\zb_i)$, our overall learning procedure learns the split function weights
% and the pruning parameters by backpropagation.
% As such, our tree induction can be integrated into deep neural networks for a
% variety of tasks and loss functions.
% In this section, we showcase this for two different tasks, namely supervised learning on tabular datasets and hierarchical clustering.
Further we visualize the trees learned by our method, and how sparsity is easily adjusted by tuning the regularization parameter $\lambda$. 

\paragraph{Architecture details.} 
We use a linear function or a multi-layer perceptron ($L$ fully-connected layers with Elu activation~\citep{clevert2015fast} and dropout) for $f_\phi(\cdot)$ and choose between linear or linear followed by Elu splitting functions $s_\theta(\cdot)$ (we limit 
%these possibilities 
the search for simplicity, there are no restrictions 
%for these choices 
except differentiability).

% These experiments are designed to show how our tree learning methodology can be flexibly adapted to different problem settings. 

% can be adapted to distinctive problem settings, 

% can be plugged into any model and even applied to raw inputs, yielding results comparable to state-of-the-art methods.


% TO ADD:
% We allow hyperparameter selection to decide on (a) $\lambda$; (b) the learning rate for solving eq.~\eqref{eq:obj}; (c) whether to use a linear function or a simple multi-layer perceptron for $f_\phi(\cdot)$; and (d) between linear or linear followed by an Elu activation \citep{clevert2015fast} splitting functions $s_\theta(\cdot)$ (we limit these possibilities for simplicity, there are no restrictions for these choices except differentiability).
%\begin{figure}[t!]
%\input{sections/architecture.tex}
%\caption{\label{fig:arch}Architecture \vlad{todo}.}
%\end{figure}
% Three settings /  model architectures:
% - [x; z] -> y (with skip connection) and linear predictor
% - [x; z] -> y (with skip connection) and MLP predictor
% - x -> z -> y (without skip connection) and MLP predictor


\subsection{Supervised Learning on Tabular Datasets}
Our first set of experiments is on supervised learning with heterogeneous tabular datasets, where we consider both regression and binary classification tasks.
We minimize the Mean Squared Error (MSE) on regression datasets and the Binary Cross-Entropy (BCE) on classification datasets.
% \paragraph{Baselines.}
We compare our results with tree-based architectures, which either train a single or an ensemble of decision trees.
Namely, we compare to the greedy classification and regression trees (CART)~\citep{breiman1984classification} and to the optimal decision tree learner~\citep[OPTREE;][]{bertsimas2017optimal}. %, but upper bounding its tree depth.
We also consider two baselines with probabilistic routing:
deep neural decision trees \citep[DNDT;][]{yang2018deep}
% , which learns a decision tree with axis-aligned differentiable binning functions and soft routing;
and deep neural decision forests~\citep{kontschieder2015deep} configured to use an ensemble size of 1 (NDF-1).
As for the ensemble baselines, we compare to NODE~\citep{popov2019neural}, the state-of-the-art method for training a forest of differentiable oblivious decision trees on tabular data, and to XGBoost~\citep{Chen:2016:XST:2939672.2939785}, a scalable tree boosting method.
% Similarly to our tree learning procedure, NODE's decision tree learning routine can be integrated in Deep Learning architectures and trained with back-propagation.
% As a downside, only oblivious trees can be trained and an ensemble of trees has to be built for good performance.
% \paragraph{Datasets.}
%
We carry out the experiments on the following datasets: \citep{mldata}
%\begin{itemize}
%\item {\bf Year.} Regression task constructed from the Million Song Dataset
%\citep{msd,mldata}.
%\item {\bf Microsoft.}
%Regression approach to the MSLR-Web10k Query--URL relevance prediction for learning to rank \citep{mslr}.
%\item {\bf Yahoo.} Regression approach to the C14 learning-to-rank challenge. \vlad{check}
%\item {\bf Click.} Binary classification for link click prediction based on the KDD Cup 2012
%dataset, encoded and subsampled following \citet{popov2019neural}.
%\item {\bf Higgs.} Binary classification for predicting Higgs boson--producing
%events. \citep{higgs,mldata}
%\end{itemize}
\textbf{Regression.}
{\em Year} \citep{msd}:
Temporal regression task constructed from the Million Song Dataset;
{\em Microsoft} \citep{mslr}:
Regression approach to the MSLR-Web10k Query--URL relevance prediction for
learning to rank;
{\em Yahoo} \citep{chapelle2011yahoo}: Regression approach to the C14 learning-to-rank challenge.
\textbf{Binary classification.}
{\em Click}: Link click prediction based on the KDD Cup 2012
dataset, encoded and subsampled following \citet{popov2019neural};
{\em Higgs} \citep{higgs}: prediction of Higgs boson--producing
events.

For all tasks, we follow the preprocessing and task setup from
\citep{popov2019neural}.
%the preprocessed datasets are available at \vlad{TODO}.
All datasets come with training/test splits.
We make use of 20\% of the training set as validation set for selecting the best model over the epochs and for tuning the hyperparameters.
We tune the hyperparameters for all methods but for OPTREE, as its long training time makes hyper-parameter tuning unfeasible. Details are provided in the supplementary.
Finally, we optimize eq.~\eqref{eq:obj} and all neural network methods (DNDT, NDF, and NODE) using the Quasi-Hyperbolic Adam~\citep{ma2018quasi} stochastic gradient descent method, with default parameters and batch size equal to $512$.
Table~\ref{tab:tabular} reports the obtained results.\footnote{DNDT, OPTREE and NDF handle only classification tasks.} 
Unsurprisingly, ensemble methods outperfom single-tree ones on all datasets, although at the cost of being harder to visualize/interpret. 
Our method has the advantage of (a) generalizing to any task; (b) outperforming or coming in second for all single-tree methods; (c) approaching the performance of ensemble-based methods.
%Among single-tree methods, ours has the advantage of generalizing to any task and having the best trade-off between prediction accuracy and training time (see Figures~\ref{fig:time-click} and~\ref{fig:time-higgs}).

% \begin{table}
% 	\begin{minipage}{0.7\linewidth}
% 		\label{tab:clust}
%         \caption{Results for hierarchical clustering. We report average and standard deviations of Dendrogram Purity over $4$ runs. Best results and all within a standard deviation from it are in bold.
%         % \vlad{make sure to explain what bold means}
%         }
%         \vspace{1ex}
%         \begin{center}
%             % \begin{tabular}{lcc}
%             % {\bf METHOD}  &{\bf GLASS} &{\bf COVTYPE} \\
%             % \hline \\
%             % Ours         & $\mathbf{0.494\pm0.025}$ & $\mathbf{0.467\pm0.006}$ \\
%             % gHHC             &$0.463\pm0.002$ & $0.444\pm0.005$ \\
%             % HKMeans             &$\mathbf{0.508\pm0.008}$ & $0.440\pm0.001$ \\
%             % BIRCH             &$0.429\pm0.013$ & $0.440\pm0.002$ \\
%             % \end{tabular}
%             \begin{tabular}{clccc}
%  & method  &{\bf YEAR} &{\bf MICROSOFT} &{\bf YAHOO} \\
%  \hline \\
% \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Single Tree}}}
% & CART & $97.40 \pm 0.37$ & $0.6914 \pm 3\text{e-}3$ & $0.6190 \pm 3\text{e-}3$ \\
% & DNDT    & - & - & - & $0.4866 \pm 1\text{e-}2$ & OOM\\
% & OPTREE  & - & - & - & $0.4100 \pm 4\text{e-}2$ & OOT\\
% & NDF-1   & - & - & - & $\bm{0.3344 \pm 5\text{e-}4}$ & $\bm{0.2644 \pm 8\text{e-}4}$\\
% & Ours    &$\bm{77.52\pm0.50}$ & $\bm{0.5772\pm12\text{e-}4}$ & $\bm{0.5937 \pm 6\text{e-}4}$ & $0.3383 \pm 15\text{e-}4$ & $0.2995\pm16\text{e-}4$\\
% \hline \\
% \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
% & NODE     &$\bm{76.21 \pm 0.12}$ & $0.5570 \pm 2\text{e-}4$ & $0.5692\pm2\text{e-}4$ & $\bm{0.3312 \pm 2\text{e-}3}$ & $\bm{0.2101\pm5\text{e-}4}$ \\
% & XGBoost  &$78.53 \pm 0.09$ & $\bm{0.5544 \pm 1\text{e-}4}$ & $\bm{0.5420\pm4\text{e-}4}$ & $\bm{0.3310 \pm 2\text{e-}3}$ & $0.2328 \pm 3\text{e-}4$\\
% \end{tabular}
%         \end{center}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.3\linewidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{figures/pruning/all-reg.pdf}
%         \vspace{-3ex}
%         \captionof{figure}{Number of empty nodes (EN) as a function of $\lambda$.}
%         \label{fig:lambda}
% 	\end{minipage}
% \end{table}

\begin{table}[t]
\caption{Results on tabular datasets. We report average and standard deviations over $4$ runs of MSE for regression datasets: {\em Year}, {\em Microsoft} and {\em Yahoo}, and error rate for classification datasets: {\em Click} and {\em Higgs}. Best result, and those within a standard deviation from it, for each family of algorithms (single tree or ensemble) are in \textbf{bold}. Dashes `-' indicate that the method cannot be run (i.e., a method is designed only for classification). Experiments are run on a machine with 16 CPUs and 63GB of RAM, with a training time limit of $3$ days. We denote methods that exceed this memory and training time as OOM and OOT, respectively.}
\label{tab:tabular}
\begin{center}
\begin{tabular}{clccccc}
 &{\bf METHOD}  &{\bf YEAR} &{\bf MICROSOFT} &{\bf YAHOO} &{\bf CLICK} &{\bf HIGGS}\\
 \hline \\
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Single Tree}}}
& CART & $97.40 \pm 0.37$ & $0.6914 \pm 3\text{e-}3$ & $0.6190 \pm 3\text{e-}3$ & $0.3780 \pm 6\text{e-}3$ & $0.3220 \pm 1\text{e-}3$\\
& DNDT    & - & - & - & $0.4866 \pm 1\text{e-}2$ & OOM\\
& OPTREE  & - & - & - & $0.4100 \pm 4\text{e-}2$ & OOT\\
& NDF-1   & - & - & - & $\bm{0.3344 \pm 5\text{e-}4}$ & $\bm{0.2644 \pm 8\text{e-}4}$\\
& Ours    &$\bm{77.52\pm0.50}$ & $\bm{0.5772\pm12\text{e-}4}$ & $\bm{0.5937 \pm 6\text{e-}4}$ & $0.3383 \pm 15\text{e-}4$ & $0.2995\pm16\text{e-}4$\\
\hline \\
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ens.}}}
& NODE     &$\bm{76.21 \pm 0.12}$ & $0.5570 \pm 2\text{e-}4$ & $0.5692\pm2\text{e-}4$ & $\bm{0.3312 \pm 2\text{e-}3}$ & $\bm{0.2101\pm5\text{e-}4}$ \\
& XGBoost  &$78.53 \pm 0.09$ & $\bm{0.5544 \pm 1\text{e-}4}$ & $\bm{0.5420\pm4\text{e-}4}$ & $\bm{0.3310 \pm 2\text{e-}3}$ & $0.2328 \pm 3\text{e-}4$\\
\end{tabular}
\end{center}
\end{table}

\subsection{Self-Supervised Hierarchical Clustering}\label{sec:clust}
To show the versatility of our method, we carry out a second set of experiments on hierarchical clustering tasks. Inspired by the recent success of self-supervised learning approaches \citep{lan2019albert,he2020momentum}, we learn a tree for hierarchical clustering in a self-supervised way. Specifically, we regress a subset of input features from the remaining features, minimizing the MSE. This allows us to use eq.~\eqref{eq:obj} to learn a hierarchy (tree). 
%This time, our method is trained in a self-supervised way, by regressing two of the available input features and minimizing the Mean Squared Error.
%Even though no supervision on the class labels is provided at training, we expect the constructed tree to group points of the same class in order to have good performance on the downstream task.
%\vlad{is there some paper we can cite for this way of doing self supervision?}
To evaluate the quality of the learned trees, we compute its dendrogram purity \citep[DP;][]{monath2019gradient}.
DP measures the ability of the learned tree to separate points from different classes, and corresponds to the expected purity of the least common ancestors of points of the same class.
%This score, however, does not account for the existing hierarchy between classes.
% For image data, we follow SimCLR's framework
% \citep{chen2020simple},
% with the LT block as encoder and a MLP as projection head,
% NT-Xent \citep{sohn,wu2018unsupervised,oord2018representation} as contrastive loss;
% \vlad{what specifically is spatial data? just ALOI? digits too?}
% \vale{just ALOI now, because the transformations proposed in SimCLR don't seem to work on DIGITS. for DIGITS, I am now regressing half of the image.}

We experiment on the following datasets: {\em Glass} \citep{mldata}:
glass identification for forensics, and {\em Covtype}
\citep{blackard1999comparative,mldata}: cartographic variables for forest cover
type identification.
%\begin{itemize}
%\item {\bf Glass.} Glass identification dataset for forensics \citep{mldata}.
%\item {\bf Covtype.} Cartographic variables for forest cover type prediction.
%\citep{blackard1999comparative,mldata}.
% \item {\bf ALOI.} Amsterdam Library of Object Images
% \citep{geusebroek2005amsterdam}.
% \item {\bf Digits.} NIST handwritten digit images
% \citep{alpaydin1998cascading,mldata}
%\end{itemize}
For {\em Glass}, we regress features `Refractive Index' and `Sodium,' and for
{\em Covtype} the horizontal and vertical `Distance To Hydrology.'
We split the datasets into training/validation/test sets, with sizes 60\%/20\%/20\%. Here we only consider linear $f_\phi$. 
%For this set of experiments, the number of fully connected layers of the MLP predictor is set to $0$, resulting in a linear predictor.
As before, we optimize Problem~\ref{eq:obj} using the Quasi-Hyperbolic Adam
algorithm, with batch size equal to $512$ for {\em Covtype} and $8$ for {\em Glass}, and tune the hyper-parameters using the validation set.

As baselines, we consider:
BIRCH~\citep{zhang1996birch} and Hierarchical KMeans (HKMeans), the standard methods for performing clustering on large datasets; and the recently proposed gradient-based Hyperbolic Hierarchical Clustering (gHHC)~\citep{monath2019gradient} designed to construct  trees in hyperbolic space.
Table~\ref{tab:clust} reports the dendrogram purity scores for all methods. Our method matches or outperforms all methods, even though not specifically tailored to hierarchical clustering.
%Even if our method is not specifically designed for hierarchical clustering problems, it achieves performance comparable or better than baselines.
\begin{table}
\caption{Results for hierarchical clustering. We report average and standard deviations of {\em dendrogram purity} over four runs. Best results and all within a standard deviation from it are in bold.}
%        \vspace{1ex}
\begin{center}
    \begin{tabular}{lcc}
    {\bf METHOD}  &{\bf GLASS} &{\bf COVTYPE} \\
    \hline \\
    Ours         & $\mathbf{0.494\pm0.025}$ & $\mathbf{0.467\pm0.006}$ \\
    gHHC             &$0.463\pm0.002$ & $0.444\pm0.005$ \\
    HKMeans             &$\mathbf{0.508\pm0.008}$ & $0.440\pm0.001$ \\
    BIRCH             &$0.429\pm0.013$ & $0.440\pm0.002$ \\
    \end{tabular}
\end{center}
\label{tab:clust}
\end{table}

% We further analyze the trees learned on {\em Glass} dataset with the proposed self-supervised procedure.
\paragraph{Tree Pruning}
The hyper-parameter $\lambda$ in eq.~\ref{eq:obj} controls how aggressively the tree is pruned, hence the amount of tree splits that are actually used to make decisions.
This is a fundamental feature of our framework as it allows to smoothly trim the portions of the tree that are not necessary for the downstream task, resulting in lower computing and memory demands at inference. % as the tree representation, and the model in general, can be compressed.
In Figure~\ref{fig:pruning}, we study the effects of pruning on the tree learned on {\em Glass} with a depth fixed to $D \!=\! 3$.
We report how inputs are distributed over the learned tree for different values of $\lambda$.
We notice that the number of empty nodes, \ie, nodes that are not traversed by any data point, increases together with $\lambda$ up to a certain value in order not to significantly deteriorate results (as measured by dendrogram purity).
%Moreover, even without the regularization term ($\lambda=0$), our method removes nodes that have few points assigned to them. % adding the pruning regularization effectively removes those nodes that have few assigned points when $\lambda=0$.

\begin{figure}
    \centering
    \includegraphics[width=.9\textwidth]{figures/pruning/pruned_all.pdf}
    \caption{{\em Glass} tree routing distribution, in rounded percent of dataset,
for $\lambda$ left-to-right in $\{0, 0.001, 0.1\}$.
The larger $\lambda$, the more nodes are pruned.
We report dendrogram purity (DP) and total empty nodes (EN).
\label{fig:pruning}}
\end{figure}

\paragraph{Class Routing}
In order to gain insights on the latent structure learned by our method, we study how points are routed through the tree, depending on their class.
The {\em Glass} dataset is particularly interesting to analyze as its classes come with an intrinsic hierarchy, \eg, with superclasses \textit{Window} and \textit{NonWindow}.
%Still, we expect points from the same class or super class to traverse the tree in a similar way.
Figure~\ref{fig:class-routing} reports the class routes for four classes.
As the trees are constructed without supervision, we do not expect the structure to exactly reflect the class partition and hierarchy. Still, we observe that points from the same class or super-class to traverse the tree in a similar way.
Indeed, trees for class \textit{Build}~\ref{fig:build} 
and class \textit{Vehicle}~\ref{fig:vehicle}, which both belong to \textit{Window} super-class, share similar paths, unlike the classes Containers~\ref{fig:cont} 
and Headlamps~\ref{fig:head}.

\begin{figure}
    \centering
    \subfigure[Window-Float-Build]{\label{fig:build}\includegraphics[width=0.4\textwidth]{figures/glass/class0.pdf}}\hfill
    \subfigure[Window-Float-Vehicle]{\label{fig:vehicle}\includegraphics[width=0.4\textwidth]{figures/glass/class2.pdf}}\hfill
    \subfigure[NonW-Containers]{\label{fig:cont}\includegraphics[width=0.4\textwidth]{figures/glass/class4.pdf}}\hfill
    \subfigure[NonW-Headlamps]{\label{fig:head}\includegraphics[width=0.4\textwidth]{figures/glass/class6.pdf}}
    % \includegraphics[width=\textwidth]{figures/glass/hier_clustering.pdf}
    \caption{Class routing distributions on {\em Glass}, with distributions normalized over each depth level. The decision tree was trained with optimal hyper-parameters, (depth $D\!=\!6$), but we plot nodes up to level $D\!=\!4$ for visualization ease.
    }
    \label{fig:class-routing}
\end{figure}



% tabular datasets
% hierarchical clustering
%   - linear splits
%   - contrastive learning images


==> sections/fig_intro.tex <==
\newsavebox{\miniz}
\savebox{\miniz}{
\begin{tikzpicture}[
  scale=1,
  every node/.style={inner sep=0pt, outer sep=0pt, draw,circle,minimum size=3pt},
  level 1/.style= {sibling distance=12pt},
  level 2/.style= {sibling distance=7pt},
  level distance=7pt
]
\node[fill=black] at (0, 0) {}
  child{node[fill=black!20] {}
    child{node[]{}}
    child{node[fill=black!20]{}}}
  child{node[fill=black!70] {}
    child{node[]{}}
    child{node[fill=black!70]{}}};
\end{tikzpicture}
}
%
\begin{tikzpicture}[scale=.86]
\node[circle,draw] (x) at (0, 1.5) {$\xb$};
\node[circle,draw,align=center,inner sep=0pt,outer sep=0pt] (z) at (0, 0) {$\zb$ \\ \usebox{\miniz}};
\node[circle,draw] (y) at (2.8, 0) {$\ell$};
\node[inner sep=0pt,outer sep=0pt] (temp) at (1.2, 0) {};
\draw[->] (x) -- node[left,font=\scriptsize] {$\mathrm{T}_{\lambda}\big(q_{\bm{\theta}}(\xb)\big)$} (z);
\draw (z) -- (temp);
\draw[dashed] (x) to (temp);
\draw[->] (temp) -- node[above, font=\scriptsize]{${f}_{\bm{\phi}}(\xb,\zb)$} (y);
\end{tikzpicture}


==> sections/methods_arxiv.tex <==
Given inputs $\{\xb_i\}_{i=1}^n$,  %where each $\xb \in [0,1]^p$.
our goal is to learn a latent binary decision tree $\cT$ with maximum depth $D$. This tree sends each input $\xb$ through branching nodes to a specific leaf node  in the tree. Specifically, all branching nodes $\cT_B \subset \cT$ split an input $\xb$ by forcing it to go to its left child if
$s_\theta(\xb) < 0$,
and right otherwise. There are three key parts of the tree that need to be identified: 1. The \emph{continuous} parameters $\theta_t \in \mathbb{R}^d$ that describe how $s_{\theta_t}$ splits inputs at every node $t$; 2. The \emph{discrete} paths $\zb$ made by each input $\xb$ through the tree; 3. The \emph{discrete} choice $a_t$ of whether a node $t$ should be active or pruned. We describe how to learn each of these below.
% Our strategy will be to first fix splitting parameters $\theta_t$ for all $t$. Then to introduce a mixed-integer program (MIP) for learning paths $\zb$ and pruning $d_t$. %We then modify this to a mixed-integer program (MIP) that solves both 2 and 3.
% Finally we sparsely relax the MIP to allow for argmin differentiation to simultaneously solve for $\theta_t$.

% Our goal is to learn $\cT$ that is good for some downstream task. To do so,
% %by learning a scoring vector $\{ \boldsymbol{\eta} \}_{i=1}^n$ where $\boldsymbol{\eta} \in \mathbb{R}^T$ that describes the benefit of sending $\xb_i$ along a particular route in the tree.
% we will learn the splitting parameters of the tree $\{ \theta_t,\}_{t \in \cT_B}$.
% % For these parameters we impose the following constrain
% % \begin{align}
% %     \sum_{j=1}^d a_{jt} = 1, \;\;\; 0 \leq \ab_t, b_t \leq 1,
% %     \;\;\; \forall t \in \cT_B. \nonumber
% % \end{align}
% Specifically, let $\cT$ have maximum depth $D$. %This tree has at most $T \!=\! 2^{(D+1)} \!-\! 1$.
%nodes that are one of two types: (a) \emph{branching nodes}: $\cT_B$; and (b) \emph{leaf nodes}: $\cT_L$. Branching nodes split an  %$\ab^\top \xb < b$

\subsection{Tree-Traversal \& Pruning Programs}

Imagine the splitting functions of the tree $s_{\theta_t}$ are fixed. Given this, the following integer linear program (ILP) describes how inputs $\xb$ traverse the tree. The solution $z_{it} \in \{0,1\}$ indicates if $\xb_i$ reaches node $t \in \cT$ (for notational simplicity let $\zb_i \in \{0,1\}^{|\cT|}$ be the vectorized indicator for $\xb_i$),
\begin{align}
    \max_{\zb_1, \ldots, \zb_n} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
    \mbox{s.t. } \forall i \in [n],\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    & r_{it} = \min \{ s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_R(t), \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    & l_{it} = \min \{ -s_{\theta_{t'}}(\xb_i), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\top \xb
    & z_{it} \in \{0, 1\}. \nonumber
\end{align}
Here $A_L(t)$ is the set of ancestors of node $t$ whose left child must be followed to get to $t$, and similarly for $A_R(t)$. The quantities $q_{it}$ (where $\qb_i \in \mathbb{R}^{|\cT|}$ is the tree-vectorized version of $q_{it}$) describe the `reward' of sending $\xb_i$ to node $t$. This is based on how well the splitting functions leading to $t$ are satisfied ($q_{it}$ is positive if all splitting functions are satisfied and negative otherwise).

Notice that the solution is unique so long as $s_{\theta_{t}}(\xb_i)
\!\neq\! 0$ for all $t \in \cT, i \in \{1, \ldots, n\}$ (\ie, $s_{\theta_{t}}(\xb_i) \!=\! 0$ means there is no preference to split $\xb_i$ left or right). Further note that \textbf{the integer constraint on $z_{it}$ can be relaxed to an interval constraint $z_{it} \in [0, 1]$ without loss of generality}. This is because if $s_{\theta_{t}}(\xb_i)
\neq 0$ then $z_t=0$ if and only if $q_t < 0$ and $z_t=1$ when $q_t > 0$ (and $q_t \neq 0$).


% To do so, we will first introduce an inner optimization problem: a linear program (LP) that describes how a set of inputs $\{\xb_i\}_{i=1}^b$ traverses through the tree given fixed splitting parameters $\{ \theta_t\}_{t \in \cT_B}$. Specifically let $z_{it} \in [0,1]$ indicate if $\xb_i$ reaches node $t \in \cT$ (let $\zb_i \in [0,1]^T$ be the vector indicator every tree node for $\xb_i$)
% \begin{align}
%     \max_{\zb_1, \ldots, \zb_b} \;\;& \sum_{i=1}^b \zb_i^\top \qb_i \label{eq:lp_no_prune} \\
%     \mbox{s.t.}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
%     & l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ % b_{t'} - \ab_{t'}^\toeq.p \xb
%     & z_{it} \in [0, 1] \nonumber
% \end{align}

While the above program works for any fixed tree, we would like to be able to also learn the structure of the tree itself. Let $\eta_t \in \bR$ be our preference for pruning/keeping node $t$ (larger $\eta_t$ indicates node $t$ should be kept). 
To encourage this pruning preference while ensuring connectivity,
we introduce an additional optimization variable $a_t \in \{0,1\}$, indicating if node $t \in \cT$ is active (if $1$) or pruned (if $0$).
We may now adapt eq.~\ref{eq:lp_no_prune} into the following pruning-aware mixed integer program (MIP):
%to learn a valid pruning that obeys $\eta_t$:
%(where $\bm{\eta} \in [0,1]^{|\mathcal{T}|}$ is $\eta_t$ vectorized for all $t$):
\begin{align}
    \max_{\zb_1, \ldots, \zb_n, \ab} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i + \boldsymbol{\eta}^\top \ab \label{eq:ourilp} \\ %\label{eq:ilp_prune} \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} \}\nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in \{0,1\}. \nonumber
    %q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
    %& r_{it} = \min \{ s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\ % \ab_{t'}^\top \xb - b_{t'}
    %& l_{it} = \min \{ -s_{\theta_{t'}}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber \\ %
    %& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT \setminus \{ \text{root} %\}\nonumber \\
    %& z_{it} \leq a_t \nonumber \\
    %& z_{it} \in [0, 1], a_t \in \{0,1\}. \nonumber
\end{align}
Here we have removed the first three constraints in eq.~\ref{eq:lp_no_prune} as they are a deterministic computation independent of $\zb_1,\ldots,\zb_n,\ab$. Further $p(t)$ indicates the parent of node $t$. The added constraint $a_t \leq a_{p(t)}$ ensures that child nodes $t$ are pruned if parent nodes $p(t)$ are pruned. While the new constraint $z_{it} \leq a_t$ ensures that no point $\xb_i$ can reach node $t$ if node $t$ is pruned. %In the above we have assumed fixed tree parameters $\theta_t$.



%%%%%%%%%%%%%%%%%%%
% OLD STUFF BELOW %
%%%%%%%%%%%%%%%%%%%

% We design a differentiable linear program (LP) that sparsely approximates an integer linear program (ILP) that is inspired by the mixed-integer program (MIP) of \citet{bertsimas2017optimal}.

% We introduce the following variables for our ILP:
% \begin{itemize}
%     % \item $\ab_t \in \mathbb{R}^d$: the splitting parameter for node $t \in \cT_B$
%     % \item $b_t \in \mathbb{R}$: the splitting threshold for node $t \in \cT_B$
%     \item $d_t \in \{0,1\}$: is node $t \in \cT$ active or not (i.e., 0 if it has it been pruned)
%     %if node $t \in \cT_B$ splits or not (if not we force all points to a leaf node)
%     \item $z_{it} \in \{0,1\}$: if $\xb_i$ reaches node $t \in \cT$
%     %\item $l_t \in \{0,1\}$: if node contains any points $t \in \cT_L$
%     %\item $c_{kt} \in \{0,1\}$: if node $t \in \cT_L$ predicts class $k$ (let $\cb_t$ be the $k$-dimensional indicator vector)
%     %\item $q_{ik} \in \{0,1\}$: if $\xb_i$ is predicted class $k$
% \end{itemize}

% % HERERERE:
% % We first observe that the following ILP produces
% % \begin{align}

% % \end{align}

% Given these variables we propose the following ILP:
% \begin{align}
%     \max \;\;& \frac{1}{nT} \sum_{i=1}^n \sum_{t \in \cT} \Bigg( \sum_{m \in A_R(t)} (\ab_m^\top \xb_i - b_m) z_{it} + \sum_{m' \in A_L(t)} ( b_{m'} - \ab_{m'}^\top \xb_i) z_{it} \Bigg) + \frac{\alpha}{T} \sum_{t \in \cT} \eta_t d_t \label{eq:ilp} \\% \in   \sum  (y_i - \langle \boldsymbol{\eta}^\top, \zb_i \rangle )^2   %+ \alpha \sum_{t \in \cT_B} d_t     % \Big( \sum_{j \in \cT_L} z_{it} \cb_{t} \Big) \label{eq:ilp} \\\
%     %\mbox{s.t.}\;\;& \sum_{k=1}^K c_{kt} = l_t, \;\;\; \forall t \in \cT_L \\
%     \mbox{s.t.}\;\;& \ab_m^\top \xb_i \geq b_m - (1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_R(t), \\
%     & \ab_m^\top (\xb_i + \mu)  \leq b_m + (1 + \mu)(1 - z_{it}), \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \forall m \in A_L(t), \\
%     %&\sum_{t \in \cT} z_{it} = d_t, \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq l_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     %&z_{it} \leq d_t, \forall t \in \cT, \\
%     %&l_{t} \leq d_t, \forall t \in \cT, \\
%     %&\sum_{i=1}^n z_{it} \geq N_{\mbox{min}} l_t, \;\;\; \forall t \in \cT, \;\;\;  i = 1, \ldots, n, \\
%     &z_{it} \leq d_t, \forall t \in \cT,  \;\;\; i = 1, \ldots, n, \\
%     & d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \\
%     & z_{ti} \leq z_{p(t)i}, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{ti} + z_{s(t)i} \leq 1, \;\;\; \forall t \in \cT \mbox{ (except root)}, \;\;\;  i = 1, \ldots, n, \\
%     & z_{\textrm{root}i} = 1, \;\;\; \forall i = 1, \ldots, n, \\
%     & d_{\textrm{root}} = 1, \\
% % & \sum_{t \in \cT_L} z_{it} = 1, \;\;\; \forall i = 1, \ldots, n, \\
% % %    & \sum_{k=1}^K c_{kt} = 1, \;\;\; \forall t \in \cT_L, \\
% % 0-c
% % 1-c
% % 1-1
% % 0-1
% % 0-0
% % 1-0
% %     \sum_{t \in \cT_L} z_{it} + c_{tk} \leq p_{ik}, \;\;\; \forall t \in \cT_L, \\
% %     \sum_{t \in \cT_L} \sum_{k=1}^K  k z_{it} c_{tk}
% %     \sum_{t \in \cT_L} z_{it}
% %     \sum_{k=1}^K k c_{tk} = p_{t}
% %     z_{it}
%     & z_{it} \in \{0, 1\}, \;\;\; i = 1, \ldots, n, \;\;\; \forall t \in \cT, \\
%     & d_t \in \{0, 1\} \;\;\; \forall t \in \cT.
% \end{align}
% where $p(t)$ is the parent node of node $t$ , $s(t)$ is the sibling node of node $t$, $\mu$ is a small constant (e.g., $5 \times 10^{-3})$, and $\boldsymbol{\eta}, \ab, b, \xb, y$ are all inputs. %Thus, the multiplication between $\cb_t$ and $z_{it}$ is the only quadratic term, all constraints are linear.

% We explain each line now:
% \begin{itemize}
%     \item (1): This line encourages z to represent the tree by zeroing out the term it is multiplied with, if that term is negative, and vice-versa.
%     % \item (1): This line takes the representation $\zb_i \in \{0, 1\}^T$ that describes the path that $\xb_i$ traverses through the tree and scores it by $\boldsymbol{\eta}$.
%     \item (2)/(3): These enforce points to follow the rules of the tree, see equations (9)-(14) in \citet{bertsimas2017optimal}.
%     \item (4): This ensures that a point does not go to a node if it has been pruned, i.e., $d_t = 0$.
%     \item (5): This ensures that a child node is pruned if its parent is pruned.
%     \item (6): Prevents a point $\xb$ from going to a child node if it does not go to a parent node.
%     \item (7): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (8)/(9): The root cannot be pruned and every point should go through it.
%     % \item
%     % %a child node from branching if a parent node doesn't branch (i.e., $d_{p(t)} = 0$).
%     % \item (4): This ensures that no points $\xb$ go to node $t$ if $l_t$ decides so. Or equivalently makes $l_t=1$ if points go to node $t$.
%     % \item (5): This makes sure that $l_t=0$ (i.e., no points go to node $t$) if that node has been pruned (i.e., $d_t=0$).
%     % \item (6): This enforces a minimum number of points $N_{\mbox{min}}$ at each leaf node.
%     % \item (7)/(8): (optional) As we assume inputs $\xb$ are bounded in $[0,1]^d$ we restrict our splitting parameters to fall in the same range $[0,1]$.
%     % %\item (8)/(9): This prunes the full tree. Specifically, this ensures that we send points left at branch node $t$ if $d_t=0$ (i.e., if we do not split at node $t$). It does so by ensuring that $\ab_t=0$ and $b_t=0$ if $d_t=0$.
%     % \item (10):
%     % \item (11): Prevents a point from going to both a node $t$ and its sibling node $s(t)$.
%     \item (10)/(11): Ensures variables are binary.
% \end{itemize}

% Relaxing $z_{it} \in [0,1]$ allows points to partially reach multiple nodes. We can think of this as each point as having some probability of going down multiple paths. %Relaxing $l_t \in [0,1]$ allows leaf nodes $t$ to partially contain points. As above this can be thought of as nodes containing points with some probability.
% Relaxing $d_t \in [0,1]$ allows nodes $t$ to be partially active. This can be thought of as a distribution over trees.

\subsection{Learning Tree Parameters}

A natural approach to learn splitting parameters $\theta_t$ would be to do so in the MIP itself, as in the optimal tree literature. However, this would severely restrict allowed splitting functions as even linear splitting functions can only practically run on at most thousands of training inputs \citep{bertsimas2017optimal}. Instead, we propose to learn $s_{\theta_{t}}$ via gradient descent.
% as function more complicated than linear/quadratic
% most high-performance MIP solvers (Gurobi, GLPK, SCIP) allow only linear/quadratic constraints
% In a twist from the optimal tree learning literature, instead of learning splitting parameters $\theta_t$ within the MIP
% we regard
% the split weights $\theta_t$ as neural network parameters and not
% variables in the nested optimization problem; we thus learn their value using gradient descent.
% To do so, first note that the first three constraints in eq.~\eqref{eq:ilp_prune} are a
% deterministic computation of the values of $\qb$. Thus we can remove these as constraints, leaving the simpler problem
% \begin{equation}\label{eq:ourilp}
% \begin{aligned}
%     \max_{\zb_1, \ldots, \zb_n, \db} \;\;& \sum_{i=1}^n \zb_i^\top \qb_i + \bm{\eta}^\top \db\\
%     \mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \setminus \{\text{root}\} \\
%     & z_{it} \leq d_t \\
%     & z_{it} \in [0, 1], d_t \in \{0,1\}.
% \end{aligned}
% \end{equation}
To do so, we must be able to compute
%To embed decision tree induction as a differentiable hidden layer in a
%neural network, we require access to
the gradients
$\pfrac{\zb}{\bm{\eta}}$ and $\pfrac{\zb}{\qb}$. However, the solutions of  eq.~\ref{eq:ourilp} are discontinuous and piecewise-constant.

To solve this, we relax the integer constraint on $\ab$ to the interval $[0,1]$ and add quadratic regularization $\nicefrac{1}{2}\sum_i \| \zb_i \|_2^2 + \nicefrac{1}{2} \| \ab \|_2^2$.
Rearranging and negating the objective yields 
%\begin{equation}
\begin{align}
   \mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \argmin_{\zb_1, \ldots, \zb_n, \ab} \;\;& \hlf\sum_{i=1}^n \| \zb_i - \qb_i \|^2 + \hlf \| \bm{\eta} - \ab \|^2 \label{eq:qp_prune}
 \\
    \mbox{s.t. } \forall i \in [n],\;\;& a_t \leq a_{p(t)}, \;\;\; \forall t \in \cT
\setminus \{\text{root}\}  \nonumber \\
    & z_{it} \leq a_t \nonumber \\
    & z_{it} \in [0, 1], a_t \in [0,1]. \nonumber
\end{align}
The regularization makes the objective strongly convex, so
$\mathrm{T}_{\bm{\eta}}$ is continuous and almost everywhere differentiable~\citep{optnet}. 
Rather than relying on generic solvers,
by using the tree structure of the constraints, we derive an efficient specialized algorithm.
%We then show how this view
%gives a direct, efficient computation of the backward pass.
The main insight, shown below, reframes pruned binary tree learning
as isotonic optimization.
\begin{proposition}\label{prop:iso}
Let $\mathcal{C}= \big\{ \ab \in \mathbb{R}^{|\mathcal{T}|} :
a_t \leq a_{p(t)} ~~\text{for all}~~ t \in \mathcal{T} \setminus \{ \text{root}
\} \big\}.$
Consider
\begin{equation}\label{eq:nested_qp_prune}
\ab^\star = \argmin_{\ab\in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\;
\sum_{t \in \mathcal{T}} \Big( \hlf {(a_t - \eta_t)}^2
+ \sum_{i: a_t \leq q_{it}} \hlf {(a_t - q_{it})}^2 \Big)\,.
\end{equation}
Define%
\footnote{Here $\operatorname{Proj}_{\mathcal{S}}(x)$ is the projection of $x$ onto set $\mathcal{S}$. If $\mathcal{S}$ are box constraints, projection amounts to clipping.}
$[z^\star]_{it} = \operatorname{Proj}_{[0, a_t^\star]}(q_{it})$.
Then, $\mathrm{T}_{\bm{\eta}}(\qb_1, \ldots, \qb_n) = \zb^\star_1, \ldots, \zb^\star_n, \ab^\star$.
\end{proposition}
\begin{proof}
The constraints and objective function of eq.~\ref{eq:qp_prune} are separable,
so we may push the minimization \wrt $\zb$ inside the objective, resulting in:
\begin{equation}
\argmin_{\ab \in \mathcal{C} \cap [0,1]^{|\mathcal{T}|}} \;\; \hlf \| \bm{\eta} - \ab \|^2
+ \sum_{t \in \mathcal{T}} \sum_{i=1}^n
\min_{0 \leq z_{it} \leq a_t} \hlf{({z}_{it} - {q}_{it})}^2\,.
\end{equation}
Each of the inner nested minimizations,
$\min_{0 \leq z_{it} \leq a_t} \hlf (z_{it} - q_{it})^2$
is a one-dimensional projection onto box constraints, with solution
$z^\star_{it} = \operatorname{Proj}_{[0, a_t]}(q_{it})$.
%\begin{equation}\label{eq:z_from_d} z_{it} = {[q_{it}]}_{[0, d_t]}.\end{equation}
We may use this result to eliminate $\zb$ from the objective,
noting that
\begin{equation}
\hlf(z^\star_{it} - q_{it})^2 =
\begin{cases}
\hlf~q_{it}^2, & q_{it} < 0\\
0, & 0 \leq q_{it} < a_t\\
\hlf(a_t - q_{it})^2, & q_{it} \geq a_t\\
\end{cases}
\end{equation}

the first two conditions are constants \wrt $a_t$
%As a function of $a_t$, the first two conditions are constants.
Thus, the objective functions eq.~(\ref{eq:qp_prune}) and eq.~(\ref{eq:nested_qp_prune})
differ by a constant. As their constraints are also the same, they have equivalent minimizers $\ab^\star$.
%This leaves us with the equivalent problem in $\db$,
%\begin{equation}\label{eq:nested_qp_prune}
%\begin{aligned}
    %\min_{\bm{d}} \;\;&
%\sum_t \Big( \hlf {(d_t - \eta_t)}^2
%+ \sum_{i: d_t \leq q_{it}} \hlf {(d_t - q_{it})}^2 \Big) \\
%\mbox{s.t.}\;\;& d_t \leq d_{p(t)}, \;\;\; \forall t \in \cT \\
%& d_t \in [0,1].
%\end{aligned}
%\end{equation}
%After solving this problem, we may use \Eqref{eq:z_from_d} to get
%the optimal $\zb$ (and likewise for gradients, using the chain rule.)
\end{proof}
\begin{algorithm}[t]\small
\caption{Latent decision tree induction via isotonic optimization.\label{alg}}
\begin{algorithmic}[1]
%\State \textbf{Input:} $\eta, \qb$; ~~~ \textbf{Output:} $\db$.
%\State \textbf{Initialize:}
\State initial partition
$\mathcal{G} \leftarrow \big\{ \{1\}, \{2\}, \cdots \}
\subset 2^\mathcal{T}$
\ForAll {$G \in \mathcal{G}$}
\State $d_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\Comment{Proposition~\ref{prop:scalar_subproblem}}
\EndFor
\While {exists $t$ such that $a_t > a_{p(t)}$}
\State $t_\text{max} \leftarrow \argmax_t \{a_t: a_t > a_{p(t)}\}$
\State merge $G \leftarrow G \cup G'$ where $t \in G$ and $p(t) \in G'$.
\State update  $a_G \leftarrow \argmin_a \sum_{t \in G} g_t(a)$
\Comment{Proposition~\ref{prop:scalar_subproblem} again}
\EndWhile
\end{algorithmic}
\end{algorithm}
\paragraph{Efficiently inducing trees as isotonic optimization.}
From Proposition~\ref{prop:iso},
notice that eq.~\ref{eq:nested_qp_prune} is an instance of tree-structured isotonic
optimization:
the objective decomposes over \emph{nodes}, and the inequality constraints
correspond to edges in a rooted tree:
\begin{equation}\label{eq:nested_qp_prune_isotonic}
\argmin_{\ab \in \mathcal{C}} \sum_{t \in \mathcal{T}} g_t(a_t)\,,
% \qquad \text{subject to}\qquad d_t \leq d_{p(t)}~\text{for all }t
%\in \cT \setminus \{ \text{root}\},
~~~~\text{where}~~~~ g_t(a_t) =
\hlf {(a_t - \eta_t)}^2
+\!\sum_{i: a_t \leq q_{it}}\!\!\hlf {(a_t - q_{it})}^2  + \iota_{[0,1]}(a_t).
\end{equation}
where $\iota_{[0,1]}(a_t)\!=\!\infty$ if $a_t \notin [0,1]$ and $0$ otherwise.
This problem can be solved by a generalized \emph{pool adjacent violators} (PAV)
algorithm: Obtain a tentative solution by ignoring the constraints, then
iteratively remove violating edges $a_t > a_{p(t)}$ by \emph{pooling together}
the nodes at the end points. At the optimum, the nodes are organized into a
partition $\mathcal{G} \subset 2^\mathcal{T}$, such that if two nodes $t, t'$
are in the same group $G \in \mathcal{G}$, then $a_t = a_t' \coloneqq a_G$.

When the inequality constraints are the edges of a rooted tree, as is the case
here, the PAV algorithm finds the optimal solution in at most $|\mathcal{T}|$ steps,
where each involves updating the $a_G$ value for a newly-pooled group by solving
a one-dimensional subproblem of the form \citep{yu2016exact}\footnote{Compared to \citet{yu2016exact}, our tree inequalities are in the opposite
direction.  This is equivalent to a sign flip of parameter $\ab$, \ie,
to selecting the \emph{maximum} violator rather than the minimum one at each
iteration.}
\begin{equation}\label{eq:scalar_subproblem}
a_G = \argmin_{a \in \bR} \sum_{t \in G} g_t(a)\,,
\end{equation}
resulting in Algorithm~\ref{alg}.
It remains to show how to solve eq.~\ref{eq:scalar_subproblem}. The next
result gives an exact and efficient solution,
with an algorithm that requires finding the nodes with highest
$q_{it}$ (\ie, the nodes where $\xb_i$ is most highly encouraged to traverse).

\begin{proposition}\label{prop:scalar_subproblem}%
The solution to the one-dimensional problem in
eq.~(\ref{eq:scalar_subproblem}) for any $G$ is given by
\begin{equation}\argmin_{a \in \bR} \sum_{t \in G} g_t(a) =
\operatorname{Proj}_{[0,1]}\big(a(k^\star)\big) \quad \text{where}\quad a(k) \coloneqq
\frac{\sum_{t \in G} \eta_t + \sum_{(i,t) \in S(k^\star)} q_{it}}{|G|+k^\star},
\end{equation}
$S(k) = \{j^{(1)}, \ldots, j^{(k)}\}$ is the set of indices $j=(i,t) \in
\{1, \ldots, n\} \times G$ into
the $k$ highest values of $\qb$, \ie,
$q_{j^{(1)}} \geq
q_{j^{(2)}} \geq \ldots \geq
%q_{j^{(k)}} \geq \ldots \geq
q_{j^{(m)}}$,
and $k^\star$ is the smallest $k$ satisfying
$a(k) > q_{j^{(k+1)}}$.
\end{proposition}

\begin{proof}
Let $G \subset \mathcal{T}$ be a subset of (pooled) node indices.
We seek to solve
\begin{equation}\label{eq:subproblem-explicit}
\argmin_{a \in \bR} \sum_{t \in G} g_t(a)
~:=~
\argmin_{a \in [0, 1]} \sum_{t \in G}
\hlf {(a - \eta_t)}^2
+ \sum_{i: a \leq q_{it}} \hlf {(a - q_{it})}^2
\end{equation}
Note that the final summation implicitly depends on the unknown $a$.
But, regardless of the
value of $a$, if $q_{it} \leq q_{i't'}$ and $q_{it}$ is included in the sum, then $q_{i't'}$ must also be included by transitivity.
We may therefore characterize the solution $a^\star$ via the number
of active inequality constraints
$k^\star = \big| \{(i, t) : a^\star \leq q_{i,t} \}\big|$.
We do not know $a^\star$, but it is trivial to find by testing all possible values of $k$. For each $k$, we may find the set $S(k)$ defined in the proposition. For a given $k$, the candidate objective is
\begin{equation}
J_k(a) = \sum_{t \in G} \hlf(a - \eta_t)^2 + \sum_{(i,t) \in S(k)} \hlf(a - q_{it})^2
\end{equation}
and the corresponding $a(k)$ minimizing it can be found by setting the gradient
to zero:
\begin{equation}
J'_k(a)
= \sum_{t \in G} (a - \eta_t)
+ \sum_{(i,t) \in S(k)} (a - q_{i,t})
:= 0
\quad
\iff
\quad
a(k) = \frac{\sum_{t \in G} \eta_t + \sum_{(i,t) \in S(k)} q_{it}}{|G|+k}.
\end{equation}
Since $|S(k)|=k$ and each increase in $k$ adds a non-zero term to the
objective, we must have $J_1\big(a(1)\big) \leq J_1\big(a(2)\big) \leq
J_2\big(a(2)\big) \leq \ldots$,
so we must take $k$ to be as small as possible,
while also ensuring the condition $|\{(i,t) : a(k) \leq q_{it}\}| = k$,
or, equivalently, that $a(k) > q_{j^{([k+1])}}$.
The box constraints may be integrated
at this point via clipping, yielding $a^\star =
\operatorname{Proj}_{[0,1]} \big(a(k^\star)\big)$.
\end{proof}

\paragraph{Benchmarking solver times}
We study the running time of Algorithm~\ref{alg} depending on the number of data points $n$ and the chosen tree depth $D$.
We compare its solving time with the time needed by the popular convex optimization framework {\bf Cvxpy}~\citep{diamond2016cvxpy, agrawal2018rewriting} to solve Problem~\ref{eq:qp_prune} with OSQP solver~\citep{osqp}\footnote{We ran experiments with the commercial solver GUROBI~\citep{gurobi} but didn't find significant differences with using OSQP.}.
We report the solving times in Figure~\ref{fig:alg-time}, where we vary one parameter $n$ or $D$ at a time and fix the other.
The algorithm that we specifically designed to solve Problem~\eqref{eq:qp_prune} is several magnitude faster than the considered generic solver.

\begin{figure}
    \centering
    \subfigure[Fixed number of points $n = 100$]{\includegraphics[width=0.45\textwidth]{figures/time-depth.pdf}
    }\hfill
    \subfigure[Fixed tree depth $D = 3$]{\includegraphics[width=0.45\textwidth]{figures/time-points.pdf}
    }
    \caption{Comparison of Algorithm~\ref{alg}'s running time (ours) with the running time of {\bf Cvxpy} with OSQP solver. $n$ takes values in a range that covers common choices of batch size. Time and $n$ axis are represented in logarithmic scale.
    }
    \label{fig:alg-time}
\end{figure}

\paragraph{Backward pass and efficient implementation details.}
Algorithm~\ref{alg} is a sequence of differentiable operations that can be
implemented \emph{as is} in automatic differentiation frameworks. However,
because of the prominent loops and indexing operations, we opt for a low-level
implementation as a \texttt{C++} extension.
Since the $\qb$ values are constant \wrt $\ab$, we only need to sort them
once as preprocessing. % in \vlad{TODO but should be sth like $\mathcal{O}(d(n \log n))$}.
For the backward pass, rather than relying on automatic
differentiation, we make two remarks about the form of $\ab$.
Firstly, its elements are organized in groups, \ie, $a_t = a_t' = a_G$ for $\{t,
t'\} \subset G$. Secondly, the value $a_G$ inside each group
depends only on  the optimal support set $S^\star_G \coloneqq S(k^\star)$ as
defined for each subproblem  by Proposition~\ref{prop:scalar_subproblem}.
Therefore, in the forward pass, we must store only the node-to-group mappings
and the sets $S^\star_G$. Then, if $G$ is the group of node $t$,
\begin{equation*}
\pfrac{a^\star_t}{\eta_{t'}} = \begin{cases}
\frac{1}{|G| + k^\star},
& 0 < a^\star_t < 1 ~\text{and}~
t' \in G,\\
0,&\text{otherwise.}
\end{cases}
~~
\pfrac{a^\star_t}{q_{it'}} = \begin{cases}
\frac{1}{|G| + k^\star},
& 0 < a^\star_t < 1,
~\text{and}~
(i,t') \in S^\star_G,\\
0,&\text{otherwise.}
\end{cases}.
\end{equation*}


\subsection{The Overall Objective}
% skip connection = concatenation of input and tree path
% MLP = [Linear, Elu, Dropout] * num layers + Linear
We are now able to describe the overall optimization procedure that simultaneously learns tree parameters (a) input traversals $\zb_1, \ldots, \zb_n$; (b) tree pruning $\ab$; and (c) split parameters $\theta_t$. Given this tree, we will additionally learn a function $f_\phi(\zb, \xb)$ to minimize an arbitrary loss $\ell(\cdot)$ as follows,
\begin{equation}
\begin{aligned}
    \min_{\bm{\theta},\bm{\eta},\bm{\phi}}\;\;& \sum_{i=1}^n \ell\big(f_\phi(\xb_i, \zb_i)\big) + \lambda \| \bm{\eta} \|_{\Omega} \label{eq:obj} \\
    \mbox{where}\;\;& \zb_1, \ldots, \zb_n, \ab := \mathrm{T}_{\bm{\eta}}\big(q_{\bm{\theta}}(\xb_1), \ldots, q_{\bm{\theta}}(\xb_n)\big)\,.
\end{aligned}
\end{equation}
Recall $\mathrm{T}_{\bm{\eta}}(\cdot)$ is the solution to the tree program (eq.~\ref{eq:qp_prune}), so we may update the parameters $\bm{\eta}$ and $\bm{\theta}$ by back-propagation. Here we define $q_{\theta}(\xb_i) := \qb_i$ to make explicit the dependence of $\qb_i$ on $\theta$. The regularization $\| \cdot \|_{\Omega}$ can be any norm (in practice we find $\Omega=\infty$ to perform the best.)

%Specifically, $\qb_i$ is given by a  deterministic function $q_{\theta}(\xb_i)$.

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}


% Given a loss function $\ell$
% Given this, we can write the overall objective
% \matt{Working on this}


% In the following, we train via end-to-end back-propagation a Deep Neural Network built as a composition of a Latent Tree (LT) layer followed by a MultiLayer Perceptron (MLP) predictor.
% We also design an optional skip connection between the input $\xb$ and the predictor to circumvent the LT layer, as illustrated in Figure~\ref{fig:arch}.
% The skip connection is particularly useful for regression tasks or when the predictor is a single linear layer, as in these scenarios relying only on the coarse tree representation may hinder results.
% We construct the MLP predictor as a sequence of fully connected layers, with Elu activation~\citep{clevert2015fast} and dropout~\citep{srivastava2014dropout}, followed by a final fully connected layer.
% We refer to the set of predictor's parameters as $\phi$.
% Given a fixed tree depth, the LT layer's training parameters consist of pruning parameter $\bm{\eta}$ and splitting parameters $\theta = \{ \bm{\theta}_t\}_{t \in \cT_B}$.

% Our optimization procedure consists in alternating between solving Problem~\ref{eq:qp_prune}, i.e. computing the tree routing $\bm{z}$, and optimizing the model parameters by gradient descent:

% \begin{align}~\label{eq:obj}
%     \bm{d}, \bm{z} &= \mathcal{LT}(\bm{\eta}, \bm{q}) \nonumber \\
%     \min_{\phi,\theta,\bm{\eta}} \;\;& \ell(\phi, \xb, \bm{z}, y) + \lambda \; \| \bm{\eta} \|_{\infty}  \\
%     \mbox{with}\;\;& q_{it} = \min \{ r_{it}, l_{it} \} \nonumber \\
%     & r_{it} = \min \{ \bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_R(t) \} \nonumber \\
%     & l_{it} = \min \{ -\bm{\theta}_{t'}(\xb), \;\; \forall t' \in A_L(t) \} \nonumber
% \end{align}

% where $\ell(.)$ is the loss function of choice, depending on the downstream task at hand, measuring the goodness of the predictor's output w.r.t. the target $y$;
% $\lambda$ is the hyper-parameter controlling the trade-off between pruning strength and performance.

% As mentioned before, our formulation allows for integrating any type of split function.
% Depending on the task and on the type of inputs, one could train decision hyper-planes or even more complex functions, such as Convolutional Neural Networks.
% In the following, we make use of decision hyper-planes, and tune whether to apply an Elu activation to their output.
% \vlad{elu is monotonic so I would expect it not to
% change the decision boundary, right? or am I missing something}
% \vale{I'd say that the splits are the same, but the leaf values used as representation are different.}

